COPA: Certifying Robust Policies for Offline Reinforcement Learning against Poisoning Attacks

As reinforcement learning (RL) has achieved near human-level performance in a variety of tasks, its robustness has raised great attention. While a vast body of research has explored test-time (evasion) attacks in RL and corresponding defenses, its robustness against training-time (poisoning) attacks remains largely unanswered. In this work, we focus on certifying the robustness of offline RL in the presence of poisoning attacks, where a subset of training trajectories could be arbitrarily manipulated. We propose the first certification framework, COPA, to certify the number of poisoning trajectories that can be tolerated regarding different certification criteria. Given the complex structure of RL, we propose two certification criteria: per-state action stability and cumulative reward bound. To further improve the certification, we propose new partition and aggregation protocols to train robust policies. We further prove that some of the proposed certification methods are theoretically tight and some are NP-Complete problems. We leverage COPA to certify three RL environments trained with different algorithms and conclude: (1) The proposed robust aggregation protocols such as temporal aggregation can significantly improve the certifications; (2) Our certification for both per-state action stability and cumulative reward bound are efficient and tight; (3) The certification for different training algorithms and environments are different, implying their intrinsic robustness properties. All experimental results are available at https://copa-leaderboard.github.io.

==> [ICLR 2022] COPA/algos-DTPA-radius.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
\setlength{\columnsep}{15pt}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\DontPrintSemicolon

    \KwIn{environment $\gE = (\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{k-1}$, maximum window size $W_{\max}$}
	\KwOut{\sysname robust size at each time step $\{\wbar K_t\}_{t=0}^{H-1}$}
    
    $s_0 \sim d_0$ \Comment*[r]{\scriptsize sample initial state}
    
    \For {$t$ from $0$ to $H-1$} {
        \For {each $a \in \gA$} {
            Compute $n_a(s_t)$ from subpolicies' $\{\pi_i\}_{i=0}^{k-1}$ decisions given $s_t$ \Comment*[r]{\scriptsize $n_a$ is defined in \Cref{subsec:notation}}
        }
        Determine the chosen action $a_t \gets \rlalgodyntmppolicy(s_t)$ and chosen window size $W'$ according to \rlalgodyntmp~(\Cref{def:dtpa-agg})\;
        $p_{\min} \gets \infty$\;
        $\wbar K_t \gets$ \Cref{alg:tpa-radius} \Comment*[r]{\scriptsize use \Cref{alg:tpa-radius} with $W$ replaced by $W'$ to compute $\wbar K_t$}
        $\wbar K_t^D \gets \wbar K_t$\;
        \For {each $a' \in \gA, a' \neq a_t$} {
            \For {each $a'' \in \gA, a'' \neq a_t$} {
                \For {$W^*$ from $1$ to $\min\{W_{\max}, t+1\}$} {
                    $a^\# \gets \argmax_{a_0\neq a', a_0\in \gA} n_{a_0}(s_{t-W^*+1:t})$\;
                    \For {$w$ from $1$ to $\max\{W', W^*\}$} {
                        Compute $\max_{a_0\in \gA} \sigma^w(a_0)$ according to \Cref{eq:L-2}
                    }
                    \For {$i$ from $0$ to $k-1$} {
                        \For {$w$ from $1$ to $\max\{W', W^*\}$} {
                            Compute $\sigma^w(\pi_i(s_{t-w}))$ according to \Cref{eq:L-2}
                        }
                        Compute $g_i$ according to \Cref{eq:L-2}
                    }
                    $\{g^{(i)}\}_{i=1}^k \gets \mathsf{sorted}(\{g_i\}_{i=0}^{k-1}, \mathtt{reverse=True})$\;
                    Compute $n_{a'}^{W^*}, n_{a^\#}^{W^*}, n_{a_t}^{W'}, n_{a''}^{W'}$\;
                    $\mathtt{tmp} \gets W'(n_{a'}^{W^*} - n_{a^\#}^{W^*}) - W^*(n_{a_t}^{W'} - n_{a''}^{W'}) - \1[a' > a_t]$ \;
                    $\mathtt{sum} \gets 0, p \gets 0$\;
                    \For {$j$ from $1$ to $k$} {
                        \If {$\mathtt{sum} + \mathtt{tmp} \ge 0$} {
                            $p \gets j-1$\;
                            \textbf{break}
                        }
                        $p \gets j, \mathtt{sum} \gets \mathtt{sum} + g^{(j)}$
                    }
                    $L_{a',a''}^{W^*, W'} \gets p, \wbar K_t^D \gets \min\{\wbar K_t^D, L_{a',a''}^{W^*, W'}\}$
                }
            }
        }
        $s_{t+1} \sim P(s_t, a_t)$
    }
    
    \KwRet{$\{\wbar K_t^D\}_{t=0}^{H-1}$}

\caption{\sysname per-state certification algorithm for \rlalgodyntmpfullname~(\rlalgodyntmp).}
\label{alg:dtpa-radius}

\end{algorithm}


==> [ICLR 2022] COPA/algos-PA-RL.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified poison sizes along time steps}
\SetKwFunction{funca}{pre-processing}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Pn{\funca{}} {
%     % \Comment*[l]{\footnotesize Preprocessing: given a trained $Q$ network, compute its output range and the \lip constant of its smoothed version}
%     Sample the input states and pass them to the given network $Q$ to compute the minimum value $V_{\min}$ and maximum value $V_{\max}$\;
%     $L=\frac{ V_{\max} - V_{\min} }{\sigma}\sqrt{\nicefrac{2}{\pi}}$\;
% }\;

% \Fn{\funcb{$s,\eps$}} {
    \Comment*[l]{\footnotesize Training Phase}
    
    \KwIn{training dataset $D$, number of partitions $k$}
	\KwOut{\rlalgo policy $\mpi$}
    
    Separate the training data $D$ into $k$ partitions $\{P_i\}_{i=0}^{k-1}$\;
    \For {each partition $P_i$} {
    	$\pi_i \leftarrow $ base policy trained on an partition $P_i$
    }
    $\mpi \leftarrow $ aggregation of $\{\pi_i\}_{i=0}^{k-1}$ via Eq.~\ref{eq:agg}\;
	\KwRet{$\mpi$}
    \columnbreak
    
    
    \Comment*[l]{\footnotesize Testing Phase}
    \KwIn{initial state distribution $d_0$, \rlalgo policy $\mpi$}
	\KwOut{a sequence of certified poison sizes along time steps}

    $s_0 \sim d_0, t \leftarrow 0$ \Comment*[r]{\scriptsize initial state observation}
    \While {$s_t \neq \perp$} {
	    \Comment*[l]{\scriptsize take action according to $\mpi$}
    	$a_t \leftarrow \mpi (s_t)$ \;
   		\Comment*[l]{\scriptsize compute the certified poison size}
    	$I_t \leftarrow \left\lfloor\frac{n_{a_t}(s_t)-\max _{a^{\prime} \neq a_t}\left(n_{a^{\prime}}(s_t)+\mathds{1}_{a^{\prime}<a_t}\right)}{2}\right\rfloor$\;
    	\Comment*[l]{\scriptsize transition to the next state}
    	$s_{t+1} \leftarrow \Gamma(s_t,a_t), t \leftarrow t+1$\;
    }
    \KwRet{ $I_0,I_1, \ldots$ }
% }
\end{multicols}
\caption{\small \textbf{PA-RL}: training, action prediction, and certification
}\label{alg:PA-RL}
\end{algorithm}


==> [ICLR 2022] COPA/algos-PPA-radius.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
\setlength{\columnsep}{15pt}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\DontPrintSemicolon

    \KwIn{environment $\gE = (\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{k-1}$}
	\KwOut{\sysname robust size at each time step $\{\wbar K_t\}_{t=0}^{H-1}$}
    
    $s_0 \sim d_0$ \Comment*[r]{\scriptsize sample initial state}
    
    \For {$t$ from $0$ to $H-1$} {
        \For {each $a \in \gA$} {
            Compute $n_a(s_t)$ from subpolicies' $\{\pi_i\}_{i=0}^{k-1}$ decisions \Comment*[r]{\scriptsize $n_a$ is defined in \Cref{subsec:notation}}
        }
        Determine the chosen action $a_t \gets \rlalgopolicy(s_t)$ according to \rlalgo~(\Cref{def:ppa-agg})\;
        Compute $\wbar K_t$ according to \Cref{eq:ppa-radius} in \Cref{thm:ppa-radius}\;
        $s_{t+1} \sim P(s_t, a_t)$
    }
    
    \KwRet{$\{\wbar K_t\}_{t=0}^{H-1}$}
    
\caption{\sysname per-state certification algorithm for \rlalgofullname~(\rlalgo).}
\label{alg:ppa-radius}

\end{algorithm}


==> [ICLR 2022] COPA/algos-PTA-RL-fixed.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified attack magnitudes along time steps}
\SetKwFunction{funca}{\textsc{ ComputePoisonSize}}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \Fn{\funcb{$s,\eps$}} {
    
    \KwIn{$k$ trained base policies $\{\pi_i\}_{i=0}^{k-1}$, fixed window size $W$, current time step $t$, and state $s_t$}
	\KwOut{action prediction $a_t$ and certification $I_t$}

	\Comment*[l]{\scriptsize Compute the smallest poison size required to alter the action selection from $a_t$ to $a$}
	 \Fn{\funca{$a_t,a,\{n_a^W\},\{c_a^i\}$}} {
		\For { $i$ from $0$ to $k-1$ } {
    		$h_i \leftarrow c_{a_t}^i + W - c_a^i$
    	}
    	sort $h_0, \ldots, h_{k-1}$ decreasingly\;
% 		$\delta \leftarrow \left\lfloor\frac{n_{a_t}^W-\left(n_{a}^W+\mathds{1}_{a<a_t}\right)}{2}\right\rfloor$\;
		$\delta \leftarrow n_{a_t}^W-\left(n_{a}^W+\mathds{1}_{a<a_t}\right)$\;
%		$I \leftarrow $ 
		\KwRet smallest $j$ such that $\sum_{i=0}^{j-1} h_i > \delta$\;
	 }

	\Comment*[l]{\scriptsize Initialization}
	\For { $a \in \gA$ } {
		$L_a^W \leftarrow \emptyset$ \Comment*[r]{\scriptsize list of models voting for $a$}
		$n_a^W \leftarrow 0$ \Comment*[r]{\scriptsize count of models voting for $a$}
	}\;
	
	\columnbreak

	\Comment*[l]{\scriptsize Compute temporal aggregated action count}
	\For { $j$ from $0$ to $\min\{W-1,t\}$ } {
		\For { $i$ from $0$ to $k-1$ } {
			$a \leftarrow \pi_i(s_{t-j})$\;
			$L_a^W \leftarrow L_a^W \cup \{ \pi_i \}$\;
			$n_a^W \leftarrow n_a^W + 1$
		}
	}
	
%	$c_a^i \leftarrow $ count of $\pi_i$ in $L_{a}^W$ \textbf{for} { $a \in \gA$ } \textbf{and} { $i$ from $0$ to $k-1$ }
	\For { $a \in \gA$ } {
    	\For { $i$ from $0$ to $k-1$ } {
    		$c_a^i \leftarrow $ count of $\pi_i$ in $L_{a}^W$
    	}
    }



	\Comment*[l]{\scriptsize Compute temporal aggregated action prediction}
	$a_t \leftarrow \argmax_{a \in \gA} n_a^W$\;

    
    \Comment*[l]{\scriptsize Compute certification}
    
%    $m \leftarrow \left\lfloor\frac{n_{a}^W-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}^W+\mathds{1}_{a^{\prime}<a}\right)}{2}\right\rfloor$
    
    
    $I_t \leftarrow \min_{a \in \gA,a \neq a_t}$ \texttt{\textsc{ ComputePoisonSize}}($a_t,a,\{n_a^W\},\{c_a^i\}$) $- 1$
        
    \KwRet{ $a_t,I_t$ }
% }
\end{multicols}
\caption{\small \textbf{PTA-RL}: action prediction and certification
}\label{alg:PTA-RL-fixed}
\end{algorithm}


==> [ICLR 2022] COPA/algos-PTA-RL-flex.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified attack magnitudes along time steps}
\SetKwFunction{funca}{pre-processing}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Pn{\funca{}} {
%     % \Comment*[l]{\footnotesize Preprocessing: given a trained $Q$ network, compute its output range and the \lip constant of its smoothed version}
%     Sample the input states and pass them to the given network $Q$ to compute the minimum value $V_{\min}$ and maximum value $V_{\max}$\;
%     $L=\frac{ V_{\max} - V_{\min} }{\sigma}\sqrt{\nicefrac{2}{\pi}}$\;
% }\;

% \Fn{\funcb{$s,\eps$}} {
    
    \KwIn{$k$ trained base policies $\{\pi_i\}_{i=0}^{k-1}$, maximum window size $U$, current time step $t$, and state $s_t$}
	\KwOut{action prediction $a_t$ and certification $I_t$}

	\Comment*[l]{\scriptsize Initialization}
	\For { $a \in \gA$ } {
		\For { $ W \in \{1,\ldots,  \min\{U, t+1\} \}$} {
			$L_a^{W} \leftarrow \emptyset$\;
			$n_a^{W} \leftarrow 0$
		}
	}

	\Comment*[l]{\scriptsize Compute temporal aggregated action count}
	\For { $W$ from $1$ to $\min\{U,t+1\}$ } {
		\If { $W > 1$ } {
			$ L_a^{W} \leftarrow L_a^{W-1} $\;
			$ n_a^{W} \leftarrow n_a^{W-1} $\;
		}
		\For { $i$ from $0$ to $k-1$ } {
			$a \leftarrow \pi_i(s_{t-W+1})$\;
			$L_a^{W} \leftarrow L_a^{W} \cup \{ \pi_i \}$\;
			$n_a^{W} \leftarrow n_a^{W} + 1$
		}
	}

    \columnbreak	
    
    \Comment*[l]{\scriptsize Compute temporal wise action margin}
	\For { $W$ from $1$ to $\min\{U,t+1\}$ } {
		$a_W^1, a_W^2 \leftarrow$ actions of \nth{1} and \nth{2} highest vote counts among $\{ n_a^{W} \}_{a \in \gA}$\;
		$\Delta_t^{W} \leftarrow n_{a_W^1}^{W} - n_{a_W^2}^{W}$
	}


    
    \Comment*[l]{\scriptsize Compute optimal window size $W_t$ and corresponding action prediction $a_t$}
	$W_t \leftarrow \argmax_{W} \Delta_t^{W}$\;
	$a_t \leftarrow \argmax_{a \in \gA} n_{a}^{W_t}$ \Comment*[l]{\scriptsize \ie, $a_t \leftarrow a_{W_t}^1$}
    
    \Comment*[l]{\scriptsize Compute certification $I_t$}
    
%    $m \leftarrow \left\lfloor\frac{n_{a}^W-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}^Whds{1}_{a^{\prime}<a}\right)}{2}\right\rfloor$
    
    \For {$i$ from $0$ to $k-1$} {
    	$c_i \leftarrow $ count of $\pi_i$ in $L_{a_t}^{W_t}$
    }
    sort $c_0,\ldots,c_{k-1}$ decreasingly\;
    $I_t \leftarrow $ largest $j$ such that $\sum_{i=0}^{j-1}c_i \leq \left\lfloor\frac{\Delta_{t}^{W_t}-\max_{W \neq W_t}\left( \mathrm{sgn}(a_W^1 \neq a_t) \cdot \Delta_{t}^{W}+\mathds{1}_{a_W^1<a}\right)}{2}\right\rfloor$
    
    \KwRet{ $a_t, I_t$ }
% }
\end{multicols}
\caption{\small \textbf{PDTA-RL}: action prediction and certification
}\label{alg:PTA-RL-flex}
\end{algorithm}


==> [ICLR 2022] COPA/algos-TPA-radius.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
\setlength{\columnsep}{15pt}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\DontPrintSemicolon

    \KwIn{environment $\gE = (\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{k-1}$, window size $W$}
	\KwOut{\sysname robust size at each time step $\{\wbar K_t\}_{t=0}^{H-1}$}
    
    $s_0 \sim d_0$ \Comment*[r]{\scriptsize sample initial state}
    
    \For {$t$ from $0$ to $H-1$} {
        \For {each $a \in \gA$} {
            Compute $n_a(s_t)$ from subpolicies' $\{\pi_i\}_{i=0}^{k-1}$ decisions \Comment*[r]{\scriptsize $n_a$ is defined in \Cref{subsec:notation}}
        }
        Determine the chosen action $a_t \gets \rlalgotmppolicy(s_t)$ according to \rlalgotmp~(\Cref{def:tpa-agg})\;
        $p_{\min} \gets \infty$\;
        \For {each $a' \in \gA, a' \neq a_t$} {
            \For {$i$ from $0$ to $k-1$} {
                Compute $h_{i,a_t, a'}$ according to \Cref{eq:tpa-radius-2}
            }
            $\{h_{a_t,a'}^{(i)}\}_{i=1}^k \gets \mathsf{sorted}(\{h_{i,a_t,a'}\}_{i=0}^{k-1}, \mathtt{reverse=True})$\;
            Compute $\delta_{a_t,a'}$\;
            $\mathtt{sum} \gets 0, p \gets 0$\;
            \For {$j$ from $1$ to $k$} {
                \If {$\mathtt{sum} + h_{a_t,a'}^{(j)} > \delta_{a_t,a'}$} {
                    $p \gets j-1$\;
                    \textbf{break}
                }
                $p \gets j, \mathtt{sum} \gets \mathtt{sum} + h_{a_t,a'}^{(j)}$\;
            }
            $p_{\min} \gets \min\{ p_{\min}, p \}$
        }
        $\wbar K_t \gets p_{\min}$\;
        $s_{t+1} \sim P(s_t, a_t)$
    }
    
    \KwRet{$\{\wbar K_t\}_{t=0}^{H-1}$}

\caption{\sysname per-state certification algorithm for \rlalgotmpfullname~(\rlalgotmp).}
\label{alg:tpa-radius}

\end{algorithm}


==> [ICLR 2022] COPA/algos-training.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \small
\setlength{\columnsep}{15pt}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\DontPrintSemicolon

    \KwIn{training dataset $D$, number of partitions $k$, deterministic hash function $h$}
	\KwOut{\sysname subpolicies $\{\pi_i\}_{i=0}^{k-1}$}
    
    \For {$i \in [k]$} {
        $D_i \gets \{\tau \in D \mid h(\tau) \equiv i \ ({\rm mod\ } k)\}$
        \Comment*[r]{\scriptsize Separate the training data $D$ into $k$ partitions}
    }
    \For {each partition $D_i$} {
    	$\pi_i \gets \gM_0(D_i)$ 
    	\Comment*[r]{\scriptsize Subpolicy trained on partition $D_i$ with offline RL algorithm $\gM_0$}
    }
	\KwRet{$\{\pi_i\}_{i=0}^{k-1}$}

\caption{\sysname training protocol.}
\label{alg:training-protocol}

\end{algorithm}


==> [ICLR 2022] COPA/algos-treesearch.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \small
\setlength{\columnsep}{15pt}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{funca}{\textsc{GetActions}}
\SetKwFunction{funcb}{\textsc{Expand}}
\DontPrintSemicolon

    \KwIn{environment $\gE = (\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{k-1}$, aggregated policy $\rlalgopolicy$ or $\rlalgotmppolicy$~(with $W$) or $\rlalgotmppolicy$~(with $W_{\max}$)}
    \KwOut{a map $M$ that maps poisoning size $K$ to corresponding certified lower bound of cumulative reward $\uj_K$}
    
    
    \Comment*[l]{\scriptsize Initialize global variables}
    
    $\mathtt{p\_que} \gets \emptyset$
    \Comment*[r]{\scriptsize initialize an empty priority queue containing tuples of $(\text{state history}s_{0:t},\text{action }a,\text{poisoning size }K,\text{reward }J)$ sorted by increasing $K$}
    
    $J_{\mathrm{global}} \gets \infty$
    \Comment*[r]{\scriptsize initialize global minimum reward}
    
    \Fn{\funca{$s_{0:t},K_{\lim}, \jcur$}}{
        {
        \color{blue}
        $A \gets \mathsf{possibleActions}(s_{0:t}, \{\pi_i\}_{i=1}^{k-1}, \pi_*, K_{\lim})$
        \Comment*[r]{\scriptsize compute the possible action set given state history, subpolicies, aggregation policy $\pi_*$, and poisoning size according to theorems in \Cref{subsec:cert-reward}}
        }
        $\mathtt{a\_list} \gets \emptyset$\;
        \For {each action $a \in \gA$} {
            \If {$P(s,a) = \bot$} {
                \textbf{continue}
                \Comment*[r]{\scriptsize game terminate here, no possible larger or lower cumulative reward to search}
            }
            $\mathtt{a\_list} \gets \mathtt{a\_list} \cup \{a\}$ 
            \Comment*[r]{\scriptsize record possible actions to expand}
        }
        \If {$A \neq \gA$} {
            $K' \gets \min_{\mathsf{possibleActions}(s_{0:t}, \{\pi_i\}_{i=0}^{k-1}, \pi_*, K) \neq A} K$\;
            $A_{\mathrm{new}} \gets \mathsf{possibleActions}(s_{0:t}, \{\pi_i\}_{i=1}^{k-1}, \pi_*, K') \setminus A$
            \Comment*[r]{\scriptsize compute the immediate actions that will possibly be chosen if enlarging the poisoning size}
            \For {each action $a \in A_{\mathrm{new}}$} {
                $\mathtt{p\_que}.\mathsf{push}((s_{0:t}, a, K', \jcur))$
            }
        }
        \KwRet{$\mathtt{a\_list}$}
    }
    
    \Pn{\funcb{$s_{0:t}, K_{\lim}, \jcur$}} {
        \If{$\jcur \ge J_{\mathrm{global}} \wedge (\text{step reward is non-negative})$} {
            \KwRet{}
            \Comment*[r]{\scriptsize pruning}
        }
        $\mathtt{a\_list} \gets$ \funca{$s_{0:t}, \{\pi_i\}_{i=0}^{k-1}, \pi_*, K_{\lim}$}
        \Comment*[r]{\scriptsize compute according to theorems in \Cref{subsec:cert-reward}}
        \If {$\mathtt{a\_list} = \emptyset$} {
            $J_{\mathrm{global}} \gets \min\{ J_{\mathrm{global}}, \jcur \}$\;
            \KwRet{}
        }
        \For {$a \in \mathtt{a\_list}$} {
            $s_{t+1} \gets P(s_t,a)$\;
            \If {$s_{t+1} = \bot$} {
                $J_{\mathrm{global}} \gets \min\{ J_{\mathrm{global}}, \jcur \}$
            }
            \Else {
                \funcb$(s_{0:t+1}, K_{\lim}, \jcur + R(s_t,a))$
            }
        }
    }
    
    
    $M \gets \emptyset$\;
    
    $s_0 \gets d_0$\;
    \Comment*[r]{\scriptsize initial state is $s_0$}
    
    \funcb($s_0, K_{\lim}=0, \jcur=0$)
    \Comment*[r]{\scriptsize expand initial trajectory}
    
    \While {$\mathtt{True}$} {
        \If {$\mathtt{p\_que} = \emptyset$} {
            \textbf{break}
            \Comment*[r]{\scriptsize no state to expand}
        }
        $(s_{0:t},a,K,J) \gets \mathtt{p\_que}.\mathsf{pop}()$
        \Comment*[r]{\scriptsize pop out the first element}
        
        $(\_, \_, K', \_) \gets \mathtt{p\_que}.\mathsf{top}()$
        \Comment*[r]{\scriptsize examine the next element}
        
        $M(K) \gets J_{\mathrm{global}}$
        \Comment*[r]{\scriptsize obtain one new point of certification result}
        
        $s_{t+1} \gets P(s_t,a)$\;
        \funcb$(s_{0:t+1}, K', J + R(s_t,a))$
        \Comment*[r]{\scriptsize expand the tree from the new node}
    }
    
    \KwRet{M}
    \Comment*[r]{\scriptsize indeed the algorithm can terminate at any time within the while loop}
    

\caption{\adasearch: adaptive tree search for cumulative reward certification.}
\label{alg:tree-search}

\end{algorithm}


==> [ICLR 2022] COPA/fig_desc/fig_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightaction}
\settoheight{\utilheightaction}{\includegraphics[width=.17\linewidth]{figs/freeway_action_dqn_30.pdf}}%


\newlength{\legendheightaction}
\setlength{\legendheightaction}{0.4\utilheightaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightaction]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $k=30$}}}
        & \makecell{\small{\textbf{Freeway, $k=50$}}}
        & \makecell{\small{\textbf{Breakout, $k=30$}}}
        & \makecell{\small{\textbf{Breakout, $k=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_dqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_dqn_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_dqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_qrdqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_qrdqn_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_qrdqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_c51_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_c51_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_c51_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($k=30$ and $k=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_50.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionfifty}
\settoheight{\utilheightactionfifty}{\includegraphics[width=.49\linewidth]{figs/Freeway_action_full_dqn_50.pdf}}%


\newlength{\legendheightactionfifty}
\setlength{\legendheightactionfifty}{0.25\utilheightactionfifty}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionfifty][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionfifty]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway}}}
        & \makecell{\small{\textbf{Breakout}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_dqn_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_c51_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($k=30$ and $k=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_full_cum.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionfullcum}
\settoheight{\utilheightactionfullcum}{\includegraphics[width=.34\linewidth]{figs/freeway_action_full_cum_dqn_30.pdf}}%


\newlength{\legendheightactionfullcum}
\setlength{\legendheightactionfullcum}{0.4\utilheightactionfullcum}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionfullcum][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionfullcum]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=30$}}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/freeway_action_full_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
% }
\caption{\small Freeway}\label{tab:cert-rad-freeway}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Breakout, $u=30$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionfullcum]{figs/breakout_action_full_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
% }
\caption{\small Breakout}\label{tab:cert-rad-breakout}
\end{subtable}


}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action stability on Atari games (full results).}
We plot the cumulative histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($u=30$ and $u=50$), and a comparison of three certification methods (PARL, TPARL, and DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise-full}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_full_cum_highway.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionfullcumhighway}
\settoheight{\utilheightactionfullcumhighway}{\includegraphics[width=.34\linewidth]{figs/freeway_action_full_cum_dqn_30.pdf}}%


\newlength{\legendheightactionfullcumhighway}
\setlength{\legendheightactionfullcumhighway}{0.4\utilheightactionfullcumhighway}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionfullcumhighway][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionfullcumhighway]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Highway, $u=30$}}}
        & \makecell{\small{\textbf{Highway, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
% }
% \caption{\small Freeway}
\label{tab:cert-rad-highway}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Highway, $u=100$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_dqn_100.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_qrdqn_100.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionfullcumhighway]{figs/highway_action_full_cum_c51_100.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
}
% \caption{\small Breakout}
\label{tab:cert-rad-highway100}
\end{subtable}


}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action stability on Highway environment (full results).}
We plot the cumulative histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on Highway environment, three partition numbers ($u=30$, $u=50$ and $u=100$), and a comparison of three certification methods (PARL, TPARL, and DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise-full-highway}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_half.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionhalf}
\settoheight{\utilheightactionhalf}{\includegraphics[width=.17\linewidth]{figs/freeway_action_half_dqn_30.pdf}}%


\newlength{\legendheightactionhalf}
\setlength{\legendheightactionhalf}{0.4\utilheightactionhalf}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionhalf][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionhalf]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=30$}}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        & \makecell{\small{\textbf{Breakout, $u=30$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($u=30$ and $u=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_half_cum.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionhalfcum}
\settoheight{\utilheightactionhalfcum}{\includegraphics[width=.17\linewidth]{figs/freeway_action_half_cum_dqn_30.pdf}}%


\newlength{\legendheightactionhalfcum}
\setlength{\legendheightactionhalfcum}{0.4\utilheightactionhalfcum}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionhalfcum][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionhalfcum]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{.925\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=30$}}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        & \makecell{\small{\textbf{Breakout, $u=30$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action stability.}
We plot the cumulative histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide the certification for different aggregation protocols (PARL, TPARL, DPARL) on two games (Freeway and Breakout) and two \#partitions ($u\in \{30, 50\}$).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs with the vertical bar on top denoting the standard deviation.
}%
\label{fig:statewise}
\vspace{-2.2em}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_action_half_cum_50.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionhalfcum}
\settoheight{\utilheightactionhalfcum}{\includegraphics[width=.17\linewidth]{figs/freeway_action_half_cum_dqn_30.pdf}}%


\newlength{\legendheightactionhalfcum}
\setlength{\legendheightactionhalfcum}{0.4\utilheightactionhalfcum}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionhalfcum][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionhalfcum]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{.925\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        & \makecell{\small{\textbf{Highway, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/highway_action_half_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/highway_action_half_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/highway_action_half_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        % & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action stability.}
We plot the cumulative histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide the certification for different aggregation protocols (PARL, TPARL, DPARL) on three environments and \#partitions $u=50$.
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs with the vertical bar on top denoting the standard deviation.
}%
\label{fig:statewise}
\vspace{-2.2em}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_breakout_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightbreakoutaction}
\settoheight{\utilheightbreakoutaction}{\includegraphics[width=.33\linewidth]{figs/breakout_action_dqn_30.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakoutaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakoutaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$k=30$}}
        & \makecell{\small{$k=50$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_dqn_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_dqn_50.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_qrdqn_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_qrdqn_50.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_c51_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_c51_50.png}
\\[-1.2ex]
        & \makecell{\small{robust size $I$}}
        & \makecell{\small{robust size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Histogram of the robust size} computed on Breakout. The results are averaged over $20$ runs, where each run corresponds to one trajectory with randomness in the environment. For ease of comparison, we constrain the maximum trajectory length to be $1000$.
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_breakout_reward.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheightbreakout}
\settoheight{\utilheightbreakout}{\includegraphics[width=.33\linewidth]{figs/breakout_c51_50.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakout}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakout][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=50$}}
        & \makecell{\small{trajectory length $t=75$}}
        & \makecell{\small{trajectory length $t=125$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_125.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_125.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_125.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for the cumulative reward on game Breakout.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under three different certification methods (PA, TPA (W=4), DTPA).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{TODO: fill in conclusion}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_breakout_reward_tight.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightbreakouttight}
\settoheight{\utilheightbreakouttight}{\includegraphics[width=.33\linewidth]{figs/breakout_c51_50_tight.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakouttight}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakouttight][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=50$}}
        & \makecell{\small{trajectory length $t=75$}}
        & \makecell{\small{trajectory length $t=125$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_125_tight.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_125_tight.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_125_tight.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Comparison of the loose and tight lower bound for the cumulative reward certification when $W=1$, evaluated on Breakout.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under two certification methods (loose vs. tight).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{This part may go into appendix if no space in main paper, or we can think about how to merge the figures?}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}

==> [ICLR 2022] COPA/fig_desc/fig_freeway_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightfreewayaction}
\settoheight{\utilheightfreewayaction}{\includegraphics[width=.33\linewidth]{figs/freeway_action_dqn_30.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightfreewayaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightfreewayaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$k=30$}}
        & \makecell{\small{$k=50$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_dqn_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_dqn_50.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_qrdqn_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_qrdqn_50.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_c51_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_c51_50.png}
\\[-1.2ex]
        & \makecell{\small{robust size $I$}}
        & \makecell{\small{robust size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Histogram of the robust size} computed on Breakout. The results are averaged over $20$ runs, where each run corresponds to one trajectory with randomness in the environment. For ease of comparison, we constrain the maximum trajectory length to be $1000$.
}%
\label{fig:statewise}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_freeway_reward.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheighta}
\settoheight{\utilheighta}{\includegraphics[width=.19\linewidth]{figs/freeway_c51_100.pdf}}%


\newlength{\legendheight}
\setlength{\legendheight}{0.5\utilheighta}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheighta][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheight]{figs/legend_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, }$t=100$}}
        & \makecell{\small{\textbf{Freeway, }$t=200$}}
        & \makecell{\small{\textbf{Freeway, }$t=400$}}
        & \makecell{\small{\textbf{Breakout, }$t=50$}}
        & \makecell{\small{\textbf{Breakout, }$t=75$}}\\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize $J$ }}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_dqn_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_dqn_75.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize $J$}}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_qrdqn_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_qrdqn_75.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize $J$}}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_c51_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_c51_75.pdf}
\\[-1.2ex]
        & \makecell{\footnotesize{poison size $I$}}
        & \makecell{\footnotesize{poison size $I$}}
        & \makecell{\footnotesize{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for the on game Freeway.}
We plot the lower bound of \textit{$J$} w.r.t. \textit{poison size} $I$ under three different certification methods (PA, TPA (W=4), DTPA).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of $t$.
\fan{TODO: fill in conclusion}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> [ICLR 2022] COPA/fig_desc/fig_freeway_reward_tight.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightatight}
\settoheight{\utilheightatight}{\includegraphics[width=.33\linewidth]{figs/freeway_dqn_100_tight.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightatight}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightatight][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=100$}}
        & \makecell{\small{trajectory length $t=200$}}
        & \makecell{\small{trajectory length $t=400$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_400_tight.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_400_tight.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_400_tight.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Comparison of the loose and tight lower bound for the cumulative reward certification when $W=1$, evaluated on Freeway.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under two certification methods (loose vs. tight).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{This part may go into appendix if no space in main paper, or we can think about how to merge the figures?}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}

==> [ICLR 2022] COPA/fig_desc/fig_reward.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightrewardall}
\settoheight{\utilheightrewardall}{\includegraphics[width=.16\linewidth]{figs/freeway_c51_100.pdf}}%


\newlength{\legendheightrewardall}
\setlength{\legendheightrewardall}{0.5\utilheightrewardall}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightrewardall][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightrewardall]{figs/legend_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\scriptsize{\textbf{Freeway, }$H=100$}}
        & \makecell{\scriptsize{\textbf{Freeway, }$H=200$}}
        & \makecell{\scriptsize{\textbf{Freeway, }$H=400$}}
        & \makecell{\scriptsize{\textbf{Breakout, }$H=50$}}
        & \makecell{\scriptsize{\textbf{Breakout, }$H=75$}}
        & \makecell{\scriptsize{\textbf{Highway, }$H=30$}}\\
\rowname{\makecell{\scriptsize \textbf{DQN} \\\footnotesize $\uj_K$ }}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_dqn_100.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_dqn_200.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_dqn_400.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_dqn_50.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_dqn_75.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/highway_dqn_30.pdf}
\\
\rowname{\makecell{\scriptsize \textbf{QR-DQN} \\\footnotesize $\uj_K$}}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_qrdqn_100.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_qrdqn_200.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_qrdqn_400.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_qrdqn_50.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_qrdqn_75.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/highway_qrdqn_30.pdf}
\\
\rowname{\makecell{\scriptsize \textbf{C51} \\\footnotesize $\uj_K$}}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_c51_100.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_c51_200.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/freeway_c51_400.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_c51_50.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/Breakout_c51_75.pdf}&
\includegraphics[height=\utilheightrewardall]{figs/highway_c51_30.pdf}
\\[-0.5ex]
        & \makecell{\scriptsize{Poisoning size $K$}}
        & \makecell{\scriptsize{Poisoning size $K$}}
        & \makecell{\scriptsize{Poisoning size $K$}}
        & \makecell{\scriptsize{Poisoning size $K$}}
        & \makecell{\scriptsize{Poisoning size $K$}}
        & \makecell{\scriptsize{Poisoning size $K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for cumulative reward (full results).}
We plot the \textit{lower bound of cumulative reward} \textit{$\uj_K$} w.r.t. \textit{poisoning size} $K$ under three different certification methods (PARL, TPARL ($W=4$), DPARL ($W_{\max}=5$)) with two partition numbers ($u\in \{30, 50\}$).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $H$.}%
\label{fig:reward-full}
\vspace{-1em}
\end{figure}



% \fan{conclusions:
% \begin{enumerate}
%     \item within each figure:
%     \begin{enumerate}
%         \item on Freeway, W=4 mostly more robust than W=1 (exception: QR-DQN: W=1 already very robust?)
%         \item on Breakout, at smaller poison size, W=1 helps; at larger poison size, W=4 helps;
%         \item on both games, \#model=50 more robust than \#model=30
%         \item (more to be added)
%     \end{enumerate}
%     \item along each column: 
%     \begin{enumerate}
%         \item QR-DQN $>$ C51 $>$ DQN
%         \item (more to be added)
%     \end{enumerate}
%     \item along each row: run longer trajectory and can see more interesting results---\eg, Freeway, DQN, $H=400$, reward drops from $4$ to $3$ to $2$ to $1$ at the turning point $I=9$, $I=11$, $I=14$, $I=16$ 
% \end{enumerate}
% }


==> [ICLR 2022] COPA/fig_desc/fig_reward_main.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheightreward}
\settoheight{\utilheightreward}{\includegraphics[width=.3\linewidth]{figs/freeway_c51_100.pdf}}%


\newlength{\legendheight}
\setlength{\legendheight}{0.27\utilheightreward}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightreward][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheight]{figs/legend_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{7mm}@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\normalsize{\textbf{Freeway, $H=200$}}}
        & \makecell{\normalsize{\textbf{Freeway, $H=400$}}}
        & \makecell{\normalsize{\textbf{Breakout, $H=50$}}}
        & \makecell{\normalsize{\textbf{Breakout, $H=75$}}}
        & \makecell{\normalsize{\textbf{Highway, $H=30$}}}\\
\rowname{\makecell{\normalsize \textbf{DQN} \\\normalsize $\uj_K$ }}&
\includegraphics[height=\utilheightreward]{figs/freeway_dqn_200.pdf}&
\includegraphics[height=\utilheightreward]{figs/freeway_dqn_400.pdf}&
\includegraphics[height=\utilheightreward]{figs/breakout_dqn_50.pdf}&
\includegraphics[height=\utilheightreward]{figs/breakout_dqn_75.pdf}&
\includegraphics[height=\utilheightreward]{figs/highway_dqn_30.pdf}
\\
\rowname{\makecell{\normalsize \textbf{QR-DQN} \\\normalsize $\uj_K$}}&
\includegraphics[height=\utilheightreward]{figs/Freeway_qrdqn_200.pdf}&
\includegraphics[height=\utilheightreward]{figs/Freeway_qrdqn_400.pdf}&
\includegraphics[height=\utilheightreward]{figs/Breakout_qrdqn_50.pdf}&
\includegraphics[height=\utilheightreward]{figs/Breakout_qrdqn_75.pdf}&
\includegraphics[height=\utilheightreward]{figs/highway_qrdqn_30.pdf}
\\
\rowname{\makecell{\normalsize \textbf{C51} \\\normalsize $\uj_K$}}&
\includegraphics[height=\utilheightreward]{figs/Freeway_c51_200.pdf}&
\includegraphics[height=\utilheightreward]{figs/Freeway_c51_400.pdf}&
\includegraphics[height=\utilheightreward]{figs/breakout_c51_50.pdf}&
\includegraphics[height=\utilheightreward]{figs/breakout_c51_75.pdf}&
\includegraphics[height=\utilheightreward]{figs/highway_c51_30.pdf}
\\[-0.5ex]
        & \makecell{\normalsize{Poisoning size $K$}}
        & \makecell{\normalsize{Poisoning size $K$}}
        & \makecell{\normalsize{Poisoning size $K$}}
        & \makecell{\normalsize{Poisoning size $K$}}
        & \makecell{\normalsize{Poisoning size $K$}}
\end{tabular}
}
% \caption{\normalsize Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for cumulative reward.}
We plot the \textit{lower bound of cumulative reward bound} \textit{$\uj_K$} w.r.t. \textit{poisoning size} $K$ under three aggregation protocols (PARL, TPARL ($W=4$), DPARL ($W_{\max}=5$)) with two \#partitions $u$, evaluated on three environments with different horizon lengths $H$.
% Each row corresponds to one RL algorithm.
}%
\label{fig:reward}
\vspace{-2.2em}
\end{figure}



% \fan{conclusions:
% \begin{enumerate}
%     \item within each figure:
%     \begin{enumerate}
%         \item on Freeway, W=4 mostly more robust than W=1 (exception: QR-DQN: W=1 already very robust?)
%         \item on Breakout, at smaller poisoning size, W=1 helps; at larger poisoning size, W=4 helps;
%         \item on both games, \#model=50 more robust than \#model=30
%         \item (more to be added)
%     \end{enumerate}
%     \item along each column: 
%     \begin{enumerate}
%         \item QR-DQN $>$ C51 $>$ DQN
%         \item (more to be added)
%     \end{enumerate}
%     \item along each row: run longer trajectory and can see more interesting results---\eg, Freeway, DQN, $H=400$, reward drops from $4$ to $3$ to $2$ to $1$ at the turning point $I=9$, $I=11$, $I=14$, $I=16$ 
% \end{enumerate}
% }


==> [ICLR 2022] COPA/fig_desc/fig_training.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheighttraining}
\settoheight{\utilheighttraining}{\includegraphics[width=.3\linewidth]{figs/Freeway_train_cmp.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheighttraining][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figs/legend_all.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}}
        % & \makecell{\small{\textbf{DQN}}}
        % & \makecell{\small{\textbf{QR-DQN}}}
        % & \makecell{\small{\textbf{C51}}}\\
% \rowname{\makecell{\small \textbf{Freeway} \\\footnotesize $\uj_K$ }}
&
\includegraphics[height=\utilheighttraining]{figs/Freeway_train_cmp-3.pdf}&
\includegraphics[height=\utilheighttraining]{figs/Breakout_train_cmp-3.pdf}&
\includegraphics[height=\utilheighttraining]{figs/Highway_train_cmp-3.pdf}
\\
% \rowname{\makecell{\small \textbf{Breakout} \\\footnotesize $\uj_K$}}&
% \includegraphics[height=\utilheightreward]{figs/Breakout_dqn_75.pdf}&
% \includegraphics[height=\utilheightreward]{figs/Breakout_qrdqn_75.pdf}&
% \includegraphics[height=\utilheightreward]{figs/Breakout_c51_75.pdf}
% \\[-1ex]
%         & \makecell{\footnotesize{Poisoning size $K$}}
%         & \makecell{\footnotesize{Poisoning size $K$}}
%         & \makecell{\footnotesize{Poisoning size $K$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small {\textbf{The \textit{convergence speed} of the proposed partition-based training compared with the standard training.}
For \textit{our proposed training}, we plot all training curves of the sampled $5$ subpolicies in \textcolor{pltblue}{\textbf{blue}}, where each subpolicy is trained on one partition of the dataset. (We do not plot all $50$ curves for visual clarity).
For \textit{standard training}, we plot the training curve of the standard policy in \textcolor{pltred}{\textbf{red}}, where the single policy is trained on the entire dataset.
In Atari games, we train each policy (or subpolicy) for a fixed number of $50$ epochs, where each epoch consumes $1$M randomly sampled training data.
In Highway environment, we train each policy (or subpolicy) for a fixed number of $3000$ epochs, where each epoch consumes $1$K randomly sampled training data.
The offline RL algorithm used is DQN.
}}%
\label{fig:training-cmp}
\end{figure}



% \fan{conclusions:
% \begin{enumerate}
%     \item within each figure:
%     \begin{enumerate}
%         \item on Freeway, W=4 mostly more robust than W=1 (exception: QR-DQN: W=1 already very robust?)
%         \item on Breakout, at smaller poisoning size, W=1 helps; at larger poisoning size, W=4 helps;
%         \item on both games, \#model=50 more robust than \#model=30
%         \item (more to be added)
%     \end{enumerate}
%     \item along each column: 
%     \begin{enumerate}
%         \item QR-DQN $>$ C51 $>$ DQN
%         \item (more to be added)
%     \end{enumerate}
%     \item along each row: run longer trajectory and can see more interesting results---\eg, Freeway, DQN, $H=400$, reward drops from $4$ to $3$ to $2$ to $1$ at the turning point $I=9$, $I=11$, $I=14$, $I=16$ 
% \end{enumerate}
% }


==> [ICLR 2022] COPA/macro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bo}[1]{\textcolor{blue}{(Bo: #1)}}
\newcommand{\ding}[1]{\textcolor{red}{(Ding: #1)}}
\newcommand{\huan}[1]{{\color{violet}(Huan: #1)}}
\newcommand{\fan}[1]{{\color{orange!90!black}(Fan: #1)}}
\newcommand{\fanm}[1]{{\color{orange!90!black}#1}}
\newcommand{\linyi}[1]{{\color{olive}(Linyi: #1)}}
\newcommand{\linyim}[1]{{\color{olive}#1}}
\newcommand{\chejian}[1]{{\color{magenta}(Chejian: #1)}}
\newcommand{\chejianm}[1]{{\color{magenta}#1}}
% \newcommand{\cz}[1]{{\color{red} #1}}
\newcommand{\mo}[1]{{\color{blue}#1}}
\newcommand{\m}[1]{{\color{orange!90!black}#1}}

\newcommand{\more}[0]{{\color{orange}..................}}
\newcommand{\tocite}[0]{{\color{blue}{[Cite]}}}
\newcommand{\TODO}[0]{{\color{blue}{TODO}}}



\usepackage{soul}
\usepackage[normalem]{ulem}
\renewcommand\sout{\bgroup\markoverwith
{\color{magenta}{\rule[.5ex]{2pt}{1pt}}}\ULon}



\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}


\newcommand*{\commentfont}{\fontsize{\tiny}\selectfont}


% % \numberwithin{equation}{section}

% \usepackage{bbm}


% % \usepackage{fancyhdr}
\usepackage{graphicx}
\usepackage{xcolor}


\usepackage{multicol}

% \usepackage{algorithm} 
\usepackage{algorithmic}  
% \usepackage[algo2e]{algorithm2e} 
% \usepackage{algorithm}
% % \usepackage{algorithmic}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{adjustbox}
\SetKwComment{Comment}{$\triangleright$\ }{}





\usepackage{nicefrac}




%% enumerate
\usepackage[shortlabels]{enumitem}
%
%
\usepackage{hyperref}
\usepackage[nameinlink]{cleveref}


\usepackage{longtable}

\usepackage{amsthm}


\usepackage{bbm}
\usepackage{dsfont}

\usepackage{multirow}





\newcommand{\brows}[1]{%
  \begin{bmatrix}
  \begin{array}{c}
  #1
  \end{array}
  \end{bmatrix}
}
\newcommand{\rotvert}{\rotatebox[origin=c]{90}{$\vert$}}
\newcommand{\rowsvdots}{\multicolumn{1}{@{}c@{}}{\vdots}}


% for 1st, 2nd, 3th...
\usepackage[super]{nth}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% definitions and theorems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \makeatletter
% \def\thm@space@setup{%
%   \thm@preskip=1mm plus 0mm minus 1mm
%   \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
% }
% \makeatother


\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{theoremappend}{Theorem}
\theoremstyle{plain}
% \newtheorem{lemma}{Lemma}
\theoremstyle{plain}
\newtheorem{prop}{Proposition}


\usepackage{thmtools}
\usepackage{thm-restate}

\theoremstyle{plain}
\declaretheorem[name=Theorem]{theorem}
\theoremstyle{plain}
% \declaretheorem[name=Lemma]{lemma}


% \newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}{Fact}[section]
\Crefname{fact}{Fact}{Facts}
% \newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{remark}
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
\newtheorem*{remark}{Remark}
% \newtheorem{conjecture}{Conjecture}


% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]


% % inline math allow break
% \makeatletter
% \def\old@comma{,}
% \catcode`\,=13
% \def,{%
%   \ifmmode%
%     \old@comma\discretionary{}{}{}%
%   \else%
%     \old@comma%
%   \fi%
% }
% \makeatother



% new commands
\newcommand{\Tau}{\mathrm{T}}
\newcommand{\eg}[0]{\textit{e.g.}}
\newcommand{\etal}[0]{\textit{et al.}\xspace}
\newcommand{\resp}[0]{\textit{resp.}}
\newcommand{\ie}[0]{\textit{i.e.}}
% \newcommand{\st}[0]{\textit{s.t.}\xspace}
\renewcommand{\wp}[0]{\textit{w.p.}\xspace}
\newcommand{\ow}[0]{\textit{o.w.}\xspace}
\newcommand{\wrt}[0]{\textit{w.r.t.}\xspace}
\newcommand{\eps}[0]{\varepsilon}
\newcommand{\lmb}[0]{\lambda}
\newcommand{\cov}[0]{\mbox{Cov}}
\newcommand{\Exp}[0]{\mbox{Exp}}
\newcommand{\var}[0]{\mbox{var}}
\newcommand{\aeq}[0]{\stackrel{\cdot}{=}}

\newcommand{\wtilde}[0]{\widetilde}
\newcommand{\wbar}[0]{\widebar}


\newcommand{\namepertmag}[0]{maximum perturbation magnitude\xspace}

\newcommand{\namef}[0]{perturbed return function\xspace}
\newcommand{\nameF}[0]{Perturbed return function\xspace}

\newcommand{\namecr}[0]{cumulative reward\xspace}
\newcommand{\namej}[0]{finite horizon cumulative reward\xspace}
\newcommand{\namepj}[0]{poisoned cumulative reward\xspace}

\newcommand{\rlalgo}[0]{PARL\xspace}
\newcommand{\rlalgotmp}[0]{TPARL\xspace}
\newcommand{\rlalgodyntmp}[0]{DPARL\xspace}
\newcommand{\rlalgoall}[0]{\{T\}PA\xspace}

\newcommand{\rlalgofullname}[0]{Per-State Partition Aggregation\xspace}
\newcommand{\rlalgotmpfullname}[0]{Temporal Partition Aggregation\xspace}
\newcommand{\rlalgodyntmpfullname}[0]{Dynamic Temporal Partition Aggregation\xspace}

\newcommand{\rlalgopolicy}[0]{\pi_{\mathrm{P}}}
\newcommand{\rlalgotmppolicy}[0]{\pi_{\mathrm{T}}}
\newcommand{\rlalgodyntmppolicy}[0]{\pi_{\mathrm{D}}}


\newcommand{\ebound}[0]{expectation bound\xspace}
\newcommand{\pbound}[0]{percentile bound\xspace}

\newcommand{\sigrtj}[0]{$\sigma$-randomized trajectory\xspace}
\newcommand{\sigrtjs}[0]{$\sigma$-randomized trajectories\xspace}
\newcommand{\sigrpi}[0]{$\sigma$-randomized policy\xspace}


\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\uit}[1]{\underline{\textit{#1}}}
\newcommand{\texttc}[1]{\texttt{\textsc{#1}}}


\newcommand{\dtv}[0]{\mathrm{D}_{\mathrm{TV}}}

\newcommand{\rzero}[0]{\rightarrow0}
\newcommand{\rinf}[0]{\rightarrow\infty}
\newcommand{\smax}[0]{\scriptsize \mbox{max}}
\newcommand{\smin}[0]{\scriptsize \mbox{min}}


\newcommand{\Eop}{\mathop{\mathbb E}}
%\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
%\newcommand{\argmin}{\mathop{\mathrm{argmin}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% project specific macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\RL}[0]{Reinforcement Learning\xspace}
\newcommand{\rl}[0]{reinforcement learning\xspace}
\newcommand{\lip}[0]{Lipschitz\xspace}
\newcommand{\env}[0]{environment\xspace}   
\newcommand{\qpi}[0]{Q^\pi}
\newcommand{\tpi}[0]{\tilde\pi}
\newcommand{\mpi}[0]{\pi_{\cal M}}
\newcommand{\tmpi}[0]{\tilde \pi_{\cal M}}
\newcommand{\wqpi}[0]{\wtilde Q^\pi}

\newcommand{\vmin}[0]{V_{\min}}
\newcommand{\vmax}[0]{V_{\max}}
\newcommand{\jmin}[0]{J_{\min}}
\newcommand{\jmax}[0]{J_{\max}}
\newcommand{\jcur}[0]{J_{\rm cur}}
\newcommand{\jglobal}[0]{J_{\rm global}}
\newcommand{\sm}[0]{\cal S_{\rm{m}}^\eps}
\newcommand{\epsball}[0]{\cal B^\eps}
\newcommand{\epsbball}[0]{\cal B^{\bar\eps}}

\renewcommand{\vert}[0]{\oplus}
\newcommand{\vertt}[2]{\vert_{t=#1}^{#2}}


\newcommand{\uj}[0]{\underline{J}}
\newcommand{\uje}[0]{\underline{J_E}}
\newcommand{\ujp}[0]{\underline{J_p}}

\newcommand{\ujefull}[0]{E\left[J_\eps^H(\pi')\right]}
\newcommand{\jfull}[0]{J_\eps^H(\pi')}





% \newcommand{\staters}[0]{\textsc{LocalRS-Act}\xspace}
% \newcommand{\glbrs}[0]{\textsc{GlobalRS-CR}\xspace}
% \newcommand{\adasearch}[0]{\textsc{LocalRS-CR}\xspace}

\newcommand{\sysname}[0]{\textsc{COPA}\xspace}

\newcommand{\staters}[0]{\textsc{\sysname-LoAct}\xspace}
\newcommand{\glbrs}[0]{\textsc{\sysname-GRe}\xspace}
\newcommand{\adasearch}[0]{\textsc{\sysname-Search}\xspace}

\newcommand{\NP}{\mathsf{NP}}

\newcommand{\norm}[1]{\lVert{#1}\rVert}
\newcommand{\dotp}[2]{\langle {#1},{#2} \rangle}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\bbm}[1]{\mathbbm{#1}}


\newcommand{\pmat}[2]{
                    \begin{pmatrix}
                    #1\\#2
                    \end{pmatrix}
                    }
\newcommand{\intt}[2]{\int_{#1}^{#2}}
\renewcommand{\cal}[1]{\mathcal{#1}}
% \renewcommand{\bf}[1]{\mathbf{#1}}
\newcommand{\tbf}[1]{{\textbf{#1}}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% spacing (blank space)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \usepackage{float}
% \setlength{\textfloatsep}{0.2cm}

\setlength{\abovedisplayskip}{-0.1mm}
\setlength{\belowdisplayskip}{-0.1mm}
\setlength{\abovedisplayshortskip}{-0.1mm}
\setlength{\belowdisplayshortskip}{-0.1mm}


\usepackage{titlesec}
\titlespacing{\section}{0pt}{6pt}{6pt}
\titlespacing{\subsection}{0pt}{6pt}{6pt}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{pltred}{RGB}{183, 85, 86}
\definecolor{pltblue}{RGB}{85, 113, 172}



% \titlespacing*{\section}
% {0pt}{2.5ex plus 0.5ex minus .2ex}{4.3ex plus .2ex}
% \titlespacing*{\subsection}
% {0pt}{2.5ex plus 0.5ex minus .2ex}{4.3ex plus .2ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% tables and figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \usepackage{float}
% \setlength{\textfloatsep}{0.1cm}

\usepackage{subcaption}

\usepackage{booktabs}
\usepackage{makecell}


\usepackage{wrapfig}

% \newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
% \newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
% \newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
% \newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

\newcommand\given[1][]{\:#1\vert\:}


% \makeatletter
% \newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\ignorespaces\fi}
% \makeatother


\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\ignorespaces\fi}
\makeatother



\usepackage{multirow}
\usepackage{subcaption}
\usepackage{siunitx}
\usepackage{chemformula}
\usepackage{collcell}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{xcolor,colortbl}

\newcommand{\CC}[1]{\cellcolor{gray!#1}}
\colorlet{tabgray}{gray!30} 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% widebar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% renew paragraph definition to save space
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\paragraph}[1]{\textbf{#1}\quad}

==> [ICLR 2022] COPA/main_text.tex <==

% \documentclass{article} % For LaTeX2e
% \usepackage{iclr2022_conference,times}

% % Optional math commands from https://github.com/goodfeli/dlbook_notation.
% \input{math_commands.tex}
% \input{macro}

% %\usepackage{hyperref}
% %\usepackage{url}

% \usepackage{silence}
% \WarningFilter{relsize}{Font size}
% \title{\sysname: Certifying Robust Policies for Offline Reinforcement Learning against Poisoning Attacks}

% % Authors must not appear in the submitted version. They should be hidden
% % as long as the \iclrfinalcopy macro remains commented out below.
% % Non-anonymous submissions will be rejected without review.

% \author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
% about author (webpage, alternative address)---\emph{not} for acknowledging
% funding agencies.  Funding acknowledgements go at the end of the paper.} \\
% Department of Computer Science\\
% Cranberry-Lemon University\\
% Pittsburgh, PA 15213, USA \\
% \texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
% \And
% Ji Q. Ren \& Yevgeny LeNet \\
% Department of Computational Neuroscience \\
% University of the Witwatersrand \\
% Joburg, South Africa \\
% \texttt{\{robot,net\}@wits.ac.za} \\
% \AND
% Coauthor \\
% Affiliation \\
% Address \\
% \texttt{email}
% }

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to \LaTeX{} to determine where to break
% % the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% % puts 3 of 4 authors names on the first line, and the last on the second
% % line, try using \AND instead of \And before the third author name.

% \newcommand{\fix}{\marginpar{FIX}}
% \newcommand{\new}{\marginpar{NEW}}


%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
\begin{document}


\maketitle

\begin{abstract}
% We present the first framework of \textbf{C}ertifying \textbf{Ro}bust Policies for general offline reinforcement learning~(RL) against \textbf{Po}isoning attacks~(\sysname).
% In general poisoning attacks, the attacker can arbitrarily insert, delete, or modify a bounded number of samples in the training set to corrupt the learned policy.
% % Against these attacks, our \sysname provides novel policy aggregation protocols and practically computable robustness certification of \emph{per-state action stability} and \emph{finite-horizon cumulative reward} for these novel protocols.
% \sysname aggregation protocols leverage the sequential nature of RL tasks, and thus apply not only training data partition aggregation but also \emph{temporal aggregation} to boost and tighten the certified robustness.
% \sysname provides novel certification methods for these aggregation protocols, since existing certification methods only support training data partitioning.\bo{what does this sentence mean?}
% For the certification of per-state action stability, we provide a novel and theoretically tight certification when the aggregation time window has a fixed length, and provide a\bo{not good} tight certification when the time window length is dynamically determined;
% for the certification of finite-horizon cumulative reward, we combine the action stability certification with an adaptive tree search algorithm.
% We further prove the computational hardness of certification problems.
% We evaluate \sysname extensively on two games~(Freeway and Breakout) with three offline RL training algorithms~(DQN, DR-DQN, C51).
% The experimental results show that: 
% (1)~The temporal aggregation in \sysname significantly boosts the certified robustness against poisoning comparing with only training data partition aggregation. \huan{some concrete numbers are better, for example ``improve certification rate by XX\% using temporal aggregation``}
% (2)~Our certification methods for both per-state action stability and finite-horizon cumulative reward are efficient and  tight.\bo{?}
% (3)~The certification patterns \huan{From the abstract it is unclear what is ``certification pattern''? maybe use another way to say it.} for different training algorithms and different games are different, implying different intrinsic robustness of them.

As reinforcement learning (RL) has achieved near human-level performance in a variety of tasks, its robustness has raised great attention.
% when applied to safety-critical domains such as autonomous driving.
While a vast body of research has explored test-time (evasion) attacks in RL and corresponding defenses, its robustness against training-time (poisoning) attacks remains largely unanswered.
% Recent studies have explored test-time attacks in RL and corresponding defenses, while the robustness of RL against training-time attacks remains largely unanswered.
In this work, we focus on \textit{certifying} the robustness of offline RL in the presence of poisoning attacks, where a subset of training trajectories could be \textit{arbitrarily} manipulated. We propose the \textit{first} certification framework, \sysname, to certify the number of poisoning trajectories that can be tolerated regarding different certification criteria. Given the complex structure of RL, we propose two  certification criteria: \emph{per-state action stability} and \emph{cumulative reward bound}.
To further improve the certification, we propose new partition and  aggregation protocols to train robust policies. 
We further prove that some of the proposed certification methods are  theoretically tight and some  are NP-Complete problems.
% In particular, for per-state action certification, we provide a novel and theoretically tight certification under fixed window aggregation, as well as a tight certification for the dynamic window aggregation.
% For the finite-horizon cumulative reward certification, we combine the action certification with an adaptive tree search algorithm to provide tight certification.
% We further prove that the theoretically tight cumulative reward certification is NP-Complete.
We leverage \sysname to certify three RL environments trained with different algorithms and conclude:
% (1)~The proposed temporal aggregation in \sysname significantly improves certified robustness for games with strong temporal continuity property {\eg, for Freeway;  on Breakout and Highway however, \rlalgo is better.}
(1)~The proposed robust aggregation protocols such as \textit{temporal aggregation} can significantly improve the certifications;
% (\ie, about \TODO\% higher for the number of tolerated poisoning trajectories) compared with vanilla partition aggregation algorithm;
(2)~Our certifications for both per-state action stability and  cumulative reward bound are efficient and tight;
(3)~The certification for different training algorithms and environments are different, implying their intrinsic robustness properties.
All experimental results are available at 
{\small{\url{https://copa-leaderboard.github.io}}}.
% \fan{conclusion for Highway: 1) similar to Breakout (and different from Freeway), \rlalgo is better than the algorithms with temporal aggregation. 2) C51 is able to certify larger poisoning size compared with DQN and QR-DQN.}


\end{abstract}

\vspace{-2mm}
\section{Introduction}
\label{sec:intro}
\vspace{-2mm}

Reinforcement learning~(RL) has been widely applied to a range of applications, including robotics~\citep{kober2013reinforcement,deisenroth2013survey,polydoros2017survey} and  autonomous  vehicles~\citep{shalev2016safe,sallab2017deep}.
In particular, offline RL~\citep{levine2020offline} is proposed to leverage previously observed data to train the policy without requiring expensive interaction with environments or online data collection, and enables the reuse of training data~\citep{agarwal2020optimistic}.
However, offline RL also raises a great safety concern on  poisoning attacks~\citep{kiourti2020trojdrl,wang2020stop,wang2021backdoorl}.
A recent survey of industry  reports that data poisoning is significantly more concerning than other threats~\citep{kumar2020adversarial}.
% In poisoning attacks, the attacker can manipulate the training data to either deteriorate the overall model performance~\citep{shafahi2018poison,zhu2019transferable}, or deviate the model behavior with inputs containing well-designed patterns~\citep{chen2017targeted,dai2019backdoor}).
% Such attacks are shown effective not only for classification~\citep{schwarzschild2021just}, but also for RL tasks~\citep{kiourti2020trojdrl,wang2020stop,wang2021backdoorl}.
For offline RL, the situation is even worse, and a recent theoretical study shows that the robust offline RL against poisoning attacks is a strictly harder problem than online RL~\citep{zhang2021corruption}.

\looseness=-1
Although there are several empirical and certified defenses for classification tasks against poisoning attacks~\citep{peri2020deep,levine2021deep,weber2020rab}, it is challenging and shown ineffective to directly apply them to RL given its complex structure~\citep{kiourti2020trojdrl}. Thus, robust offline RL against poisoning attacks remains largely unexplored with no mention of robustness certification. 
% For classification tasks, there exist both empirical defenses and certified defenses against poisoning attacks.
% The empirical defenses provide satisfactory robustness against existing attacks~\citep{peri2020deep} and provide robustness guarantees under some approximated assumptions~\citep{steinhardt2017certified}.
% The certified defenses provide rigorous and practically computable guarantees against arbitrary attacks as long as the attack size is bounded~\citep{levine2021deep,weber2020rab}. 
% However, for RL, the defenses against poisoning attacks are relatively unexplored.
% The existing defenses that are geared towards classification tasks are shown ineffetive in RL tasks~\citep{kiourti2020trojdrl}.
In addition, though some theoretical analyses provide general robustness bounds for RL, they either assume a bounded distance between the learned and Bellman optimal policies or are limited to linear MDPs~\citep{zhang2021corruption}. To the best of our knowledge, there is no robust RL method that is able to provide \emph{practically computable} \emph{certified robustness} against  poisoning attacks.
% \footnote{Some theoretical analyses provides robustness bounds either by assuming bounded distance between the learned policy and Bellman optimal policy or are limited to linear MDPs. Therefore, they do not directly lead to a practically computable robustness certification for general deep RL tasks.}
% This is a challenging problem due to the unique sequential nature of RL tasks and lack of certification criteria.
In this paper, we tackle this problem by proposing the first framework of \underline{C}ertifying r\underline{o}bust policies for general offline RL against  \underline{p}oisoning \underline{a}ttacks (\textbf{\sysname}).

% \paragraph{Threat Model: General Poisoning Attack.}
% % The general poisoning attack on the training data of offline RL tasks with a discrete action space and discrete time steps.
% % In this scenario,
% In poisoning attacks against offline RL, the training data contains a finite set of training trajectories, and the attacker is allowed to arbitrarily insert, remove, or modify a bounded number of such training trajectories.
% We call this bounded number as the \textit{poisoning size}.

% Formally, the attacker can arbitrarily change the training set from $D$ to $\wtilde D$, as long as the size of symmetric difference between $D$ and $\wtilde D$ is upper bounded by attack size $K \in \sN$.
% Note that modifying an individual data point causes the removal of original data point and the insertion of a new one, thus increasing the symmetric difference by $2$.
% This threat model  is commonly used  in classification tasks~\citep{levine2021deep} and closely related to the $\epsilon$-contamination model in robust statistics~\citep{diakonikolas2016robust}.
% Such a threat model is rather general in the sense that different adversarial goals can be achieved.

% with such flexible manipulations.

\textbf{Certification Criteria.}
One critical challenge in certifying robustness for offline RL is the certification criteria, since the prediction consistency is no longer the only goal as in classification.
We propose two criteria based on the properties of RL: \underline{per-state action stability} and \underline{cumulative} \underline{reward} \underline{bound}.
% For per-state action stability, suppose \sysname's policy chooses action $a_t$ at current time step $t$, \sysname can compute a lower bound $\wbar K$~(robust threshold), such that for arbitrarily attacks whose attack size $K \le \wbar K$, the policy after poisoning is guaranteed to still choose action $a_t$.
The former guarantees that at a specific time, the policy learned with \sysname will predict the same action before and after attacks under certain conditions.
This is important for guaranteeing the safety of the policy at critical states, \eg, braking when seeing pedestrians.
For  cumulative reward bound,  a lower bound of the cumulative reward for the policy learned with \sysname is guaranteed under certain poisoning conditions.
This directly guarantees the worst-case overall performance.
% of the policy under poisoning attacks satisfying certain constraints.

\textbf{\sysname Framework.}
\sysname is composed of two components:  policy partition and aggregation protocol and  robustness certification method.
We propose three policy partition aggregation protocols: \underline{\rlalgo}~(\rlalgofullname), \underline{\rlalgotmp}~(\rlalgotmpfullname), and \underline{\rlalgodyntmp}~(\rlalgodyntmpfullname), and propose certification methods for each of them corresponding to both proposed certification criteria.
% {\rlalgo} 
% divides the training data into $u$ parts following certain protocol and independently train $u$ subpolicies.
% During inference, at each state, the action with the highest votes across these subpolicies is chosen as the final action.
% However, \rlalgo does not leverage the unique temporal continuity nature of RL.
% % Indeed, in common RL tasks, the chosen actions usually do not differ too much among adjacent steps.
% To better leverage the temporal continuity of RL, we propose {\rlalgotmp} with a predetermined time window size $W$, and count the highest action votes for all the recent $W$ states as the action for the current state.
% As a result, if the votes of the top two actions are too similar in \rlalgo, we can aggregate votes from other recent states to enlarge the margin and thus ensure high certified robustness.
% Taking a step further, in {\rlalgodyntmp}, we propose to dynamically optimize the time window size $W$.
% and heuristically achieve high certified robustness accordingly.
% We propose novel certification methods for each aggregation protocol under different certification criteria. 
In addition, for \textit{per-state action stability}, we prove that our certifications for \rlalgo and \rlalgotmp are theoretically tight.
% the tight tolerable threshold of poisoning size $\wbar K$ for \rlalgo can be derived based on existing work for classification tasks~\citep[Theorem 1]{levine2021deep}.
% For policies trained with \rlalgotmp which will potentially achieve a tighter certification bound, the challenge is to carefully figure out the marginal gain of the optimal attack on each subpolicy considering action flipping.
% To this end, we propose a novel greedy algorithm that yields a theoretically tight and efficiently computable certification.
% In contrast, the na\"ive extension of Theorem~1 in \citep{levine2021deep} yields suboptimal certification.
% For \rlalgodyntmp, the problem is even more involved, where the poisoning attack may also shift the dynamic window size and thus flip the chosen action.
% We provide a nontrivial algorithm that enumerates the optimal attacks on each subpolicy considering both the changing window size and action flipping combined with certain relaxation.
For \textit{cumulative reward bound}, we propose an adaptive search algorithm, where we compute the possible action set for each state under certain poisoning conditions.
Concretely, we propose a novel method to compute the precise action set for \rlalgo and efficient algorithms to compute a superset of the possible action set which leads to sound certification for \rlalgotmp and \rlalgodyntmp.
We further prove that
for \rlalgo our certification is theoretically tight, 
for \rlalgotmp the theoretically tight certification is $\NP$-complete, 
and for \rlalgodyntmp it is open whether theoretically tight certification exists.
% For \rlalgotmp, we further prove the $\NP$-completeness of computing the precise possible action set. 
% We also prove the general $\NP$-completeness of cumulative reward certification.

% We evaluate \sysname thoroughly on two different games with three offline RL training algorithms~(DQN, DR-DQN, C51).
% The experimental results show that: 
% (1)~The proposed temporal aggregation protocol in \sysname,  significantly boosts the certified robustness;
% (2)~Our certification methods are efficient and tight;
% (3)~The certification for different training algorithms and games are different, implying their intrinsic robustness properties.

\underline{\textbf{Technical Contributions.}} We take the first step towards certifying the robustness of offline RL against poisoning attacks, and we make contributions on both theoretical  and practical fronts.
% summarize our main technical contributions as follows:
\begin{itemize}[leftmargin=*,noitemsep]
    \item We abstract and formulate the robustness certification for offline RL against poisoning attacks, and we propose two certification criteria: per-state action stability and cumulative reward bound.
    
    \looseness=-1
    \item We propose the first framework \sysname for certifying robustness of offline RL against  poisoning attacks.
    \sysname includes novel policy aggregation protocols and  certification methods.
   
   \item We prove the tightness of the proposed certification methods for the aggregation protocol \rlalgo.
    We also prove the computational hardness of the certification for \rlalgotmp.
    
    \item We conduct thorough experimental evaluation for \sysname on different RL environments with three offline RL algorithms, demonstrating the effectiveness of \sysname,
    % aggregation protocols and certification methods in terms of boosting the certified robustness~(\ie, \TODO\% higher for the number of tolerated poisoning trajectories) 
    together with several interesting findings.
\end{itemize}
% Finally, we also provide several future directions from both the theoretical front and practical perspectives as discussed in \Cref{subsec:cert-reward}.\linyi{maybe remove this sentence? we don't discuss practical open problems there, and we lack the space a bit}
% , \eg, whether a tighter certification method for \rlalgodyntmp exists or certification for \rlalgodyntmp is $\NP$-complete; and whether better partitioning and training mechanisms exist.

% \vspace{-1mm}
% \section{Preliminaries and Notations}
%     \label{sec:prelim-threat-model}
%     \vspace{-1mm}
%     We introduce the preliminaries and notations in this section.

\vspace{-2mm}
\section{Related Work}
\vspace{-2mm}

\looseness=-1
Poisoning attacks~\citep{nelson2008exploiting,diakonikolas2016robust} are critical threats in machine learning, which are claimed to be more concerning than other threats~\citep{kumar2020adversarial}.
Poisoning attacks
% , including triggerless and backdoor attacks, 
widely exist in classification~\citep{schwarzschild2021just}, and 
both empirical defenses~\citep{liu2018fine,chacon2019deep,peri2020deep,steinhardt2017certified} and certified defenses~\citep{weber2020rab,jia2020certified,levine2021deep} have been proposed.
{\color{blue}

}
% Our work is inspired by the aggregation and randomized smoothing methodologies in classification, but we tackle unique RL challenges by providing novel action aggregation protocols and certification criteria and methods.

\looseness=-1
% The poisoning attack and its defenses in RL are relatively unexplored. 
After \citet{kiourti2020trojdrl} show the existence of effective backdoor poisoning attacks in RL,
% From the attack side, \citet{kiourti2020trojdrl} show that effective poisoning attacks, in particular backdoor attacks, exist in RL.
a recent work theoretically and empirically validates the existence of reward poisoning in online RL~\citep{zhang2020adaptive}.
Furthermore, \citet{zhang2021corruption} theoretically prove that the offline RL is more difficult to be robustified against poisoning than online RL considering linear MDP.
From the defense side, 
% based on online learning theory, 
\citet{zhang2021corruption} propose robust variants of the Least-Square Value Iteration algorithm that provides probabilistic robustness guarantees under linear MDP assumption.
In addition, Robust RL against reward poisoning is studied in~\citet{banihashem2021defense}, but robust RL against general poisoning is less explored.
In this background, we aim to provide the certified robustness for general offline RL algorithms against  poisoning attacks, which is the first work that achieves the goal.
% our work is based on robust aggregation, and is the first framework that is able to provide computable deterministic robustness certification for offline RL to the best of our knowledge.
{\color{black} We discuss broader related work in \Cref{adxsec:related-works}.}



\vspace{-2mm}
\section{Certification Criteria of \sysname}
\label{sec:criteria}
\vspace{-2mm}

    In this section, we propose two robustness certification criteria for offline RL against general poisoning attacks: per-state action stability and cumulative reward bound.

    % \subsection{Preliminaries and Notations}
        \label{subsec:prelim}
        \label{subsec:notation}
        
        \paragraph{Offline RL.}
        We model the RL environment by an episodic finite-horizon Markov decision process~(MDP) $\gE = (\gS, \gA, R, P, H, d_0)$, where $\gS$ is the set of states, $\gA$ is the set of discrete actions, $R: \gS \times \gA \to \sR$ is the reward function,  $P: \gS \times \gA \to \gP(\gS)$ is the stochastic transition function with $\gP(\cdot)$ defining the set of probability measures, $H$ is the time horizon, and $d_0 \in \gP(\gS)$ is the distribution of the initial state.
        At time step $t$, the RL agent is at state $s_t \in \gS$. 
        After choosing action $a_t \in \gA$, the agent transitions to the next state $s_{t+1} \sim P(s_t,a_t)$ and receives reward $r_t = R(s_t, a_t)$.
        After $H$ time steps, the cumulative reward $J = \sum_{t=0}^{H-1} r_t$.
        We denote a consecutive sequence of all states between time step $l$ and $r$ as $s_{l:r} := [s_l, s_{l+1}, \dots, s_r]$.
        
        % \paragraph{Offline RL.}
        Here we focus on offline RL, for which the threat of poisoning attacks is practical and more challenging to deal with~\citep{zhang2021corruption}.
        % where the agent learns the policy without interacting with the environment or simulator but just uses a fixed dataset of trajectories to learn the policy.
        % Thus, offline RL saves the huge cost of collecting vast amounts of data from scratch during training for complex real world problems~\tocite.
        Concretely, in offline RL, a training dataset $D = \{\tau_i\}_{i=1}^{N}$ consists of logged trajectories, where each trajectory $\tau=\{(s_{j},r_{j},a_j, s'_j)\}_{j=1}^{l} \in (\gS \times \gA \times \sR \times \gS)^l$ consists of multiple tuples denoting the transitions (\ie, starting from state $s_j$, taking the action $a_j$, receiving reward $r_j$, and transitioning to the next state $s_j'$).
        
        % \paragraph{Subpolicy and Aggregated Policy in \sysname.}
        % We call each learned policy in offline RL \emph{subpolicy} and represent it by $\pi_i = \gM_i(D_i): \gS \to \gA, 0\le i< u$, where $u$ is the number of subpolicies, and $\gM_i$ is the RL training algorithm that learns $\pi_i$ from training dataset $D_i$.
        % % Such dependency may be omitted when there is no ambiguity.
        % As we will introduce in \Cref{subsec:training-protocol}, the subpolicy $\pi_i$'s training dataset $D_i$ is a subset of the whole set $D$.
        % Note that we do not make any  assumption on the learning algorithms or the gap between learned and optimal policies.
        % % We only need a deterministic function from $\gS$ to $\gA$, that is determined by the training dataset. 
        
        % We define $[u] := \{0,1,\dots,u-1\}$.
        % The \emph{policy indicator} $\1_{i,a}: \gS \to \{0,1\}$ is defined by $\1_{i,a}(s) := \1[\pi_i(s) = a]$, which indicates whether the subpolicy $\pi_i$ chooses action $a$ given current state $s$.
        % The \emph{aggregated action count} $n_a: \gS \to \sN_{\ge 0}$ is the number of votes across all trained $u$ subpolicies for action $a$ given current state $s$:
        % $
        %     n_a(s) := | \{i \, \mid \, \pi_i(s) = a, i \in [u] \} | = \sum_{i=0}^{u-1} \1_{i,a}(s).
        % $
        % Specifically, we denote $n_a(s_{l:r})$ for $\sum_{j=l}^r n_a(s_j)$, \ie, the sum of votes for all states between time step $l$ and $r$.
        % {\color{blue} Besides subpolicies, we will introduce aggregation protocols that produce \emph{aggregated policies} in \Cref{sec:main}.}
        
        % Besides subpolicies, we propose different aggregation protocols that produce \emph{aggregated policies}.
        % % $\rlalgopolicy$, $\rlalgotmppolicy$, and $\rlalgodyntmppolicy$  (\Cref{sec:main}).
        % % We will focus on robustness certification for these aggregated policies.
        % % These aggregated policy is based on subpolicies' action choices for the current state or recent several states.
        % The action of such an aggregated policy is calculated based on the prediction of different subpolicies given current and several recent states. How to decide the aggregation length of the states depends on the proposed aggregation protocols (details in \Cref{sec:main}).
        % Formally, an aggregated policy can be written as a function $\pi_\star: \gS^\star \to \gA$, where $\gS^\star$ is a sequence of states, and we focus on providing robustness certification for these aggregated policies. \bo{shorten and move this to sec 3, we can merge with sec 3 to save space}
        % % When there is no ambiguity, we may omit the dependency on $\{\pi_i\}_{i=1}^u$.
        
        % \paragraph{Notations.}
        
    % \paragraph{Threat Model: Poisoning Attacks.}
    %     \label{subsec:threat-model}
    %     We consider the general poisoning attack as the threat model, where the entries in the training dataset can be arbitrarily modified by the adversary as long as the number of modified entries is bounded. 
        % The threat model is general in the sense that poisoning attacks and backdoor attacks, although for different goals, both change only training data points.
        % This setting is well known as the \textit{data poisoning attack} in the literature of adversarial attacks in classification tasks~\citep{nelson2008exploiting}. It is also closely related to the \textit{$\eps$-contamination model} in the robust statistics literature~\citep{diakonikolas2016robust}.
        % 
        
        % Recall that in offline RL, a dataset 
        % % %$D=\{(s_i, a_i, r_i, s_i')\}_{i=1}^{N} \in (\cal S \times \cal A \times \bb R \times \cal S)^N$ 
        % $D$
        % containing logged trajectories is used for training an RL agent.
        % The dataset $D$ can be poisoned in the following manner. 
        % For each trajectory $\tau\in D$, the adversary is allowed to replace it with an arbitrary trajectory $\tilde\tau$, and then the poisoning  dataset $\wtilde D$ is revealed to the learner. 
        % We denote $D \ominus \wtilde D = (D \backslash \wtilde D) \bigcup (\wtilde D \backslash D)$ as the \textit{symmetric difference} between  two datasets $D$ and $\wtilde D$.
        % For instance, adding or removing one trajectory causes a symmetric difference of magnitude $1$, while replacing one trajectory with a new one leads to a symmetric difference of magnitude $2$.
        % We refer to the size of the symmetric difference as the \textit{poisoning size}, and we will provide robustness certification given the upper bound of the poisoning size.
        % constrain the attacker's ability by setting an upper bound for the poisoning size. 
        %For example, in the $\eps$-contamination model, the attack magnitude is restricted to be no larger than $\eps N$.

% \vspace{-1mm}
% \section{Certification Criteria of \sysname}
% \label{sec:criteria}
% \vspace{-1mm}

%     In this section, we propose two robustness certification criteria for offline RL against general poisoning attacks: per-state action stability and finite-horizon cumulative reward.

  \textbf{Poisoning Attacks.}\quad 
% In offline RL, a dataset 
%         % %$D=\{(s_i, a_i, r_i, s_i')\}_{i=1}^{N} \in (\cal S \times \cal A \times \bb R \times \cal S)^N$ 
%         $D$
%         containing logged trajectories is used for training an RL agent.
        Training dataset $D$ can be poisoned in the following manner. 
        For each trajectory $\tau\in D$, the adversary is allowed to replace it with an arbitrary trajectory $\wtilde\tau$, generating a manipulated  dataset $\wtilde D$. 
        We denote $D \ominus \wtilde D = (D \backslash \wtilde D) \bigcup (\wtilde D \backslash D)$ as the \textit{symmetric difference} between  two datasets $D$ and $\wtilde D$.
        For instance, adding or removing one trajectory causes a symmetric difference of magnitude $1$, while replacing one trajectory with a new one leads to a symmetric difference of magnitude $2$.
        We refer to the size of the symmetric difference as the \textit{poisoning size}.
        
   \textbf{Certification Goal.}\quad
   To provide the robustness certification  against poisoning attacks introduced above, 
    we aim to certify the \textit{test-time} performance of the trained policy in a clean environment.
    Specifically,
    in the \textit{training phase},  the RL training algorithm and our aggregation protocol can be jointly modeled by $\cal M:\cal D\rightarrow (\gS^\star \to \gA)$ which provides an aggregated policy,
    where $\gS^\star$ denotes the set of all consecutive state sequences.
    Our \textbf{goal} is to provide robustness certification for the poisoned aggregated policy $\tpi = \gM(\wtilde D)$, given bounded poisoning size (\ie, $|D \ominus \wtilde D| \leq \wbar{K}$).
    % Here $\wtilde D$ is the poisoning data based on original~(\ie, clean) dataset $D$.
    
    
    % After the training is finished, in the \textbf{testing phase}, we deploy the poisoned policy $\tpi$ in a clean environment to evaluate its actual performance.
    % , and obtain the robustness certification under different criteria.
    %Note that when we certify the trained/learned policy $\tpi$, our certification is based on the \textit{test-time performance} of $\tpi$ after the training is done.
    % Concretely, 
    % we propose two criteria: \textit{per-state action stability} and \textit{lower bound of the cumulative reward}; we introduce the details below.
    
    \paragraph{Robustness Certification Criteria: Per-State Action Stability.}
    We first aim to certify the robustness of the poisoned policy in terms of the stability of per-state action during test time.
    
    \begin{definition}[Robustness Certification for Per-State Action Stability]
    	\label{def:per-state}
    	Given a clean dataset $D$, 
    	we define the robustness certification for \textit{per-state action stability} as that for \textit{any} $\wtilde D$ satisfying $| D\ominus \wtilde D | \leq \wbar K$, 
    	the {action} predictions of the poisoned  and  clean policies for the state~(or state sequence) $s$ are the same, \ie, $\tpi = \gM(\wtilde D), \pi = \gM(D), \tpi(s) = \pi(s)$, under the
    	the tolerable {poisoning threshold}  $\wbar K$.
    % 	{\color{blue}
    	In an episode, we denote the tolerable poisoning threshold for the state at step $t$ by $\wbar K_t$.
    % 	}
    % 	, 
    % 	such that for \textit{any} $\wtilde D$ that satisfies $| D\ominus \wtilde D | \leq \wbar K$, 
    % 	the \textit{action} predictions of the poisoned  and  clean policies for the state~(or state sequence) $s$ are the same (action stability), \ie, $\tpi = \gM(\wtilde D), \pi = \gM(D), \tpi(s) = \pi(s)$.
    % 	
    % 	\textit{state} $s$ during test time
    	
    % 	, given by the poisoned policy $\tpi=\cal M(\wtilde D)$, will be the same as the action prediction given by the clean policy $\pi=\cal M(D)$, \ie, $\pi(s)=\tpi(s)$.
    \end{definition}
    
    \looseness=-1
    The definition encodes the requirement that, for a particular state, any poisoned policy will always give the same action prediction as the clean one, as long as the poisoning size is within $\wbar K$~($\wbar K$ computed in \Cref{sec:main}).
    % The $\wbar K$ is the certification that we need to compute.
    In this definition, $s$ could be either a state or a state sequence, 
    since our aggregated policy~(defined in \Cref{subsec:prelim}) may aggregate multiple recent states to make an action choice.
    % In practice, we compute $\wbar K_t$ at each step $t$ in an episode.
    
    \paragraph{Robustness Certification Criteria: Lower Bound of Cumulative Reward.}
    We also aim to certify poisoned policy's overall performance in addition to the prediction at a particular state.
    Here we measure the overall performance by the cumulative reward $J(\pi)$~(formally defined in \Cref{adxsec:protocol}).
    
    % \begin{definition}[Cumulative Reward]
    %     \label{def:cum-reward}
    %     Let $P: \cal S \times \cal A \rightarrow \cal P(\cal S)$ be the transition function  with $\cal P(\cdot)$ defining the set of probability measures.  
    %     % Let $\Gamma:\cal S\times \cal A\rightarrow \cal S$ be the transition function, 
    %     Let $R,d_0,H$ be the reward function, initial state distribution, and time horizon.
    %     % Suppose each state trajectory contains at most $H$ time steps, and 
    %     We denote $J(\pi)$  as the \emph{cumulative reward} of the given policy $\pi$:
    %     \begin{small}
    %     \begin{equation}
    %         \label{eq:cum-reward}
    %         J(\pi)  := \E \sum_{t=0}^{H-1} R(s_t, a_t),
    %         \text{ where } a_t=\pi(s_t),s_{t+1}\sim P(s_t,a_t),s_0\sim d_0,
    %     \end{equation}
    %     \end{small}
    % \end{definition}

    % % The definition sums up the reward across all $H$ steps to get the cumulative reward.
    % It is natural to adapt this definition when there is a discount factor.
    % If policy $\pi$ considers recent $n_t$ states instead of only $s_t$ to make action predictions, we can change $a_t = \pi(s_t)$ to $a_t = \pi(s_{t-n_t+1 : t})$ in \Cref{eq:cum-reward}.
    Now we are ready to define the robustness certification for cumulative reward bound.
    \begin{definition}[Robustness Certification for Cumulative Reward Bound]
    	\label{def:cert-cum-reward}
    	\looseness=-1
    	Robustness certification for cumulative reward bound 
    % 	\bo{Defined in Appendix xxxx, move def 2 to appendix}\linyi{moved} 
    	is the \emph{lower bound} of \textit{\namecr} $\uj_K$ such that $\uj_K \leq J(\tpi)$ for any $\tpi = \cal M (\wtilde D)$ where $|D \ominus \wtilde D| \le K$, \ie, $\tpi$ is trained on poisoned dataset $\wtilde D$ within poisoning size $K$.
    \end{definition}


% \section{Preliminaries}
% \label{sec:prelim}


% % In this section we will provide
% % background on Q-learning and randomized smoothing.
% % , and then establish the connections between them to show how to provide probabilistic robustness certification for deep Q-Networks via smoothing.

% \looseness=-1 \textbf{Q-learning and Deep Q-Networks (DQNs).}\quad
% %In this paper, we focus on 
% Markov decision processes (MDPs) are at the core of RL.
% Our focus is on discounted discrete-time MDPs, which are defined by tuple $(\cal S,\cal A, R,P,\gamma, d_0)$, 
% where $\cal S$ is a set of states (each with dimensionality $N$), 
% $\cal A$ represents a set of discrete actions, 
% $R:\cal S\times \cal A\rightarrow\bb R$ is the reward function, 
% and $P: \cal S\times \cal A \rightarrow \cal P(\cal S)$ is the transition function with $\cal P(\cdot)$ defining the set of probability measures,
% % Concretely, the transition probability
% % $p(s'|s,a) = \Pr\left[s_{t+1}=s'\mid s_t = s,a_t=a\right]$.
% $\gamma \in [0,1]$ is the discount factor, 
% and $d_0 \in \cal P(\cal S)$ is the distribution over the initial state. 
% At time step $t$, the agent is in the state $s_t \in \cal S$. After choosing action $a_t \in \cal A$, the agent transitions to the next state $s_{t+1}\sim P(s_t,a_t)$ and receives reward $r_t = R(s_t,a_t)$. The goal is to learn a policy $\pi:\cal S\rightarrow \cal P(\cal A)$ that maximizes the expected cumulative reward $\mathbb{E}[\sum\nolimits_t \gamma^t r_t]$.
% % , where the expectation is with respect to the randomness in the environment dynamics and policy.

% \iffalse
% Q-learning~\citep{watkins1992q} learns an action-value function (Q-function), $Q^\star(s,a)$, which is
% %is a value-based learning approach that aims to optimize a policy to maximize the expected value of the total reward over all successive steps, starting from the current state.
% %% estimate the value of taking any action at any given state. 
% %The optimal action-value function $Q^\star(s,a)$ is defined to be 
% the maximum expected cumulative reward  the agent can achieve after taking action $a$ in state $s$:
% %achievable by any strategy after seeing the state $s$ and taking the action $a$, 
% % and the optimal policy $\pi^\star$ is the greedy policy 
% % and the induced policy $\pi$ are

% % \begin{small}
% % \begin{align*}
%     $Q^\star(s,a) = R(s,a) + \gamma \underset{s'\sim P(s,a)}{\bb E}\left[\max_{a'} Q^\star (s',a') \right]$.
% % \end{align*} 
% % \end{small}
% The (optimal) policy is defined as taking the best action in each state determined by the Q-function:
% $
% \pi(s) = \arg\max_{a \in \cal A} Q^\star(s,a)
% $.
% In deep Q-Networks (DQNs)~\citep{mnih2013playing},  $Q^\star$ is approximated using a neural network parametrized by $\theta$, \ie, $Q(s,a;\theta) \approx Q^\star(s,a)$.
% Let $\rho:\cal S\times \cal A\rightarrow \bb R$ be the  distribution defined over states $s$ and actions $a$, the network can be trained by minimizing the loss function 
% % \begin{small}
% % \begin{align*}
%     $\cal L(\theta) = \underset{(s,a)\sim \rho,s'\sim P(s,a)}{\bb E}\left[ \left(R(s,a)+\gamma \max _{a^{\prime}} Q\left(s^{\prime}, a^{\prime} ; \theta\right)-Q(s, a ; \theta)\right)^{2}\right].$
% % \end{align*}
% % \end{small}
% \fi


% Q-learning~\citep{watkins1992q} learns an action-value function (Q-function), $Q^\star(s,a)$, which is 
% the maximum expected cumulative reward  the agent can achieve after taking action $a$ in state $s$:
%     $Q^\star(s,a) = R(s,a) + \gamma \underset{s'\sim P(s,a)}{\bb E}\left[\max_{a'} Q^\star (s',a') \right]$.
% % The (optimal) policy is defined as taking the best action in each state determined by the Q-function:
% % $
% % \pi(s) = \arg\max_{a \in \cal A} Q^\star(s,a)
% % $.
% In deep Q-Networks (DQNs)~\citep{mnih2013playing},  $Q^\star$ is approximated using a neural network parametrized by $\theta$, \ie, $Q^\pi(s,a;\theta) \approx Q^\star(s,a)$.
% Let $\rho\in\cal P(\cal S \times \cal A)$ be the observed distribution defined over states $s$ and actions $a$, the network can be trained via minimizing loss function 
%     $\cal L(\theta) = \underset{(s,a)\sim \rho,s'\sim P(s,a)}{\bb E}\left[ \left(R(s,a)+\gamma \max _{a^{\prime}} Q^\pi\left(s^{\prime}, a^{\prime} ; \theta\right)-Q^\pi(s, a ; \theta)\right)^{2}\right].$
% The greedy policy $\pi$ is defined as taking the action with highest $Q^\pi$ value in each state $s$: $\pi(s) = \arg\max_{a\in \cal A} Q^\pi(s,a)$.



% \textbf{Offline RL.}\quad
% Modern RL algorithms are mostly ``online'' where the agent learns the policy as it interacts with the environment or simulator. 
% However, actively collecting vast amounts of data from scratch for each experiment via the interactions can be forbiddingly expensive in complex real world problems. This calls for the arise of ``offline'' RL which learns from a fixed dataset of \textit{trajectories}.
% Concretely, an offline RL dataset 
% $D = \{\tau_i\}_{i=1}^{N}$ is consisted of logged trajectories, where each trajectory $\tau=\{(s_{j},r_{j},a_j, s'_j)\}_{j=1}^{l} \in (\cal S \times \cal A \times \bb R \times \cal S)^l$ is consisted of multiple tuples denoting the transitions (starting from the state $s_j$, taking the action $a_j$, receiving the reward $r_j$, and transitioning to the next state $s_j'$).


% %Concretely, an offline RL dataset 
% %$D=\{(s_i, a_i, r_i, s_i')\}_{i=1}^{N} \in (\cal S \times \cal A \times \bb R \times \cal S)^N$
% %is consisted of logged tuples of transitions, where each tuple denotes a transition that starts from the state $s$, and achieves reward $r$ and transitions to the next state $s'$ upon taking the action $a$. 
% %For ease of notation, we denote such a transition as $\mathbf{t}\in D$.

% \fan{TODO: add preliminaries for rand smooth for poisoning and the DPA framework}

% \textbf{Certified Robustness for Classifiers via Randomized Smoothing.}\quad
%     Randomized smoothing~\citep{cohen2019certified} has been proposed to provide probabilistic certified robustness for  classification models.
%     It achieves the state-of-the-art certified robustness on large-scale datasets such as ImageNet under $\ell_2$-bounded constraints~\citep{salman2019provably,yang2020randomized}.
%     % achieved the state-of-the-art certified robustness on large ImageNet and CIFAR-10 dataset under $L_2$ norm.
%     % For a single ML model, to obtain robust certification for large radius classifier it needs to predict correctly with high probability even when the input is corrupted by random noise.
%     % Several approaches have further improved it by:
%     % (1)~choosing different smoothing distributions for different $L_p$ norms~\citepp{dvijotham2019framework,zhang2020black,yang2020randomized},
%     % and (2)~training more robust smoothed classifiers, using data augmentation~\citepp{cohen2019certified}, unlabeled data~\citepp{carmon2019unlabeled}, adversarial training~\citepp{salman2019provably}, regularization~\citepp{li2019certified,zhai2019macer}, and denoising~\citepp{salman2020black}.
%     %     However, within our knowledge, there is no work studying how to customize randomized smoothing for RL.
%     In particular, given a base model and a test instance, a smoothed model will be constructed by outputting the most probable prediction over different Gaussian perturbed inputs.
%     % Formally, 
%     % let $\delta \sim \gN(0, \sigma^2 I)$ be a random noise drawn from the Gaussian distribution,
%     % the smoothed classifier would predict 
%     % \begin{small}
%     % $$\wtilde F(x) = \argmax_{c\in\cal C} \Pr_{\delta \sim \gN(0, \sigma^2 I)} (F(x + \delta) = c)$$
%     % \end{small}where $F: \sR^d \to \{1,\dots,|\cal C|\}$ denotes the base classification model with the class set $\cal C$.
%     % % Intuitively, the confidence score for each class is given by the probability of predicting that class under noised inputs.
%     % In this paper, we will focus on how to leverage different smoothing strategies at local and global levels to smooth a given policy and provide the certified robustness for Q-learning based on different criteria.





% \section{Robustness Certification for Robustness against Poisoning in Q-learning}

% In this section, we first introduce the threat model in terms of poisoning attacks in offline RL. We then present two criteria for certifying robustness against this threat model.

% \subsection{Threat Model}

% We consider the threat model where the entries in the training dataset can be modified by the adversary. This setting is well known as the \textit{data poisoning attack} in the literature of adversarial attacks in classification tasks~\citep{nelson2008exploiting}. It is also closely related to the \textit{$\eps$-contamination model} in the robust statistics literature~\citep{diakonikolas2016robust}.

% Concretely, in the offline RL setting, a dataset 
% %$D=\{(s_i, a_i, r_i, s_i')\}_{i=1}^{N} \in (\cal S \times \cal A \times \bb R \times \cal S)^N$ 
% $D$
% containing existing logged trajectories is available for training an RL agent.
% The dataset $D$ can be poisoned in the following manner. 
% For each trajectory $\tau\in D$, the adversary is allowed to replace it with an arbitrary trajectory $\tilde\tau$.
% After the replacements, the newly obtained dataset $\wtilde D$ is revealed to the learner. 
% We denote $D \ominus \wtilde D = (D \backslash \wtilde D) \bigcup (\wtilde D \backslash D)$ as the \textit{symmetric difference} between the two datasets $D$ and $\wtilde D$.
% For example, adding or removing one trajectory causes a symmetric difference of magnitude $1$, while replacing one trajectory with a new one leads to a symmetric difference of magnitude $2$.
% We refer to the size of the symmetric difference as the \textit{poison size}. 
% %For example, in the $\eps$-contamination model, the attack magnitude is restricted to be no larger than $\eps N$.

% \subsection{Different Criteria for Certifying Robustness against Poisoning}

% To provide the certification for robustness against the poisoning attack as introduced above, 
% we aim to certify the \textit{test-time} performance of the policy learned on the poisoned \textit{training} dataset.
% Specifically, we separate the description into two phases: \textbf{training phase} and \textbf{testing phase}.
% In the \textbf{training phase}, let the RL training algorithm be $\cal M:\cal D\rightarrow \Pi$ which operates on the given dataset and outputs a policy, our goal is to provide certification for the learned policy $\tpi = \cal M(\wtilde D)$, where $\wtilde D$ is obtained as a result of poisoning the clean dataset $D$.
% After the training is finished, in the \textbf{testing phase}, we deploy the trained/learned policy $\tpi$ in a clean environment, and obtain the robustness certification under different criteria.
% %Note that when we certify the trained/learned policy $\tpi$, our certification is based on the \textit{test-time performance} of $\tpi$ after the training is done.
% Concretely, 
% we propose two criteria: \textit{per-state action stability} and \textit{lower bound of the cumulative reward}; we introduce the details below.

% \textbf{Robustness certification for Per-State Action.}\quad
% We first aim to explore the robustness of the trained model in terms of the stability of per-state action during test time, assuming the training is conducted on a poisoned dataset.

% \begin{definition}[Certification for per-state action]
% 	\label{def:per-state}
% 	Given a clean dataset $D$, we define the robustness certification for per-state action as the \textit{robust poison threshold} $\wbar K$, such that for \textit{any} $\wtilde D$ that satisfies $| D\ominus \wtilde D | \leq \wbar K$, the \textit{action} prediction at an encountered \textit{state} $s$ during test time, given by the poisoned policy $\tpi=\cal M(\wtilde D)$, will be the same as the action prediction given by the clean policy $\pi=\cal M(D)$, \ie, $\pi(s)=\tpi(s)$.
% \end{definition}

% \textbf{Robustness certification for Cumulative Reward.}\quad
% In addition to the robustness certification in terms of the per-state action stability, we also define the robustness certification regarding the cumulative reward under the same threat model.

%     \begin{definition}[Cumulative reward]
%     \label{def:cum-reward}
%     Let $P: \cal S \times \cal A \rightarrow \cal P(\cal S)$ be the transition function of the environment with $\cal P(\cdot)$ defining the set of probability measures.  
%     % Let $\Gamma:\cal S\times \cal A\rightarrow \cal S$ be the transition function, 
%     Let $R,d_0,\gamma$ be the reward function, initial state distribution, and discount factor as introduced in~\Cref{sec:prelim}.
%     % Suppose each state trajectory contains at most $H$ time steps, and 
%     We denote $J(\pi)$  as the \emph{cumulative reward} corresponding to the given policy $\pi$: 

% %    \begin{small}
%     \begin{align}
%     J(\pi)  := \sum_{t=0}^{\infty} \gamma^t R(s_t, \pi(s_t)),
%     \text{ where }s_{t+1}\sim P(s_t,a_t),s_0\sim d_0,
%     \end{align}
% %    \end{small}
%     \end{definition}
    

% \begin{definition}[Robustness Certification for cumulative reward]
% 	\label{def:cert-cum-reward}
% 	The robustness certification for cumulative reward is the \emph{lower bound} of \textit{\namecr} $\uj_K$ such that $\uj_K \leq J({\wtilde \pi})$ for any $\tpi = \cal M (\wtilde D)$ learned on the poisoned dataset $\wtilde D$ under poison threshold $K$.
% \end{definition}

\vspace{-2mm}
\section{Certification Process of \sysname}
    \label{sec:main}
\vspace{-1mm}
    In this section, we introduce our framework \sysname, which is composed of \emph{training protocols}, \emph{aggregation protocols}, and \emph{certification methods}.
    The training protocol combined with an offline RL training algorithm provides subpolicies.
    The aggregation protocol aggregates the subpolicies  as an aggregated policy.
   The certification method certifies the robustness of the aggregated policy against poisoning attacks corresponding to different certification criteria provided in Section~\ref{sec:criteria}.
    
    % In \Cref{subsec:training-protocol}, we introduce the shared partition training protocol in \sysname;
    % in \Cref{subsec:agg-protocol}, we propose three aggregation protocols: \rlalgo, \rlalgotmp, and \rlalgodyntmp respectively;
    % in \Cref{subsec:cert-radius}, we introduce methods for certifying per-state action for aggregated policies;
    % and in \Cref{subsec:cert-reward}, we introduce methods for certifying cumulative reward for aggregated policies.
    % in \Cref{subsec:discussion}, we summarize.

\textbf{Overview of Theoretical Results.}\quad
    In \Cref{table:theory-overview}, we present an overview of our theoretical results: For each proposed aggregation protocol and certification criteria, we provide the corresponding certification method and core theorems, and we also provide the tightness analysis for each certification.
    % In addition, we prove the $\NP$-completeness of tight cumulative reward certification (\Cref{thm:general-hardness-reward}).

    \begin{table}[t]
        \centering 
        \caption{\small Overview of theoretical results in \Cref{sec:main}. ``Certification'' columns entail our certification theorems. ``Analysis'' columns entail the analyses of our certification bounds, where ``tight'' means our certification is theoretically tight, ``$\NP$-complete'' means the tight certification problem is $\NP$-complete, and ``open'' means the tight certification problem is still open.
        \Cref{thm:ppa-radius,prop:ppa-radius-tightness,thm:compare-tight-loose-action-set-ppa} are in \Cref{adxsec:ppa-per-state,adxsubsec:proof-C62}.
        }
        \label{table:theory-overview}
        \vspace{-2mm}
        \resizebox{0.95\textwidth}{!}{
        \begin{tabular}{c|cc|cc|cc}
            \toprule
            \multirow{3}{*}{\shortstack{Certification \\ Criteria}} & \multicolumn{6}{c}{Proposed Aggregation Protocol} \\
            \cline{2-7}\\[-1.5ex]
             & \multicolumn{2}{c|}{\rlalgo~($\rlalgopolicy$, \Cref{def:ppa-agg})} & \multicolumn{2}{c|}{\rlalgotmp~($\rlalgotmppolicy$, \Cref{def:tpa-agg})} & \multicolumn{2}{c}{\rlalgodyntmp~($\rlalgodyntmppolicy$, \Cref{def:dtpa-agg})} \\
             & Certification & Analysis & Certification & Analysis & Certification & Analysis \\
            \midrule
            Per-State Action & \Cref{thm:ppa-radius} & tight~(\Cref{prop:ppa-radius-tightness}) & \Cref{thm:tpa-radius} & tight~(\Cref{prop:tpa-radius-tightness}) & \Cref{thm:dtpa-radius} & open  \\
            Cumulative Reward & \Cref{thm:action-set-ppa} & tight~(\Cref{thm:compare-tight-loose-action-set-ppa}) & \Cref{thm:action-set-tpa} & $\NP$-complete~(\Cref{thm:np-complete-tpa-action-set}) & \Cref{thm:action-set-dtpa} & open \\
            \bottomrule
        \end{tabular}}
        \vspace{-1em}
    \end{table}

    % \section{Our Framework: \sysname}
        % \label{sec:main}
    
    %\fan{aggregation protocol}
    %In this section, we introduce Partition Aggregation for \RL (\rlalgo), an RL training algorithm that can effectively achieve certifiable training-time robustness. 
    %The intuition for the robustness arises from the aggregation over the action predictions given by an ensemble of DQN models.
    %We first briefly introduce the notations, and then outline the algorithm.
    %
    %\fan{certification}
    %In this section, we go into the details regarding the certification that can be obtained for the policy $\mpi$ obtained via \rlalgo, corresponding to the two criteria: per-state action (\Cref{def:per-state}) and cumulative reward (\Cref{def:cert-cum-reward}).

    \vspace{-2mm}
    \subsection{Partition-Based Training Protocol}
        \label{subsec:training-protocol}
        \vspace{-2mm}    
        \sysname's training protocol contains two stages: partitioning  and training.
        We denote $D$ as the entire offline RL training dataset. 
        %, and one subset of it be $T \subseteq D$.
        % \in 2^D$, where $2^D$ represents the power set of $D$.
        %A tuple $t=(s,a,r,s')\in D$ represents a transition starting from $s$, and upon taking the action $a$, receiving the reward $r$ and transitioning to the next state $s'$.
        We abstract an offline RL training algorithm~(\eg, DQN) by $\gM_0: 2^D \rightarrow \Pi$, where $2^D$ is the power set of $D$, and $\Pi = \{ \pi : \gS \rightarrow \gA \}$ is the set of trained policies.
        Each trained policy in $\Pi$ is a function mapping a given state to the predicted action.
        
        % $:\cal S \rightarrow \cal A$ represents a trained DQN policy. The base DQN policy first takes a given subset of the dataset $D$ as the training dataset for learning the DQN. After training is done, for a given state $s \in \cal S$ encountered during test time, the model outputs an action prediction $a \in \cal A$.
        
        \looseness=-1
        % We next describe our partition based training protocol in detail.
        % Linyi: I already defined a macro for \paragraph, so that \paragraph == \textbf{} \quad
        \paragraph{Partitioning Stage.}
        In this stage,
        we separate the training dataset $D$ into $u$ partitions $\{D_i\}_{i=0}^{u-1}$ that satisfy $\bigcup_{i=0}^{u-1}D_i=D$ and $\forall i\neq j,D_i\cap D_j=\emptyset$. 
        Concretely, when performing  partitioning, for each trajectory $\tau \in D$, we \textit{deterministically} assign it to one unique partition.
        The assignment is only dependent on the trajectory $\tau$ itself, and not impacted by any modification to other parts of the training set.
        One design choice of such a deterministic assignment is using a deterministic hash function $h$ to compute the assignment, \ie,
        % \begin{align}
        $
            D_i = \{ \tau \in D \mid h(\tau) \equiv i \ ({\rm mod\ } u)\},\forall i \in [u].
        $
        % \end{align}
        
        % Then, in the \textit{training} stage, 
        \looseness=-1
        \paragraph{Training Stage.}
        In this stage,
        for each training data partition $D_i$, we independently apply an RL  algorithm $\gM_0$ to train a policy $\pi_i = \gM_0(D_i)$.
        Hereinafter, we call these trained polices as \emph{subpolicies} to distinguish from the aggregated policies.
        % we apply the base DQN training mechanism $\gM_0$ on each partition $D_i$ and obtain a trained model $\pi_i = \gM_0(D_i)$.
        % \paragraph{Subpolicies.}
        % We call each learned policy in offline RL \emph{subpolicy} and represent it by $\pi_i = \gM_i(D_i): \gS \to \gA, 0\le i< u$, where $u$ is the number of subpolicies, and $\gM_i$ is the RL training algorithm that learns $\pi_i$ from training dataset $D_i$.
        % % Such dependency may be omitted when there is no ambiguity.
        % As we will introduce in \Cref{subsec:training-protocol}, the subpolicy $\pi_i$'s training dataset $D_i$ is a subset of the whole set $D$.
        % Note that we do not make any  assumption on the learning algorithms or the gap between learned and optimal policies.
        % % We only need a deterministic function from $\gS$ to $\gA$, that is determined by the training dataset. 
        Concretely, let $[u] := \{0,1,\dots,u-1\}$.
        % The output of the training protocol is a set of $u$ subpolicies $\{\pi_i\}_{i=0}^{u-1}$, and the detailed algorithm description is in \Cref{adxsec:alg}.
        For these subpolicies, the \emph{policy indicator} $\1_{i,a}: \gS \to \{0,1\}$ is defined by $\1_{i,a}(s) := \1[\pi_i(s) = a]$, indicating whether subpolicy $\pi_i$ chooses action $a$ at state $s$.
        The \emph{aggregated action count} $n_a: \gS \to \sN_{\ge 0}$ is the number of votes across all the subpolicies for action $a$ given state $s$:
        $
            n_a(s) := | \{i | \pi_i(s) = a, i \in [u] \} | = \sum_{i=0}^{u-1} \1_{i,a}(s).
        $
        Specifically, we denote $n_a(s_{l:r})$ for $\sum_{j=l}^r n_a(s_j)$, \ie, the sum of votes for states between time step $l$ and $r$.
         A detailed algorithm of the training protocol is in \Cref{adxsubsec:algo-train}.
        
       
        Now we are ready to introduce the proposed  aggregation protocols in \sysname~(\rlalgo, \rlalgotmp, \rlalgodyntmp) that generate \emph{aggregated policies} based on subpolicies, and corresponding  certification.
        
        
        % % After $\pi_i$ is trained, 
        % After training is done,
        % for a given state $s_t \in \gS$ at time step $t$ during testing, the policy $\pi_i$ gives the action prediction $a_t = \pi_i(s_t)$.
        % For ease of characterization, we introduce another notation $\lmb_i^a(s_t) = \mathds{1}_{\pi_i(s_t)=a}$ to represent whether the policy $\pi_i$ gives the prediction of action $a$ at state $s_t$.
        % Aggregating the action predictions of all policies, we define an \textit{aggregated action count} $n_a$ that represents the number of votes for action $a$ among $u$ base policies
        % \begin{align}
        %     n_{a}(s_t)&:=\left|\left\{i \in\{0, \ldots, u-1\} \mid \pi_{i}(s_t)=a\right\}\right|,\quad \forall a \in \cal A.
        % \end{align}
        % As a generalization of the \textit{aggregated action count} $n_a$ which aggregate only at the model level, we additionally consider the aggregation along the time steps, and accordingly define a \textit{temporally aggregated action count} $n_a^W$ which represents the number of votes for action $a$ among $u$ base policies in the past $W$ time steps. We refer to the time span $W$ as the \textit{window size} for temporal aggregation in the later text. The definition of $n_a^W$ is provided as follows:
        % \begin{align}
        %     n_a^{W}(s_t) &:= \sum_{j=0}^{\min\{W-1,t\}} \left| \{ i \in \{0,\dots,u-1\} \mid  \pi_i(s_{t-j}) = a \}\right|,\quad \forall a\in\gA.
        % \end{align}
        
        % \fan{TODO: 
        % \begin{enumerate}
        %     \item separate algorithm 1 into two algos: training (in 4.1) and inference + certification (in 4.2)
        % \end{enumerate}
        % }
    
    \vspace{-2mm}
    \subsection{Aggregation Protocols: \rlalgo, \rlalgotmp, \rlalgodyntmp}
        \label{subsec:agg-protocol}
        \vspace{-2mm}
        With $u$ learned subpolicies $\{\pi_i\}_{i=0}^{u-1}$, we propose three different aggregation protocols in \sysname to form three types of aggregated policies for each certification criteria:
        \rlalgo, \rlalgotmp, and \rlalgodyntmp.
        
        \textbf{\rlalgofullname~(\rlalgo).}
        Inspired by aggregation in classification~\citep{levine2021deep},  \rlalgo aggregates subpolicies by choosing actions with the highest votes.
        We denote the \rlalgo aggregated policy by $\rlalgopolicy: \gS \to \gA$.
        When there are multiple highest voting actions, we break ties deterministically by returning the ``smaller'' ($<$) action, which can be defined by numerical order, lexicographical order, etc.
        Throughout the paper, we assume $\argmax$ over $\gA$ always uses $<$ operator to break ties.
        The formal definition of the protocol is in \Cref{adxsec:protocol}.
        
     
        
        
        % \looseness=-1
        The intuition behind \rlalgo is that the poisoning attack within size $K$ can change at most $K$ subpolicies.
        Therefore, as long as the margin between the votes for top and runner-up actions is larger than $2K$ for the given state, after poisoning, we can guarantee that the aggregated \rlalgo policy will not change its action choice.
        We will formally state the robustness guarantee 
        % in \Cref{thm:ppa-radius} 
        in \Cref{subsec:cert-radius}.
        
        \paragraph{\rlalgotmpfullname~(\rlalgotmp).}
        In the sequential decision making process of RL, it is likely that certain important states are much more vulnerable to poisoning attacks, which we refer to as \emph{bottleneck states}.
        Therefore, the attacker may just change the action predictions for these bottleneck states to deteriorate the
        overall performance, say, the cumulative reward.
        For example, in Pong game, we may lose the round when choosing an immediate bad action when the ball is closely approaching the paddle.
        Thus, to improve the overall certified robustness, we need to focus on improving the tolerable poisoning threshold for these bottleneck states.
        Given such intuition and goal, we propose \rlalgotmpfullname~(\rlalgotmp) and the aggregated policy is denoted as $\rlalgotmppolicy$, which is formally defined in \Cref{def:tpa-agg} in \Cref{adxsec:protocol}.
        
        \rlalgotmp is based on two insights:
        (1)~Bottleneck states have lower tolerable poisoning threshold, which is because the vote margin between the top and runner-up actions is smaller at such state;
        (2)~Some RL tasks satisfy temporal continuity~\citep{legenstein2010reinforcement,veerapaneni2020entity}, indicating that  good action choices are usually similar across states of adjacent time steps, \ie, adjacent states.
        Hence, we leverage the subpolicies' votes from adjacent states to enlarge the vote margin, and thus increase the tolerable poisoning threshold.
        To this end, 
        % \rlalgotmp aggregates the subpolicies' votes for \emph{both} current state and  recent states.
        % Concretely,
        in \rlalgotmp, we predetermine a \emph{window size} $W$, and choose the action with the highest  votes across recent $W$ states.
        
        
        % The robustness certification theorems and methods for this aggregated policy will be described in \Cref{subsec:cert-radius,subsec:cert-reward}.

        \paragraph{\rlalgodyntmpfullname~(\rlalgodyntmp).}
        The \rlalgotmp uses a fixed window size $W$ across all states. Since the specification of the window size $W$ requires certain prior knowledge, plus that the same fixed window size $W$ may not be suitable for all states, it is preferable to perform \emph{dynamic temporal aggregation} by using a flexible window size. 
        Therefore, we propose \rlalgodyntmpfullname~(\rlalgodyntmp), which dynamically selects the window size $W$ towards maximizing the tolerable poisoning threshold \emph{per step}.
        Intuitively, \rlalgodyntmp selects the window size $W$ such that the average vote margin over selected states is maximized.
        To guarantee that only recent states are chosen, we further constrain the maximum window size ($W_{\max}$).
        
        \begin{definition}[\rlalgodyntmpfullname]
            Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and maximum window size $W_{\max}$, at time step $t$, the \rlalgodyntmpfullname~(\rlalgodyntmp) defines an aggregated policy $\rlalgodyntmppolicy: \gS^{\min\{t+1, W_{\max}\}} \to \gA$ such that
            \begin{small}
            \begin{equation}
                \rlalgodyntmppolicy(s_{\max\{t - W_{\max} + 1,0\}:t}) := \argmax_{a\in \gA} n_a(s_{t-W'+1:t}),
                \mathrm{\ where\ }
                W' = \argmax_{1\le W \le \min\{W_{\max}, t+1\}} \Delta_t^W.
                \label{eq:dtpa-agg-1}
            \end{equation}
            \end{small}
            In the above equation, $n_a$ is defined in \Cref{subsec:notation} and $\Delta_t^W$ is given by
            \begin{small}
            \begin{equation}
                \begin{aligned}
                    & \Delta_t^W := \dfrac{1}{W} \left(
                        n_{a_1}(s_{t-W+1:t}) - n_{a_2}(s_{t-W+1:t})
                    \right), \\
                    \mathrm{\ where\ } \quad &
                    a_1 = \argmax_{a\in \gA} n_a(s_{t-W+1:t}), 
                    a_2 = \argmax_{a\in \gA, a\neq a_1} n_a(s_{t-W+1:t}).
                \end{aligned}
                \label{eq:dtpa-agg-2}
            \end{equation}
            \end{small}
            \label{def:dtpa-agg}
        \end{definition}
        \vspace{-1em}
        In the above definition, $\Delta_t^W$ encodes the average vote margin between top action $a_1$ and runner-up action $a_2$ if choosing window size $W$.
        Thus, $W'$ locates the window size with maximum average vote margin, and its corresponding action is selected.
        Again, we use the mechanism described in \rlalgo to break ties.
        Robustness certification methods for \rlalgodyntmp are  in \Cref{subsec:cert-radius,subsec:cert-reward}.
        
        In \Cref{adxsec:running-example}, we present a concrete example to demonstrate how different aggregation protocols induce different tolerable poisoning thresholds, and illustrate bottleneck and non-bottleneck states.
        
        % Given a window size $W$, we denote the top action and the runner-up action according to aggregated action counts by $a^{W,(1)}(s_t)$ and $a^{W,(2)}(s_t)$ \huan{Define the notation $n_a^W$?}:
        % \linyi{Nice catch! I updated the definition to eliminate $n_a^W$}
        % \begin{equation}
        %     a^{W,(1)}(s_t) := \argmax_{a\in \gA} n_a^W(s_t),\,
        %     a^{W,(2)}(s_t) := \argmax_{a\in \gA, a\neq a^{W,(1)}(s_t)} n_a^W(s_t).
        % \end{equation}
        % To dynamically select the window size $W$, we define the average count margin $\Delta_t^W$ when window size is $W$:
        % \begin{equation}
        %     \Delta_t^W := \dfrac{n^W_{a^{W,(1)}(s_t)} (s_t) - n^W_{a^{W,(2)}(s_t)} (s_t)}{W}.
        % \end{equation}
        % We select the window size that achieves the largest average count margin and extract its top-counted action, as our policy $\pi_{\gM_{D}}$.
        % Moreover, we avoid selecting exceedingly long window size by only considering window size smaller or equal to predefined $W_{\max}$.
        % Formally,
        % \begin{equation}
        %     \pi_{\gM_D}(s_t) := \argmax_{a\in \gA} n_a^{W'} (s_t), \, \mathrm{where} \, W' = \argmax_{W \le W_{\max}} \Delta_t^W.
        % \end{equation}
    
    \vspace{-2mm}
    \subsection{Certification of Per-State Action Stability}
        \label{subsec:cert-radius}
        \vspace{-2mm}
        In this section, we present our robustness certification theorems and methods for \textit{per-state action}.
        For each of the aggregation protocols~(\rlalgo, \rlalgotmp, and \rlalgodyntmp), at each time step $t$, we will compute a valid \emph{tolerable poisoning threshold} $\wbar K$ as defined in \Cref{def:per-state}, such that the chosen action at step $t$ does not change as long as the poisoning size $K \le \wbar K$.
        
        \textbf{Certification for \rlalgo.}
        Due to the space limit, we defer the robustness certification method for \rlalgo to \Cref{adxsec:ppa-per-state}.
        The certification method is based on \Cref{thm:ppa-radius}.
        We further show the theoretical tightness of the certification in \Cref{prop:ppa-radius-tightness}.
        All the theorem statements are in \Cref{adxsec:ppa-per-state}.
        
        
        \textbf{Certification for \rlalgotmp.}
        We certify the robustness of \rlalgotmp following \Cref{thm:tpa-radius}.
        
        \begin{theorem}
            \label{thm:tpa-radius}
            Let $D$ be the clean training dataset;
            let $\pi_i = \gM_0(D_i), 0\le i \le u-1$ be the learned subpolicies according to \Cref{subsec:training-protocol} from which we define $n_a$~(\Cref{subsec:notation});
            and let $\rlalgotmppolicy$ be the \rlalgotmpfullname policy: $\rlalgotmppolicy = \gM(D)$ where $\gM$ abstracts the whole training-aggregation process.
            $\wtilde D$ is a poisoned dataset and $\wtilde \rlalgotmppolicy$ is the poisoned policy:
            $\wtilde \rlalgotmppolicy = \gM(\wtilde D)$.
            
            For a given state $s_t$ encountered at time step $t$ during test time, 
            let $a := \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t})$, then
            {\color{black}
            at time step $t$ the tolerable poisoning threshold~(see \Cref{def:per-state})
            }
            \begin{small}
            \begin{equation}
                \wbar K_t = \min_{a' \neq a, a'\in \gA} 
                % \argmax_{\sum_{i=1}^p h_{a,a'}^{(i)} \le \delta_{a,a'}} p
                {
                \color{black}
                \max \left\{p \,\Big\lvert\, \sum_{i=1}^p h_{a,a'}^{(i)} \le \delta_{a,a'} \right\}
                }
                \label{eq:tpa-radius-1}
            \end{equation}
            \end{small}
            % is a \emph{tolerable threshold} at time step $t$ in \Cref{def:per-state},
            where $\{h_{a,a'}^{(i)}\}_{i=1}^u$ is a nonincreasing permutation of 
            \begin{small}
            \begin{equation}
                \small
                \left\{ 
                \sum_{j=0}^{\min\{W-1, t\}} \1_{i,a}(s_{t-j}) + \min\{W, t+1\} - 
                \sum_{j=0}^{\min\{W-1, t\}} \1_{i,a'}(s_{t-j}) \right\}_{i=0}^{u-1} =: \{h_{i,a,a'}\}_{i=0}^{u-1},
                \label{eq:tpa-radius-2}
            \end{equation}
            \end{small}
            and $\delta_{a,a'} := n_a(s_{\max\{t-W+1,0\}:t}) - (n_{a'}(s_{\max\{t-W+1,0\}:t}) + \1[a'<a])$.
            Here, $\1_{i,a}(s) = \1[\pi_i(s)=a]$~(\Cref{subsec:notation}), and $W$ is the window size.
        \end{theorem}
        
        % \vspace{-1em}
        % \begin{proof}[Proof sketch.]
        %     Let $t_s = \max\{t-W+1,0\}$.
        %     We consider the condition of successful poisoning, which is to enable $a'$ to satisfy $\wtilde n_{a'}(s_{t_s:t}) + \1[a'<a] > \wtilde n_a(s_{t_s:t})$ after the poisoning.
        %     We figure out the optimal attack strategy towards satisfying this constraint and negation of this optimal attack brings the theorem statement.
        %     % Thus, we need to maximize $\wtilde n_{a'}(s_{t_s:t}) - \wtilde n_a(s_{t_s:t})$.
        %     % The optimal attack strategy on subpolicy $i$ provides a gain of $h_{i,a,a'}$ on the objective.
        %     % Since poisoning different subpolicies is independent, and the optimal attack will greedily choose subpolicies with maximum gains to poison.
        %     % A negation of this optimal attack strategy brings the theorem statement.
        %     We defer the detailed proof to \Cref{adxsubsec:proof-C2}.
        % \end{proof}
        
        \begin{remark}
            We defer the detailed proof to \Cref{adxsubsec:proof-C2}.
            The theorem provides a per-state action certification for \rlalgotmp.
            The detailed algorithm is in \Cref{alg:tpa-radius}~(\Cref{adxsec:alg-perstate}).
            The certification time complexity per state is $O(|\gA| u (W + \log u))$ and can be further optimized to $O(|\gA| u \log u)$ with proper prefix sum caching across time steps.
            We prove the certification for \rlalgotmp is theoretically tight in \Cref{prop:tpa-radius-tightness}~(proof in \Cref{adxsubsec:proof-C3}). 
            We also prove that directly extending \Cref{thm:ppa-radius} for \rlalgotmp~(\Cref{cor:tpa-radius-2}) is loose in \Cref{adxsubsec:proof-C4}.
        \end{remark}
      
        
        \begin{proposition}
            \label{prop:tpa-radius-tightness}
            Under the same condition as \Cref{thm:tpa-radius}, for any time step $t$,
            there exists an RL learning algorithm $\gM_0$, and a poisoned dataset $\wtilde D$, such that $| D \ominus \wtilde D | = \wbar K_t + 1$, and $\wtilde \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t}) \neq \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t})$.
        \end{proposition}
        
        % % By the argument that after poisoning, the aggregated action count $\wtilde n_a(s_{\max\{t-W+1,0\}:t}) - n_a(s_{\max\{t-W+1,0\}:t}) \in [-K\min\{W,t+1\},K\min\{W,t+1\}]$, 
        % A direct extension of \Cref{thm:ppa-radius}, \Cref{cor:tpa-radius-2}, can also provide a robustness certification for \rlalgotmp.
        
        % \begin{corollary}
        %     \label{cor:tpa-radius-2}
        %     Under the same condition as \Cref{thm:tpa-radius},
        %     \begin{equation}
        % 	    \wbar K_t = \left\lfloor\frac{n_{a}(s_{\max\{t-W+1,0\}:t})-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}(s_{\max\{t-W+1,0\}:t})+\1[a^{\prime}<a]\right)}{2\min\{W,t+1\}}\right\rfloor
        % 	    \label{eq:rpa-radius-2}
        % 	\end{equation}
        % 	is a \emph{tolerable poisoning threshold} at time step $t$ in \Cref{def:per-state}, where $W$ is the window size.
        % \end{corollary}
        % % The proof is in \Cref{adxsec:proofs}.
        % However, the certification from \Cref{cor:tpa-radius-2} is looser than \Cref{thm:tpa-radius}, \ie, the $\wbar K_t$ from \Cref{cor:tpa-radius-2} is smaller or equal to \Cref{thm:tpa-radius}.
        % Proof and discussion is deferred to \Cref{adxsubsec:loose-tpa-and-compare}.
        
        \textbf{Certification for \rlalgodyntmp.}
        % We certify the robustness of \rlalgodyntmp following \Cref{thm:dtpa-radius}.
        \Cref{thm:dtpa-radius} provides certification for \rlalgodyntmp.
        
        \begin{theorem}
            \label{thm:dtpa-radius}
            Let $D$ be the clean training dataset;
            let $\pi_i = \gM_0(D_i), 0\le i \le u-1$ be the learned subpolicies according to \Cref{subsec:training-protocol} from which we define $n_a$~(see \Cref{subsec:notation});
            and let $\rlalgodyntmppolicy$ be the \rlalgodyntmpfullname:
            $\rlalgodyntmppolicy = \gM(D)$ where $\gM$ abstracts the whole training-aggregation process.
            $\wtilde D$ is a poisoned dataset and $\wtilde \rlalgodyntmppolicy$ is the poisoned policy:
            $\wtilde \rlalgodyntmppolicy = \gM(\wtilde D)$.
            
            For a given state $s_t$ encountered at time step $t$ during test time, let $a := \rlalgodyntmppolicy(s_{\max\{t - W_{\max} + 1,0\}:t})$ and $W'$ be the chosen time window~(according to \Cref{eq:dtpa-agg-1}), then tolerable poisoning threshold
            \begin{small}
            \begin{equation}
                \wbar K_t^D = \min\left\{ \wbar K_t,\, \min_{1\le W^* \le \min\{W_{\max}, t+1\}, W^* \neq W', a'\neq a, a''\neq a} L_{a',a''}^{W^*, W'} \right\}
                \label{eq:dtpa-radius}
            \end{equation}
            \end{small}
            % is a \emph{tolerable poisoning threshold} at time step $t$ in \Cref{def:per-state}, 
            where $\wbar K_t$ is defined by \Cref{eq:tpa-radius-1} with  $W$ as $W'$ and $L_{a,a''}^{W^*, W'}$ defined by the below \Cref{def:L}.
        \end{theorem}
        
        \begin{definition}[$L$ in \Cref{thm:dtpa-radius}]
            \label{def:L}
            Under the same condition as \Cref{thm:dtpa-radius}, for given $W^*, W', a, a', a''$,
            we let $a^\# := \argmax_{a_0\neq a', a_0\in \gA} n_{a_0}(s_{t-W^*+1:t})$, then
            \begin{small}
            \begin{equation}
                L_{a',a''}^{W^*, W'} :=
                % \argmax_{
                %     \sum_{i=1}^p g^{(i)} + W'(n_{a'}^{W^*} - n_{a^\#}^{W^*}) - W^*(n_{a}^{W'} - n_{a''}^{W'}) - \1[a' > a]
                %     < 0
                % } p,
                {\color{black}
                \max \left\{ p \,\Big\lvert\, 
                \sum_{i=1}^p g^{(i)} + W'(n_{a'}^{W^*} - n_{a^\#}^{W^*}) - W^*(n_{a}^{W'} - n_{a''}^{W'}) - \1[a' > a]
                    < 0
                \right\}
                }
                \label{eq:L-1}
            \end{equation}
            \end{small}
            where $n_a^w$ is a shorthand of $n_a(s_{t-w+1:t})$ and $\{g^{(i)}\}_{i=1}^u$ is a nonincreasing permutation of $\{g_i\}_{i=0}^{u-1}$.
            Each $g_i$ is defined by
            % \vspace{-0.5em}
            % \begin{equation}
                % g_i := \sum_{w=0}^{\max\{W^*, W'\}} \max_{a_0\in \gA} \sigma^w(a_0) - \sigma^w(\pi_i(s_{t-w})),
                % \begin{aligned}
                %     \sigma^w(a_0) := & W'\1[a_0=a', w\le W^*] - W'\1[a_0=a^\#, w\le W^*] \\
                %     & - W^* \1[a_0=a, w\le W'] + W^* \1[a_0=a'', w \le W'].
                % \end{aligned}
                % \resizebox{\textwidth}{!}{$
            \begin{small}
            \begin{equation}
                g_i:= \sum_{w=0}^{\max\{W^*, W'\}} 
                \max_{a_0\in \gA} \sigma^w(a_0) - \sigma^w(\pi_i(s_{t-w})), \text{ where }  
                \label{eq:L-2} 
            \end{equation}
            \end{small}
            \resizebox{\textwidth}{!}{$
                    \sigma^w(a_0) := W'\1[a_0=a', w\le W^*] - W'\1[a_0=a^\#, w\le W^*] %\\
                    % & 
                    - W^* \1[a_0=a, w\le W'] + W^* \1[a_0=a'', w \le W'].
            $}
            % \end{equation}
            % We let $a_1 := a, a_2 := a'', a_3 := a', a_4 := \argmax_{a\neq a_3} n_a^{W^*}(s_t)$.
            % For each policy $\pi_i$, for each $w \in [W_{\max}+1]$, we define an auxiliary function $\sigma^{w}: \gA \to \sR$ such that
            % \begin{equation}
            %     \sigma^w(a) := W' \1[a=a_3, w\le W^*] - W' \1[a=a_4, w\le W^*] - W^* \1[a=a_1, w \le W'] + W^* \1[a=a_2, w \le W'].
            % \end{equation}
            % The auxiliary margin $g_i \in \sR$ of each policy $\pi_i$ is defined by
            % \begin{equation}
            %     g_i := \sum_{w=0}^{W_{\max}} \max_{a\in \gA} \sigma^w(a) - \sigma^w(\pi_i(s_{t-w})).
            % \end{equation}
            % Let $\{g^{(i)}\}_{i=1}^u$ be a non-increasing sorted permutation of $\{g_i\}_{i=0}^{u-1}$.
            % Then,
            % \begin{equation}
            %     J_{a',a''}^{W^*,W'} := \argmax_{\sum_{i=1}^p g^{(i)} + W'(n_{a_3}^{W^*} - n_{a_4}^{W^*}) - W^*(n_{a_1}^{W'} - n_{a_2}^{W'}) - \1[a_3 > a_1] \le 0} p.
            % \end{equation}
        \end{definition}
        \vspace{-1em}
        
        \begin{proof}[Proof sketch.]
            A successful poisoning attack should change the chosen action from $a$ to an another $a'$.
            If after attack, the chosen window size is still $W'$, the poisoning size should be at least larger than $\wbar K_t$ according to \Cref{thm:tpa-radius}.
            If the chosen window size is not $W'$, we find out that the poisoning size is at least $\min_{a''\neq a} L_{a',a''}^{W^*, W'} + 1$ from a greedy-based analysis.
            % Taking the global minimum over $L_{a',a''}^{W^*,W'}$  yields a sufficient condition of robustness, as any window size $W'$ and any other action $a'$ cannot successfully poison the action choice.
            Formal proof is in \Cref{adxsubsec:proof-C5}.
        \end{proof}
        
            \begin{remark}
            The theorem provides a valid per-state action certification for \rlalgodyntmp policy.
            The detailed algorithm is in \Cref{alg:dtpa-radius}~(\Cref{adxsec:alg-perstate}).
            The certification time complexity per state is $O(W_{\max}^2 |\gA|^2 u + W_{\max} |\gA|^2 u \log u)$, which in practice adds similar overhead compared with \rlalgotmp certification~(\textcolor{black}{see~\Cref{adxsubsec:stat-dparl}}).
            Unlike certification for \rlalgo and \rlalgotmp, the certification given by \Cref{thm:dtpa-radius} is not theoretically tight.
            % although in practice, the certification is still tight  as shown in \TODO.
            An interesting future work would be providing a tighter  per-state action certification for \rlalgodyntmp.
        \end{remark}
        
    \vspace{-2mm}
    \subsection{Certification of Cumulative Reward Bound}
        \label{subsec:cert-reward}
        \vspace{-2mm}
        % {\color{blue}
        % Due to the space limit, we defer the robustness certification methods for cumulative reward to \Cref{adxsec:cumulative-reward}.
        % In summary, we propose a novel adaptive tree search algorithm \adasearch to compute a lower bound of cumulative reward under poisoning attacks, as long as the poisoning size is within predefined threshold $K$.
        % The core of the algorithm is to figure out the possible action set $A(K)$: given previous states, subpolicies, and the poisoning threshold $K$, what are the possible actions that can be chosen by the current aggregated policy.
        
        % For \rlalgo, we compute possible action set by \Cref{thm:action-set-ppa}, which gives theoretically tight possible action set and is tighter than a direct extension of \rlalgo's per-state certification.
        % For \rlalgotmp, we compute possible action set by \Cref{thm:action-set-tpa}.
        % Interestingly, for \rlalgotmp, computing a theoretically tight possible action set is an $\NP$-complete problem.
        % This leads to the hardness of targeted attack on \rlalgotmp, and indicates the robustness property of \rlalgotmp.
        % For \rlalgodyntmp, we compute possible action set by \Cref{thm:action-set-dtpa}.
        % For \rlalgodyntmp, an open problem is whether theoretically tight certification is also an $\NP$-complete problem as in \rlalgotmp.
        % We conjecture this is true, and leave it as an interesting future direction.
        
        % We list the expressions of $A(K)$ for different aggregation protocols in \Cref{tab:AK-expressions}.
        % Please refer to \Cref{adxsec:cumulative-reward} for theorem statements and other details.
        % }
        
        % \begin{table}[t]
        %     \centering
        %     \caption{\small Expressions of possible action set $A(K)$ given poisoning threshold $K$ for different aggregation protocols.
        %     Full theorem statements are in \Cref{thm:action-set-ppa,thm:action-set-tpa,thm:action-set-dtpa}~(in \Cref{adxsec:cumulative-reward}).}
        %     \vspace{-1em}
        %     \resizebox{\textwidth}{!}{
        %     \begin{tabular}{c|c}
        %         \hline
        %         Protocol & $A(K)$ \\
        %         \hline
        %         \rlalgo & $\left\{
        %             a \in \gA 
        %             \,\Big\lvert\,
        %             \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a'<a], 0\} \le K
        %         \right\}$ \\
        %         % \hline
        %         \rlalgotmp & $\left\{ a \in \gA 
        %             \,\Big\lvert\,
        %             \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
        %         \right\}$ \\
        %         % \hline
        %         \rlalgodyntmp & $ \displaystyle
        %         % \begin{aligned}
        %             \{a_t\} \cup 
        %             \left\{ 
        %             a' \in \gA
        %             \,\Big\lvert\,
        %                 \min_{1\le W^*\le \min\{W_{\max}, t+1\}, W^* \neq W', a''\neq a_t} L_{a',a''}^{W^*,W'} \le K
        %             \right\} %\\
        %             \cup
        %             \left\{
        %             a \in \gA
        %             \,\Big\lvert\,
        %                 \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
        %             \right\}
        %         % \end{aligned}
        %         $ \\
        %         \bottomrule
        %     \end{tabular}
        %     }
        %     \label{tab:AK-expressions}
        % \end{table}
        
        
        \vspace{-2mm}
        In this section, we present our robustness certification for \textit{cumulative reward bound}.
        We assume the deterministic RL environment throughout the cumulative reward certification for convenience, \ie, the transition function is $P: \gS \times \gA \to \gS$
        % instead of $P: \gS \times \gA \to \gP(\gS)$ 
        and the initial state is a fixed $s_0 \in \gS$.
        % rather than $d_0 \in \gP(\gS)$.
        The certification goal, as listed in \Cref{def:cum-reward}, is to obtain a lower bound of cumulative reward under  poisoning attacks, given bounded poisoning size $K$.
        {\color{black}
        The cumulative reward certification is based on a novel adaptive search algorithm \adasearch inspired from \cite{wu2022crop}; we tailor the algorithm to certify against poisoning attacks. We defer detailed discussions and complexity analysis to~\Cref{adxsubsec:alg-reward}.
        % instead of adversarial state perturbations as in \cite{wu2022crop}.
        % A detailed discussion and complexity analysis of the algorithm is in \Cref{adxsubsec:alg-reward}.
        }
        
        \paragraph{\adasearch Algorithm Description.}
        The pseudocode is in \Cref{alg:tree-search}~(\Cref{adxsubsec:alg-reward}).
        The method starts from the base case: when the poisoning threshold $K_{\mathrm{cur}} = 0$, the lower bound of cumulative reward $\uj_{K_{\mathrm{cur}}}$ is exactly the reward without poisoning.
        The method then gradually increases the poisoning threshold $K_{\mathrm{cur}}$, by finding the immediate larger $K' > K_{\mathrm{cur}}$ that can expand the possible action set along the trajectory.
        With the increase of $K_{\mathrm{cur}} \gets K'$, the attack may cause the poisoned policy $\tpi$ to take different actions at some states, thus resulting in new trajectories.
        We need to figure out \emph{a set of all possible actions} to exhaustively traverse all possible trajectories.
        We will introduce theorems to compute this set of possible actions.
        With this set, the method effectively explores these new trajectories by formulating them as expanded branches of a trajectory tree.
        Once all new trajectories are explored, the method examines all leaf nodes of the tree and figures out the minimum reward among them, which is the new lower bound of cumulative reward $\uj_{K'}$ under new poisoning size $K'$.
        We then repeat this process of increasing poisoning size from $K'$ and expanding with new trajectories until we reach a predefined threshold for poisoning size $K$.

        
        % As we can see, the core of \adasearch is figuring out the \emph{possible action set}.
        \begin{definition}[Possible Action Set]
            \label{def:possible-action-set}
            Given previous states $s_{0:t}$, the subpolicies $\{\pi_i\}_{i=0}^{u-1}$, the aggregation protocol~(\rlalgo, \rlalgotmp, or \rlalgodyntmp), and the poisoning size $K$, the \emph{possible action set} $A$ at step $t$ is a subset of action space: $A \subseteq \gA$, such that for any poisoned policy $\wtilde \pi$, as long as the poisoning size is within $K$, the chosen action at step $t$ will always be in $A$, \ie, $a_t = \wtilde \pi(s_{0:t}) \in A$.
        \end{definition}
        
        \paragraph{Possible Action Set for \rlalgo.}
        The following theorem gives the possible action set for \rlalgo.
        
        \begin{theorem}[Tight \rlalgo Action Set]
            \label{thm:action-set-ppa}
            Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
            then the \emph{possible action set} at step $t$
            \begin{small}
            \begin{equation}
                A^T(K) = \left\{
                    a \in \gA 
                    \,\Big\lvert\,
                    \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a'<a], 0\} \le K
                \right\}.
                \label{eq:action-set-ppa}
            \end{equation}
            \end{small}
        \end{theorem}
        \vspace{-0.5em}
        % \begin{remark}
            We defer the proof to \Cref{adxsubsec:proof-C61}.
            Furthermore, in \Cref{adxsubsec:proof-C62} we show that:
            1)~The theorem gives theoretically tight possible action set;
            2)~In contrast, directly extending \rlalgo's per-state certification gives loose certification.
        % \end{remark}
        
        % \begin{proof}[Proof sketch.]
        %     Within poisoning size $K$, the optimal attack strategy towards making $a \in \gA$  the chosen action is to let some subpolicies flip their action to $a$.
        %     Then the problem is what subpolicies need to be selected to flip.
        %     It turns out to be all subpolicies whose current action $a'$ has votes $\ge n_a(s_t) + K + 1 - \1[a' < a]$, which completes the proof.
        %     Detailed proof is in \Cref{adxsubsec:proof-C61}.
        % \end{proof}
        
        % \begin{remark}
        % In \Cref{adxsubsec:proof-C62} we prove that   \Cref{thm:action-set-ppa} is  theoretically tight in \Cref{thm:compare-tight-loose-action-set-ppa}. In addition, we show that a direct extension of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) can also yield possible action set~(\Cref{cor:loose-action-set-ppa} in \Cref{adxsubsec:proof-C61}), which is loose than \Cref{thm:action-set-ppa} as proved in \Cref{thm:compare-tight-loose-action-set-ppa}.
        % In other words, a theoretically tight possible action set combined with the proposed \adasearch leads to a theoretically tight certification of cumulative reward. 
        %     % In \Cref{adxsubsec:proof-C61},
        %     % we show that a direct extension of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) can also yield possible action set~( \Cref{cor:loose-action-set-ppa}), and in \Cref{adxsubsec:proof-C62} we prove \Cref{thm:compare-tight-loose-action-set-ppa} stating that \Cref{thm:action-set-ppa} is tighter than \Cref{cor:loose-action-set-ppa}, and \Cref{thm:action-set-ppa} is also theoretically tight.
        % \end{remark}
        
        % In contrast, a generalization of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) yields a loose action set.
        % \begin{corollary}[Loose \rlalgo Action Set]
        %     \label{cor:loose-action-set-ppa}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
        %     then the \emph{possible action set} at step $t$
        %     \begin{equation}
        %         A^L(K) = \left\{
        %             a \in \gA
        %             \,\Big\lvert\,
        %             \max_{a'\in \gA} n_{a'}(s_t) - n_a(s_t) \le 2K - \1[a > \argmax_{a'\in \gA} n_{a'}(s_t)]
        %         \right\}.
        %         \label{eq:loose-action-set-ppa}
        %     \end{equation}
        % \end{corollary}
        
        % As the following theorem show, the \Cref{cor:loose-action-set-ppa} is typically looser than \Cref{thm:action-set-ppa}, and indeed \Cref{thm:action-set-ppa} is theoretically tight.
        % We also compare \Cref{thm:action-set-ppa} and \Cref{cor:loose-action-set-ppa} in practice in \TODO.
        
        % \begin{theorem}
        %     \label{thm:compare-tight-loose-action-set-ppa}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
        %     $A^T(K), A^L(K)$ are defined according to \Cref{eq:action-set-ppa,eq:loose-action-set-ppa} accordingly, then
        %     \begin{enumerate}[leftmargin=*]
        %         \item $A^T(K) \subseteq A^L(K)$; and there are subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$ such that $A^T(K) \subsetneq A^L(K)$.
                
        %         \item Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$, for any $a \in A^T(K)$, there exists a poisoned training set $\wtilde D$ whose poisoning size $|D \ominus \wtilde D| \le K$ and some RL training mechanism, such that $\wtilde \rlalgopolicy(s_t) = a$ where $\wtilde \rlalgopolicy$ is the poisoned \rlalgo policy trained on $\wtilde D$.
        %     \end{enumerate}
        % \end{theorem}
        
        % We defer the proofs of \Cref{cor:loose-action-set-ppa} and \Cref{thm:compare-tight-loose-action-set-ppa} to \Cref{adxsubsec:proof-C62}.
        
        % \begin{remark}
        %     Specifically, the first point in \Cref{thm:compare-tight-loose-action-set-ppa} shows that the certification from \Cref{cor:loose-action-set-ppa} is usually looser than that from \Cref{thm:action-set-ppa}; and the second point shows the theoretical tightness of \Cref{thm:action-set-ppa}.
        %     Indeed, a theoretically tight possible action set combined with the proposed \adasearch leads to a theoretically tight certification of cumulative reward.
        % \end{remark}
        
        \paragraph{Possible Action Set for \rlalgotmp.}
        The following theorem gives the possible action set for \rlalgotmp.
        \vspace{-1em}
        \begin{theorem}
            \label{thm:action-set-tpa}
            Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgotmp as defined in \Cref{def:tpa-agg},
            then the \emph{possible action set} at step $t$
            \begin{small}
            \begin{equation}
                A(K) = \left\{ a \in \gA 
                    \,\Big\lvert\,
                    \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
                \right\},
                \label{eq:action-set-tpa}
            \end{equation}
            \end{small}
            where $h_{a',a}^{(i)}$ and $\delta_{a',a}$ follow the definition in \Cref{thm:tpa-radius}.
        \end{theorem}
        
        % \begin{remark}
            We defer the proof to \Cref{adxsubsec:proof-C7}.
            The possible action set here is no longer theoretically tight.
            Indeed, the problem of computing a possible action set with minimum cardinality for \rlalgotmp is $\NP$-complete as we shown in the following theorem~(proved in \Cref{adxsubsec:proof-C8}), where we reduce computing theoretically tight possible action set to the set cover problem~\citep{karp1972reducibility}.
            This result can be viewed as the hardness of targeted attack.
            In other words, the optimal \emph{untargeted} attack on \rlalgotmp can be found in polynomial time, while the optimal \emph{targeted} attack on \rlalgotmp is $\NP$-complete, which indicates the robustness property of proposed \rlalgotmp. 
        % \end{remark}
        
        % \begin{proof}[Proof sketch.]
        %     We first show that any possible action $a$ must be able to be poisoned to achieve higher votes than any other actions $a'$.
        %     Therefore, a necessary condition is that, after applying the greedy selection strategy to shrink the vote margin between $a'$ and $a$, the votes of $a$ is higher than the votes of $a'$, \ie, $\sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}$.
        %     The detailed proof is in \Cref{adxsec:proofs}.
        % \end{proof}
        
        % The possible action set given by \Cref{thm:action-set-tpa} is no longer theoretically tight.
        % In other words, there may exist a possible action set with fewer elements than that given by \Cref{eq:action-set-tpa}.
        % Indeed, the problem of computing a possible action set with minimum cardinality for \rlalgotmp is $\NP$-complete.
        
        \begin{theorem}
            \label{thm:np-complete-tpa-action-set}
            Under the condition of \Cref{def:possible-action-set}, suppose we use \rlalgotmp~(\Cref{def:tpa-agg}) as the aggregation protocol, then computing a possible action set $A(K)$ such that any possible action set $S$ satisfies $|A(K)| \le |S|$ is  $\NP$-complete.
            \vspace{-0.5em}
        \end{theorem}
        
        % We prove the theorem by a reduction to set cover problem~\citep{karp1972reducibility}, with proofs in \Cref{adxsec:proofs}.
        
        % \begin{remark}
        %     This theorem shows a counter-intuitive property of \rlalgotmp aggregated policy.
        %     From \Cref{thm:tpa-radius}, \rlalgotmp has a theoretically tight certification of per-state action, which can be computed in $O(|\gA|u(W+\log u))$ time.
        %     From the proof, we can  craft an optimal attack that deviates the chosen action from the clean policy's choice, which can be viewed as untargeted attack.
        %     In contrast, from \Cref{thm:np-complete-tpa-action-set}, \rlalgotmp \emph{cannot} determine whether a particular action $a'$ can be chosen with a poisoning attack unless $\NP = \mathsf{P}$.
        %     This can be viewed as the hardness of targeted attack.
        %     In other words, the optimal \emph{untargeted} attack on \rlalgotmp can be found in polynomial time, while the optimal \emph{targeted} attack on \rlalgotmp is $\NP$-complete, which indicates the robustness property of proposed \rlalgotmp. 
        % \end{remark}
        
        \paragraph{Possible Action Set for \rlalgodyntmp.}
        The following theorem gives the possible action set for \rlalgodyntmp.
        \vspace{-1em}
        \begin{theorem}
            \label{thm:action-set-dtpa}
            Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgotmp as defined in \Cref{def:dtpa-agg},
            then the \emph{possible action set} at step $t$
            \begin{small}
            \begin{equation}
                \label{eq:action-set-dtpa}
                % \begin{aligned}
                %     A(K) = \{a_t\} & 
                %     \cup 
                %     \left\{ 
                %     a' \in \gA
                %     \,\Big\lvert\,
                %         \min_{1\le W^*\le \min\{W_{\max}, t+1\}, W^* \neq W', a''\neq a_t} L_{a',a''}^{W^*,W'} \le K
                %     \right\} \\
                %     & 
                %     \cup
                %     \left\{
                %     a \in \gA
                %     \,\Big\lvert\,
                %         \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
                %     \right\}
                % \end{aligned}
                \resizebox{0.9\linewidth}{!}{
                $ \displaystyle
                A(K) = \{a_t\} 
                \cup 
                \left\{ 
                a' \in \gA
                \,\Big\lvert\,
                    \min_{\substack{1\le W^*\le \min\{W_{\max}, t+1\},\\ W^* \neq W', a''\neq a_t}} L_{a',a''}^{W^*,W'} \le K
                \right\}
                \cup
                \left\{
                a \in \gA
                \,\Big\lvert\,
                    \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
                \right\}
                $
                }
            \end{equation}
            \end{small}
            where
            $a_t = \rlalgodyntmppolicy(s_{\max\{t - W_{\max} + 1,0\}:t})$ is the clean policy's chosen action,
            $W'$ is defined by \Cref{eq:dtpa-agg-1},
            $L_{a',a''}^{W^*,W'}$ is defined by \Cref{def:L} with $a$ being replaced by $a_t$,
            and $h_{a',a}^{(i)}, \delta_{a',a}$ is defined in \Cref{thm:tpa-radius} with $W$ replaced by $W'$.
        \end{theorem}
        
        % \begin{remark}
            We prove the theorem in \Cref{adxsubsec:proof-C8}.
            As summarized in \Cref{table:theory-overview}, we further prove the tightness or hardness of certification for \rlalgo and \rlalgotmp, while for \rlalgodyntmp it is an interesting open problem  on whether theoretical tight certification is possible in polynomial time.
            % We leave it as an interesting future exploration.
        % \end{remark}
        
        % \begin{proof}[Proof sketch.]
        %     The possible action set given by \Cref{eq:action-set-dtpa} is composed of three parts that encode the possible actions:
        %     (1)~the actions chosen by the aggregated policy without poisoning;
        %     (2)~the actions that may be chosen if the poisoning attack shifts the chosen window size;
        %     (3)~the actions that may be chosen if the poisoning attack does not shift the chosen window size.
        %     For each category, we show that the given set includes all possible actions.
        %     A detailed proof is in \Cref{adxsec:proofs}.
        % \end{proof}
        
        % \begin{remark}[Open problem]
        %     For two aggregation protocols~(\rlalgo and \rlalgotmp), we either provide theoretically tight certification or show they are $\NP$-complete.
        %     In contrast,
        %     for the \rlalgodyntmp aggregation protocol,  we only prove the theoretically tight certification for per-state action~(\Cref{thm:dtpa-radius}). For cumulative reward~(via possible action set given by \Cref{thm:action-set-dtpa}) we do not prove its theoretical tightness in polynomial time (in exponential time we can provide theoretically tight certification by enumerating all $|\gA|^{uW_{\max}}$ possible assignments)).
        %     % nor we show whether theoretically tight certification in polynomial time exists~(in exponential time we can have theoretically tight certification by enumerating all $|\gA|^{uW_{\max}}$ possible assignments).
        %     We conjecture that the theoretically tight certification for \rlalgodyntmp is an $\NP$-complete problem, and leave it as an interesting future exploration.
        % \end{remark}
        
        % \linyi{Deleted the NP-complete statement of cumulative reward certification, since with finite state space, the problem is not NP-complete. It is just the state space is exponentially large for current problems so the reward certification also needs exponential time. I will do a global search to make other parts consistent.}
        
        % \paragraph{General Hardness of Cumulative Reward Certification.}
        % To this point, we have introduced the theorems for computing possible action sets for \rlalgo, \rlalgotmp, and \rlalgodyntmp aggregation protocols.
        % They can be combined with \adasearch to provide robustness certification for cumulative reward.
        % In the worst case, \adasearch needs to explore a superset of all trajectories of possible poisoned policies, which seems to be costly~(though performs good in practice as shown in \TODO).
        % One may think that whether more efficient and tighter certification method exists.
        % However, the following result implies that theoretically tight certification may need inevitably high computational cost.
        % \begin{theorem}
        %     \label{thm:general-hardness-reward}
        %     The problem of computing $\max \uj_K$ defined by \Cref{def:cert-cum-reward} given general deterministic environment $\gE=(\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{u-1}$, poisoning size $K$, and aggregation protocols belonging to \rlalgo, \rlalgotmp, and \rlalgodyntmp is $\NP$-complete.
        % \end{theorem}
        
        % \begin{proof}[Proof sketch.]
        %     We prove the theorem by encoding the classical \textsf{3-SAT} problem with a sequential decision making environment.
        %     The detailed proof is in \Cref{adxsec:proofs}.
        % \end{proof}

% {
% \color{gray}
% \subsection{\rlalgo: \rlalgofullname}


% \subsubsection{\rlalgo Protocol Definition}

%     \label{subsec:ppa-agg-def}


% % \fan{TODO: clean up the description}

% % during \textbf{test} time, for each encountered state $s_t \in \cal S$, we take the majority vote over the action predictions of all the base DQNs, 
% % %which gives the \textit{aggregated action count} $n_a$ and the \textit{aggregated action prediction} $\mpi$ as follows:
% % which gives the aggregated action prediction:
% % \begin{align}
% % 	\label{eq:cnt}
% % 	n_{a}(s_t)&:=\left|\left\{i \in\{0 \ldots u-1\} \mid \pi_{i}(s)=a\right\}\right|,\quad \forall a \in \cal A,\\
% % 	\label{eq:agg}
% % 	\pi_{\cal M} (s_t)&:=\argmax_{a\in \cal A} n_a(s_t),
% % \end{align}
% % where $n_a$ is the \textit{aggregated action count} that represents the number of votes for action $a$ among $u$ base policies, and $\mpi$ is the \textit{aggregated policy} given by \rlalgo.
% % When taking the argmax in eq.~\ref{eq:agg}, we break ties deterministically by returning the ``smaller'' action---we define a ``smaller-than'' operator $<$ on the action set. Examples include numerical order, lexicographical order, and so on.


% % \input{algos-PA-RL}


% \subsubsection{Cumulative Reward Certification for \rlalgo}

% Now we turn to provide the cumulative reward certification for \rlalgo, which aims to compute the lower bound of cumulative reward $\uj_K$ given the attack size $K$.
% We assume the environment to be deterministic following \citep{wu2022crop}, otherwise it would be intractable to obtain a deterministic cumulative reward bound.
% Formally, the transition function $P$ is a mapping from $\gS \times \gA$ to $\gS$ instead of $\gP(\gS)$, and the initial state $d_0 = s_0 \in \gS$ rather than $d_0 \in \gP(\gS)$.

% \begin{theorem}
% 	Let $(\rho_t^1, \ldots, \rho_t^{|\cal A|-1})$ be a list of certified attack magnitudes for state $s_t$ at time step $t$, where $\rho_t^i$ denotes the magnitude such that if the attack magnitude $| D \ominus \wtilde D | \leq\rho_t^i$, the possible action at time step $t$ will belong to the actions corresponding to top $i$ votes at state $s_t$. 
% %	Let $j_i$ be the index of the action of the $i$-th highest votes, \ie, $n_{a_{j_1}} \geq n_{a_{j_2}} \geq \cdots n_{a_{j_{|\cal A|}}}$	
%         The  definition of $\rho_t$ in~\Cref{thm:radius} is equivalent to $\rho_t^1$ here. 
%         The magnitudes can be computed similarly as follows:
% %        \vspace{-1mm}
% %        \begin{small}
%         \begin{align}
%                 \rho_t^i := \left\lfloor\frac{n_{a}(s_t)-\left(n_{a_{i+1}}(s_t)+\mathds{1}_{a_{i+1}<a}\right)}{2}\right\rfloor,\quad 1\leq i< |\cal A|,
%         \end{align}
% %        \end{small}
%         where $a$ is the action of the highest number of votes, and $a_{i+1}$ is the action of the $(i+1)$-th highest number of votes, \ie, $n_a(s_t)\geq n_{a_2}(s_t)\geq \cdots \geq n_{a_{|\cal A|}}(s_t)$; wherever $n_{a_j}(s_t) = n_{a_l}(s_t)$, $a_j < a_l$.
% \end{theorem}


% \fan{tree search algorithm description (almost the same as CROP, just that in CROP the expansion is guided by the certified radius $r$, here, the expansion is guided by the certified poison size $K$.}


% \subsection{\rlalgotmp: \rlalgotmpfullname}


% \subsubsection{\rlalgotmp: Partition Aggregation with Temporal Aggregation}

%     In sequential decision making process such as RL tasks, it is quite likely that a bad action choice in some certain time step severly hurts the overall performance, say, the cumulative reward.
%     For example, in the Pong game, we may lose the round when choosing an immediate bad action when the ball is closely approaching the pad.
%     Thus, to improve the overall certified robustness, we need to focus on improving the tolerated poison threshold of these ``bottleneck'' time steps.
%     Given \Cref{thm:radius}, the tolerated poison threshold is proportional to the margin between the top-voted action's votes and the runner-up actions' votes.
%     Therefore, we need to enlarge the margin of votes for these bottleneck time steps.
    
%     We observe that, in many reinforcement learning scenarios, the states across adjacent time steps are similar. 
%     For example, they are usually adjacent frames in a game.
%     Thus, we can expect the same optimal action across these time steps.
%     As a result, we aggregate the model votes across adjacent time steps to make the action prediction for this time step.
%     In this way, for a bottleneck time step where the vote margin is small, we can enlarge such margin with the help of large margins from adjacent non-bottleneck time steps.
%     We call this strategy \emph{temporal aggregation}.
    
%     Concretely, we consider a window size $W$ as the time span for temporal aggregation. 
% %    let the window size $W$ be a predetermined hyper-parameter.
%     Suppose the current time step is $t$, and the encountered state at time step $t$ is $s_t$.
%     Similarly to eq.~\ref{eq:cnt} and eq.~\ref{eq:agg}, we then define the \textit{temporal aggregated action count} $n_a^{W}$ and the \textit{temporal aggregated \rlalgotmp policy} $\pi_{\gM_W}$ as follows:
%     \begin{align}
%         n_a^{W}(s_t) &:= \sum_{j=0}^{\min\{W-1,t\}} \left| \{ i \in \{0,\dots,u-1\} \, | \, \pi_i(s_{t-j}) = a \}\right|,\quad \forall a\in\gA,\\
%         \pi_{\gM_W}(s_t) &:= \argmax_{a\in \gA} n_a^{W}(s_t).
%     \end{align}
    
    


% \subsubsection{Certification w.r.t. Per-State Action for \rlalgotmp}

% % \fan{Do we need to separately put \textit{fixed window size} and \textit{flexible window size} to two subsections, or merge them? 

% % Reason for separating: the aggregation protocol and certification are very different; 

% % Reason for putting together: both fall into temporal aggregation.}

% %    and our \rlalgo chooses $\pi_{\gM}(s) := \argmax_{a\in \gA} n_a^{t,W}(s)$.
    
%     A straightforward generalization of \Cref{thm:radius} yields:
%     \begin{lemma}
%     	\label{lem:temporal-agg}
%         Let $\gM_W$ be the algorithm \rlalgotmp and $\pi_{\gM_W}=\gM_W(D)$ be the policy learned via $\gM$ on the clean dataset $D$, where $W$ denotes the window size for temporal aggregation.
% %        Suppose the inference protocol leverages temporal aggregation with window size $W$.
%         For a given state $s_t$ encountered at time step $t$, let $a := \pi_{\gM_W}(s_t)$ and  $<$ be the ``smaller-than'' operator defined on the action set as described in~\Cref{sec:dpa},
% %        the robust poison size is larger or equal to $\rho_t$, where
%         \begin{equation}
%             I_t := \Big\lfloor
%                 \dfrac{ n_a^{W}(s_t) - \max_{a'\neq a}(n_{a'}^{W}(s_t) + \mathds{1}_{a'<a}) } {2 \cdot \min\{W,t+1\} }.
%             \Big\rfloor
%         \end{equation}
%         Then, $I_t$ is a lower bound of the robust poison size $\wbar K(s_t)$ defined in~\Cref{def:per-state}.
%     \end{lemma}

% 	\fan{TODO: update the theorem for the tighter lower bound}
	
% 	\fan{TODO: update the text description for the certification strategy based on~\Cref{alg:PTA-RL-fixed}}
	
	
% 	\input{algos-PTA-RL-fixed}
    
% 	Intuitively, $n_a^{t,W}(s)$ is the accumulative votes across the last $W$ time steps for action $a$, given the trajectory $(s_{t-W}, \cdots, s_t)$.
% 	Suppose time step $t$ is a bottleneck time step where the vote margin between chosen action and runner-up action is just $1$.
% 	But for other recent time steps, the margin is $5$ on average.
% 	Then, without temporal aggregation, we cannot certify robustness~($\rho_t = 0$ according to \Cref{thm:radius});
% 	now, with temporal aggregation, as long as the time window $W > 4$, we can certify robust radius $\rho_t = 2$ according to \Cref{lem:temporal-agg}. 
	
	
% \subsubsection{Certification w.r.t. Cumulative Reward for \rlalgotmp}


% \subsection{\rlalgodyntmp: \rlalgodyntmpfullname}

%     \subsubsection{\rlalgodyntmp: Partition Aggregation with Dynamic Temporal Aggregation}

% 	Since the specification of the window size $W$ requires certain prior knowledge, plus that the same fixed window size $W$ may not be suitable for all time steps, it is preferable to use a flexible window size $W_t$ for each time step $t$. 
% 	Following the idea of enlarging the margin by aggregating over a window rather than merely the current step, an intuitive extension for dynamically determining the window size would be choosing the $W_t$ that leads to the largest margin.
% 	We next present the formulation of the dynamic strategy.
    
%     Basically, at each time step, for each window size $W\in\{1,\ldots,W_{\rm max}\}$, we can compute the temporal aggregated action count $n_a^{W}$ for each action $a \in \gA$. 
%     Let $\Delta^W$ denote the margin between the votes of the best action $a^1$ and the runner-up action $a^2$ at window size $W$, 
%     we would then choose the window size $W_t$ that gives the largest margin, \ie,
%     \begin{align}
% 	    \Delta^W_t &:= n_{a^1}^{W}(s_t) - n_{a^2}^{W}(s_t),\quad \forall W\in\{1,\ldots,W_{\rm max}\},\\
% 	    W_t &:= \argmax_{W} \Delta^W.
%     \end{align}


%     \subsubsection{Certification w.r.t. Per-State Action for \rlalgodyntmp}
%     \begin{theorem}
		
% 	\end{theorem}

% 	\input{algos-PTA-RL-flex}
	

    
%     \subsubsection{Certification w.r.t. Cumulative Reward for \rlalgodyntmp}
    
% }
   
\vspace{-2mm} 
\section{Experiments}
\vspace{-2mm}
\label{sec:exp}
\looseness=-1
In this section, we present the evaluation for our \sysname framework, specifically, 
% the partition-based training protocol (\Cref{subsec:training-protocol}), 
the aggregation protocols (\Cref{subsec:agg-protocol}) and the certification methods under different certification criteria (\Cref{subsec:cert-radius,subsec:cert-reward}). 
% We first describe the experimental procedure, followed by certification for per-state action stability in~\Cref{subsec:eval-action} and cumulative reward in~\Cref{subsec:eval-reward}. 
We defer the description of the offline RL algorithms (DQN~\citep{mnih2013playing}, QR-DQN~\citep{dabney2018distributional}, and C51~\citep{bellemare2017distributional}) used for training the subpolicies to~\Cref{adxsubsec:rl-algos}, and the 
concrete experimental procedures  to~\Cref{adxsubsec:exp-proc}.
% we present the evaluation for the certification of per-state action stability here in~\Cref{subsec:eval-action} and cumulative reward in~\Cref{subsec:eval-reward}.}
% In each part, we provide comparisons on multiple levels: 1) the RL algorithm $\gM_0$, 2) the aggregation protocol, 3) the partition number $u$, and 4) different games.
As a summary, we obtain similar conclusions from per-state action certification and  reward certification:
1) QR-DQN and C51 are oftentimes more certifiably robust than DQN; 
% \chejian{In Highway, C51 $>$ DQN $>$ QR-DQN.}
2) temporal aggregation (\rlalgotmp and \rlalgodyntmp) achieves higher certification for environments satisfying  temporal continuity, \eg, Freeway;
3) larger partition number improves the certified robustness;
4) Freeway is the most stable and robust \env among the three.
More interesting discussions are deferred to~\Cref{adxsec:exp-results}.


\vspace{-2mm}
\subsection{Evaluation of Robustness Certification for Per-State Action Stability}
\label{subsec:eval-action}
\vspace{-2mm}

We provide the robustness certification for per-state action stability based on~\Cref{subsec:cert-radius}.

\textbf{Experimental Setup and Metrics.}\quad
We evaluate the aggregated policies $\rlalgopolicy$, $\rlalgotmppolicy$, and $\rlalgodyntmppolicy$ following \Cref{subsec:agg-protocol}.
% ~\Cref{thm:ppa-radius},~\Cref{thm:tpa-radius} and~\Cref{thm:dtpa-radius}.
Basically, in each run, we run one trajectory (of maximum length $H$) using the derived policy, and
compute $\wbar K_t$ at each time step $t$.
Given $\{\wbar K_t\}_{t=0}^{H-1}$, we obtain a cumulative histogram---for each threshold $\wbar K$, we count the time steps that achieve a threshold no smaller than it and then normalize,
% the counts by the time horizon,
\ie, $\nicefrac{\sum_{t=0}^{H-1} \1 [\wbar K_t \geq \wbar K]}{H}$.
We call this quantity \textit{stability ratio} since it reflects the per-state action stability w.r.t. given poisoning thresholds.
We also compute an \textit{average tolerable poisoning thresholds} for a trajectory, defined as $\nicefrac{\sum_{t=0}^{H-1} \wbar K_t}{H}$.
More details are deferred to~\Cref{adxsubsec:exp-proc}.





% \input{fig_desc/fig_action}

% \input{fig_desc/fig_action_half}

% \input{fig_desc/fig_action_half_cum}
\input{fig_desc/fig_action_half_cum_50}


% \input{fig_desc/fig_action_50}

% \input{fig_desc/fig_freeway_action}
% \input{fig_desc/fig_breakout_action}

\looseness=-1
\textbf{Evaluation Results.}\quad
We present the comparison of per-state action certification for different RL methods and certification methods in~\Cref{fig:statewise}.
% For clear presentation, 
We plot partial poisoning thresholds on the $x$-axes here, and omit full results in~\Cref{adxsubsec:full-action}, where we also 
% cover results for 
report
the average tolerable poisoning thresholds.
We additionally report benign empirical reward and the comparisons with standard training in~\Cref{adxsubsec:emp-reward,adxsubsec:cmp-training}, as well as more analytical statistics in~\Cref{adxsubsec:stat-dparl,adxsubsec:cmp-traj-num}.
% In the Appendix, we additionally report benign empirical reward in~\ref{adxsubsec:emp-reward} {\color{blue} and compare with standard training in~\ref{adxsubsec:cmp-training}.
% We include more analytical statistics for \rlalgodyntmp in~\ref{adxsubsec:stat-dparl}, and report the maximum tolerable poisoning threshold vs. the total number of trajectories in~\ref{adxsubsec:cmp-traj-num}.
% % , as well as a comparison between \sysname with standard training in~\Cref{adxsubsec:cmp-training}.
% }

The cumulative histograms in~\Cref{fig:statewise} can be compared in different levels.
% both the \textit{aggregation protocol} level and the \textit{RL algorithm} level.
Basically, we compare the \textit{stability ratio} at each tolerable poisoning thresholds $\wbar K$---\textit{higher ratio at larger poisoning size indicates stronger certified robustness}.
On the \textbf{RL algorithm} level, 
% we see that 
QR-DQN and C51 consistently outperform the baseline DQN, and C51 has a substantial advantage  particularly in Highway.
% \chejian{C51 algorithm is clearly better than DQN and QR-DQN.}
On the \textbf{aggregation protocol} level, we observe different behaviors in different environments.
On Freeway, methods with temporal aggregation (\rlalgotmp and \rlalgodyntmp) achieve higher robustness, and \rlalgodyntmp achieves the highest certified robustness in most cases;
while on Breakout and Highway, the single-step aggregation \rlalgo is oftentimes better.
This difference is due to the different properties of environments.
Our temporal aggregation is developed based on the assumption of consistent action selection in adjacent time steps. This assumption is true in Freeway while violated in Breakout and Highway.
A more detailed explanation of environment properties is omitted to~\Cref{adxsubsec:cmp-games}.
On the \textbf{partition number} level, a larger partition number generally allows larger tolerable poisoning thresholds as shown in~\Cref{adxsubsec:full-action}.
% \chejianm{according to~\Cref{fig:statewise-full} and~\Cref{fig:statewise-full-highway}}.
Finally, on the \textbf{RL environment} level, Freeway achieves much higher certified robustness for per-state action stability than Highway, followed by Breakout, implying that Freeway is an environment that accommodates more stable and robust policies.

\vspace{-2mm}
\subsection{Evaluation of Robustness Certification for Cumulative Reward Bound}
\label{subsec:eval-reward}
\vspace{-2mm}

We provide the robustness certification for cumulative reward bound according  to~\Cref{subsec:cert-reward}.

\looseness=-1
\textbf{Experimental Setup and Metrics.}\quad
We evaluate the aggregated policies $\rlalgopolicy$, $\rlalgotmppolicy$, and $\rlalgodyntmppolicy$ following~\Cref{thm:action-set-ppa},~\Cref{thm:action-set-tpa} and~\Cref{thm:action-set-dtpa}.
We compute the lower bounds of the cumulative reward $\uj_K$ w.r.t. the poisoning size $K$ using the \adasearch algorithm introduced in~\Cref{subsec:cert-reward}.
We provide details of the evaluated trajectory length along with the rationales in~\Cref{adxsubsec:exp-proc}.
% \m{For Atari games,}
% we adopt the trajectory length $H=400$ for evaluating Freeway and $H=75$ for  Breakout.
% \m{We explain the rationale for the configuration of trajectory length in~\Cref{adxsubsec:exp-proc}.}
% To achieve determinism in the game environment, we use the environment version that entails deterministic transition and reward; we also fix the start state $s_0$ in all runs.

% \input{fig_desc/fig_reward}

\input{fig_desc/fig_reward_main}

\textbf{Evaluation Results.}\quad
We present the comparison of reward certification for different RL algorithms and certification methods in~\Cref{fig:reward}.
Essentially, at each poisoning size $K$, we compare the lower bound of cumulative reward achieved by different RL algorithms and certification methods---\textit{higher value of the lower bound implies stronger certified robustness}.
% We next provide detailed discussions on multiple levels.
On the \textbf{RL algorithm} level, QR-DQN and C51 almost invariably outperform the baseline DQN algorithm.
% QR-DQN and DQN can achieve higher rewards than C51 when poisoning size is small}.
On the \textbf{aggregation protocol} level, methods with temporal aggregation consistently surpass the single-step aggregation \rlalgo on Freeway but not the other two, as analyzed in~\Cref{subsec:eval-action}.
In addition, we note that  \rlalgodyntmp is sometimes not as robust as \rlalgotmp.
We hypothesize two reasons: 1) the dynamic mechanism is more susceptible to the attack, \eg, the selected optimal window size is prone to be manipulated; 2) the lower bound is looser for \rlalgodyntmp given the difficulty of computing the possible action set in \rlalgodyntmp (discussed in~\Cref{thm:action-set-dtpa}).
On the \textbf{partition number} level, a larger partition number ($u=50$) demonstrates higher robustness.
On the \textbf{horizon length} level, the robustness ranking of different policies is similar under different horizon lengths with slight differences, corresponding to the property of finite-horizon RL.
On the \textbf{RL environment} level, Freeway can tolerate a larger poisoning size than Breakout and Highway.
% , implying that Freeway accommodates more robust policies than Breakout.
More results and discussions are in~\Cref{adxsubsec:full-reward}.

% \input{fig_desc/fig_freeway_reward}

% \input{fig_desc/fig_breakout_reward}

% \input{fig_desc/fig_freeway_reward_tight}

% \input{fig_desc/fig_breakout_reward_tight}

%\subsubsection*{Author Contributions}
%If you'd like to, you may include  a section for author contributions as is done
%in many journals. This is optional and at the discretion of the authors.
%
%\subsubsection*{Acknowledgments}
%Use unnumbered third level headings for the acknowledgments. All
%acknowledgments, including those to funding agencies, go at the end of the paper.




\vspace{-2mm}
\section{Conclusions}
\vspace{-2mm}

    In this paper, we proposed \textbf{\sysname}, the first framework for certifying robust policies for offline RL against poisoning attacks.
    \sysname includes three policy aggregation protocols.
    % : \rlalgo, \rlalgotmp, and \rlalgodyntmp.
    For each aggregation protocol, \sysname provides a sound certification for both per-state action stability and cumulative reward bound.
    Experimental evaluations on different environments and different offline RL training algorithms show the effectiveness of our robustness certification in a wide range of scenarios.


\subsubsection*{Acknowledgments}
    This work is partially supported by the NSF grant No.1910100, NSF CNS 20-46726 CAR, Alfred P. Sloan Fellowship, the U.S. Department of Energy by the Lawrence Livermore National Laboratory under Contract No. DE-AC52-07NA27344 and LLNL LDRD Program Project No. 20-ER-014, and Amazon Research Award.

\textbf{Ethics Statement.}\quad
In this paper, we prove the first framework for certifying robust policies for offline RL against poisoning attacks.
On the one hand, such framework provides rigorous guarantees in practice RL tasks and thus significantly alleviates the security vulnerabilities of offline RL algorithms against training-phase poisoning attacks.
The evaluation of different RL algorithms also provides a better understanding about the different degrees of security vulnerabilities across different RL algorithms. 
On the other hand, the robustness guarantee provided by our framework only holds under specific conditions of the attack.
Specifically, we require the attack to change only a bounded number of training trajectories.
Therefore, users should be aware of such limitations of our framework, and should not blindly trust the robustness guarantee when the attack can change a large number of training instances or modify the training algorithm itself.
As a result, we encourage researchers to understand the potential risks, and evaluate whether our constraints on the attack align with their usage scenarios when applying our \sysname to real-world applications.
We do not expect any ethics issues raised by our work.

\textbf{Reproducibility Statement.}\quad
All theorem statements are substantiated with rigorous proofs in \Cref{adxsec:proofs}.
In \Cref{adxsec:alg}, we list the pseudocode for all key algorithms.
Our experimental evaluation is conducted with publicly available OpenAI Gym toolkit~\citep{brockman2016openai}.
We introduce all experimental details in both \Cref{sec:exp} and \Cref{adxsec:exp}.
Specifically, we build the code upon the open-source code base of \citet{agarwal2020optimistic}, and we upload the source code at \url{https://github.com/AI-secure/COPA} for reproducibility purpose.


\bibliography{iclr2022_conference}
\bibliographystyle{iclr2022_conference}

\appendix
\newpage

\section{Omitted Definitions}
    \label{adxsec:protocol}
    
    \subsection{Cumulative Reward}
    
        \begin{definition}[Cumulative Reward]
            \label{def:cum-reward}
            Let $P: \cal S \times \cal A \rightarrow \cal P(\cal S)$ be the transition function  with $\cal P(\cdot)$ defining the set of probability measures.  
            % Let $\Gamma:\cal S\times \cal A\rightarrow \cal S$ be the transition function, 
            Let $R,d_0,H$ be the reward function, initial state distribution, and time horizon.
            % Suppose each state trajectory contains at most $H$ time steps, and 
            We denote $J(\pi)$  as the \emph{cumulative reward} of the given policy $\pi$:
            \begin{small}
            \begin{equation}
                \label{eq:cum-reward}
                J(\pi)  := \E \sum_{t=0}^{H-1} R(s_t, a_t),
                \text{ where } a_t=\pi(s_t),s_{t+1}\sim P(s_t,a_t),s_0\sim d_0,
            \end{equation}
            \end{small}
        \end{definition}
    
        % The definition sums up the reward across all $H$ steps to get the cumulative reward.
        It is natural to adapt this definition when there is a discount factor.
        If policy $\pi$ considers recent $n_t$ states instead of only $s_t$ to make action predictions, we can change $a_t = \pi(s_t)$ to $a_t = \pi(s_{t-n_t+1 : t})$ in \Cref{eq:cum-reward}.

    \subsection{\rlalgo~(\rlalgofullname) Protocol}
    
        \begin{definition}[\rlalgofullname]
            Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$,
            the \rlalgofullname~(\rlalgo) protocol defines an aggregated policy $\rlalgopolicy: \gS \to \gA$ such that
            \begin{small}
            \begin{equation}
                \rlalgopolicy(s) := \argmax_{a\in \gA} n_a(s),
                \label{eq:ppa-agg}
            \end{equation}
            \end{small}
            where $n_a(s)$ is defined in \Cref{subsec:notation}.
            \label{def:ppa-agg}
        \end{definition}
        As mentioned in \Cref{sec:main}, when the $\argmax$ in \Cref{eq:ppa-agg} returns multiple elements, we break ties deterministically by returning the ``smaller'' ($<$) action, which can be defined by numerical order, lexicographical order, etc.
        % Hereinafter, we assume $\argmax$ over $\gA$ always uses $<$ operator to break ties.

    \subsection{\rlalgotmp~(\rlalgotmpfullname) Protocol}
    
        \begin{definition}[\rlalgotmpfullname]
            Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and window size $W$,
            at time step $t$,
            the \rlalgotmpfullname~(\rlalgotmp) defines an aggregated policy $\rlalgotmppolicy: \gS^{\min\{t + 1, W\}} \to \gA$ such that
            \begin{small}
            \begin{equation}
                \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t}) 
                % := \argmax_{a\in \gA} \sum_{j=\max\{t-W+1,0\}}^t n_a(s_j) 
                = \argmax_{a\in \gA} n_a(s_{\max\{t-W+1,0\}:t}),
                \label{eq:tpa-agg}
            \end{equation}
            \end{small}
            where $s_{l:r}$ and $n_a$ are defined in~\Cref{subsec:notation}. 
            \label{def:tpa-agg}
        \end{definition}
        
        In the above definition, at time step $t$, the input of policy $\rlalgotmppolicy$ contains all states between time step $\max\{t-W+1,0\}$ and $t$ within window size $W$; and the output is the policy prediction with the highest votes across these states.
        Recall that in \Cref{subsec:notation}, we define $n_a(s_{l:r}) = \sum_{j=l}^r n_a(s_j)$.
        We break ties in the same way as in \rlalgo.


\section{Illustration of \sysname Aggregation Protocols}
    \label{adxsec:running-example}
    
    \begin{table}[h]
        \centering
        \caption{\small A concrete example of action predictions, where ``1'' means action $a_1$ and ``2'' means action $a_2$. 
        When there is no poisoning attack, the corresponding time window spans by \rlalgo, \rlalgotmp, and \rlalgodyntmp are shown by \colorbox{green!25}{green}, \colorbox{blue!25}{blue}, and \colorbox{pink!25}{pink} respectively. All aggregated policies choose action $a_1$, but have different tolerable poisoning thresholds as shown in the last column.}
        \begin{tabular}{c|cccccccc|c}
            \toprule
            Action Prediction for & $s_0$ & $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ & $s_7$ & $\wbar K$ at $s_7$ \\
            \midrule
            $\pi_0$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
            $\pi_1$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
            $\pi_2$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
            $\pi_3$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 2 \\
            $\pi_4$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 2 \\
            $\pi_5$ & 1 & 1 & 1 & 2 & 1 & 2 & 2 & 2 \\
            \hline\hline
            \rlalgo~($\rlalgopolicy$, \Cref{def:ppa-agg}) & & & & & & & & \multicolumn{1}{|c|}{\cellcolor{green!25} 1} & $0$ \\
            \cline{3-9}
            \rlalgotmp with $W=7$~($\rlalgotmppolicy$, \Cref{def:tpa-agg}) & & \multicolumn{6}{|c}{\cellcolor{blue!25}} &
            \multicolumn{1}{c|}{\cellcolor{blue!25} 1} & $2$ \\
            \cline{2-9}
            \rlalgodyntmp with $W_{\max}=8$~($\rlalgodyntmppolicy$, \Cref{def:dtpa-agg}) & \multicolumn{7}{c}{\cellcolor{pink!25}} &
            \multicolumn{1}{c|}{\cellcolor{pink!25} 1} &
            $1$ \\
            \bottomrule
        \end{tabular}
        \label{tab:adx-example}
    \end{table}
    
    % We use a concrete example to illustrate the three aggregation protocols and their pre-state action tolerable poisoning thresholds respectively.
    % We use a concrete example to illustrate bottleneck states and non-bottleneck states, and demonstrate how different aggregation protocols induce different tolerable poisoning thresholds.
    We present a concrete example to demonstrate how different aggregation protocols induce different tolerable poisoning thresholds, illustrate bottleneck and non-bottleneck states, and provide additional discussions.

    Suppose the action space contains two actions $\gA = \{a_1, a_2\}$, and there are six subpolicies $\{\pi_i\}_{i=0}^{u-1}$ where $u=6$.
    We are at time step $t = 7$ now.
    When there is no poisoning, the subpolicies' action predictions for state $s_0$ to $s_7$ are shown by \Cref{tab:adx-example}.
    After aggregation, all aggregated policies will choose action $a_1$ at $t=7$.
    
    
    \paragraph{\rlalgo~(\Cref{def:ppa-agg}).}
    The \rlalgo aggregation protocol only uses the current state $s_7$ to aggregate the votes.
    On $s_7$, three subpolicies choose action $a_1$ and three others choose action $a_2$.
    By breaking the tie with $a_1 < a_2$, the \rlalgo policy $\rlalgopolicy(s_7)=a_1$.
    The tolerable poisoning threshold $\wbar K_t = 0$, because one action flipping from $a_1$ to $a_2$ by poisoning only one subpolicy can change the aggregated policy to $a_2$.
    
    \paragraph{\rlalgotmp~(\Cref{def:tpa-agg}).}
    The \rlalgotmp aggregation protocol uses window size $W=7$.
    This implies that, we aggregate all states $s_{1:7}$ to count the votes and decide the action.
    Since $n_{a_1}(s_{1:7}) = 36$ and $n_{a_2}(s_{1:7}) = 6$,
    after poisoning two subpolicies, we still $\wtilde n_{a_1}(s_{1:7}) \ge \wtilde n_{a_2}(s_{1:7})$.
    Thus, we achieve an tolerable poisoning threshold $\wbar K_t = 2$.
    
    Compared with \rlalgo, the temporal aggregation in \rlalgotmp increases the vote margin between $a_1$ and $a_2$ and thus improve the tolerable poisoning threshold at current state.
    
    \paragraph{\rlalgodyntmp~(\Cref{def:dtpa-agg}).}
    The \rlalgodyntmp aggregation protocol chooses the window size $W'=8$ since this window size gives the largest average vote margin $\Delta_t^{W'}$~(defined in \Cref{eq:dtpa-agg-1}).
    We can easily find out that with poisoning size $K=1$, we will still choose $\wtilde W'=8$ as the window size and the resulting votes for $a_1$ can be kept higher than votes for $a_2$.
    However, when it comes to $K=2$, if we totally flip subpolicies $\pi_0$ and $\pi_1$ to let them always predict action $a_2$, then the \rlalgodyntmp aggregated policy will turn to choose $W'=1$ as the window size and then choose action $a_2$ as the action output.
    Thus, we achieve a tolerable poisoning threshold $\wbar K_t = 1$ this time.
    
    
    \paragraph{Illustrations of Bottleneck and Non-Bottleneck States.}
    According to our illustration in \Cref{subsec:agg-protocol}, bottleneck states are those where subpolicies vote for diverse actions but the best action is the same as previous states, and non-bottleneck states are those where subpolicies mostly vote for the same action.
    As we can see, $s_0$ to $s_6$ are non-bottleneck states since the subpolicies almost unanimously vote for one action.
    In contrast, $s_7$ is a bottleneck state.

    From the perspectives of different \textit{aggregation protocols}, we observe that for the bottleneck state $s_7$, both \rlalgotmp and \rlalgodyntmp exploit temporal aggregation to boost the certified robust poisoning threshold~(from $0$ to $2$ and from $0$ to $1$ respectively), thus demonstrating the effectiveness of \rlalgotmp and \rlalgodyntmp on improving certified robustness.
    On the other hand, for non-bottleneck states $s_0$ to $s_6$, we can easily see that different aggregation protocols do not differ much in terms of provided certified robustness levels.

    \paragraph{Explanations for Bottleneck and Non-Bottleneck States.}
    We provide additional discussions regarding \textit{why bottleneck states are vulnerable} and \textit{why our temporal aggregation strategy can effectively alleviate the problem}. We first explain the existence of the bottleneck states. Given the property of the bottleneck states that there is high disagreement among different subpolicies on such states, they may lie close to the decision boundary. This may be a result of poisoning, or simply due to the intrinsic difficulty of the state. On the other hand, such states naturally exist in the rollouts (like natural adversarial examples~\citep{hendrycks2021natural}), and may induce high instability of the rollouts during testing. We next discuss additional intuitions for our temporal aggregation. Essentially, temporal aggregation effectively leverages the adjacent non-bottleneck states to rectify the decisions at the bottleneck states, based on the assumption of temporal continuity which has been revealed and utilized in several previous works~\citep{legenstein2010reinforcement,veerapaneni2020entity,ye2021mastering}.
    
\section{Certification of Per-State Action Stability for \rlalgo}

    \label{adxsec:ppa-per-state}
    
        We certify the robustness of \rlalgo following \Cref{thm:ppa-radius}.
        \begin{theorem}
        	\label{thm:ppa-radius}
        	Let $D$ be the clean  training dataset; let $\pi_i = \gM_0(D_i), 0\le i \le u-1$ be the learned subpolicies according to \Cref{subsec:training-protocol} from which we define $n_a$~(see \Cref{subsec:notation});
        	and let $\rlalgopolicy$ be the \rlalgofullname policy: $\rlalgopolicy = \gM(D)$ where $\gM$ abstracts the whole training-aggregation process.
        	$\wtilde D$ is a poisoned dataset and $\wtilde \rlalgopolicy$ is the poisoned policy: $\wtilde \rlalgopolicy = \gM(\wtilde D)$.
        	
        	For a given state $s_t$ encountered at time step $t$ during test time, let $a := \rlalgopolicy(s_t)$, then
        	\begin{small}
        	\begin{equation}
        	    \wbar K_t = \left\lfloor\frac{n_{a}(s_t)-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}(s_t)+\1[a^{\prime}<a]\right)}{2}\right\rfloor.
        	    \label{eq:ppa-radius} \small
        	\end{equation}
        	\end{small}
        % 	is a \emph{tolerable poisoning threshold} at time step $t$ in \Cref{def:per-state}.
            	
            % 	Let $\cal M$ be the algorithm \rlalgo and $\mpi = \cal M(D)$ be the policy learned via $\cal M$ on the clean dataset $D$.
            % %	$\tpi$ be the policy output by . 
            % 	For a given state $s_t$ encountered at time step $t$ during test time, let $a := \mpi(s_t)$, $<$ be the ``smaller-than'' operator defined on the action set as described in~\Cref{sec:dpa},
            % 	\begin{align}
            % 		I_t :=\left\lfloor\frac{n_{a}(s_t)-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}(s_t)+\mathds{1}_{a^{\prime}<a}\right)}{2}\right\rfloor.
            % 	\end{align}
            % 	Then, $I_t$ is a lower bound of the robust poison threshold $\wbar K(s_t)$ defined in~\Cref{def:per-state}, meaning that for any poisoned training set $\wtilde D$, as long as $| D \ominus \wtilde D| \leq I_t$, the action prediction given by the clean policy $\mpi = \cal M(D)$ and the poisoned policy $\tmpi = \cal M(\wtilde D)$ will be the same on the given state $s_t$, \ie, $\mpi(s_t)=\tmpi(s_t)$.
        \end{theorem}
        
        \begin{remark}
            The theorem provides a valid per-state action certification for \rlalgo,
            since according to \Cref{def:per-state}, as long as the poisoning size is smaller or equal to $\wbar K_t$, \ie, $| D \ominus \wtilde D | \le \wbar K_t$, the action of the poisoned policy is the same as the clean policy: $\wtilde \rlalgopolicy(s_t) = \rlalgopolicy(s_t) = a$.
            To compute $\wbar K_t$, according to \Cref{eq:ppa-radius}, we rely on the aggregated action count $n_a$ for state $s_t$ from subpolicies.
            The $a' < a$ is the ``smaller-than'' operator introduced following \Cref{def:ppa-agg}.
        \end{remark}
        
        \begin{proof}[Proof of \Cref{thm:ppa-radius}.]
            % According to \citep{levine2021deep},
            Suppose the poisoning size is within $K$, then after poisoning, the aggregated action count $\wtilde n_a(s_t) \in [n_a(s_t) - K, n_a(s_t) + K]$ where $n_a(s_t)$ is such count before poisoning.
            Thus, to ensure the chosen action does not change, a necessary condition is that $\wtilde n_a(s_t) \ge \wtilde n_{a'}(s_t) + \1[a' < a]$ for any other $a' < a$.
            Solving $K$ yields \Cref{eq:ppa-radius}.
        \end{proof}
        
        We use the theorem to compute the per-state action certification for each time step $t$ along the trajectory, and the detailed algorithm  is in \Cref{alg:ppa-radius}~(\Cref{adxsec:alg}).
        Furthermore, we prove that this certification is theoretically tight as the following proposition shows. The proof is in \Cref{adxsubsec:proof-C1}.
        
        \looseness=-1
        \begin{proposition}
            Under the same condition as \Cref{thm:ppa-radius}, for any time step $t$, there exists an RL learning algorithm $\gM_0$, and a poisoned dataset $\wtilde D$, such that $|D \ominus \wtilde D| = \wbar K_t + 1$, and $\wtilde \rlalgopolicy (s_t) \neq \rlalgopolicy(s_t)$.
            \label{prop:ppa-radius-tightness}
        \end{proposition}


\section{A Table of Possible Action Set}

    % \label{adxsec:cumulative-reward}
        
        % \vspace{-2mm}
        
        
        \begin{table}[h]
            \centering
            \caption{\small Expressions of possible action set $A(K)$ given poisoning threshold $K$ for different aggregation protocols.
            Full theorem statements are in \Cref{thm:action-set-ppa,thm:action-set-tpa,thm:action-set-dtpa}~(in \Cref{subsec:cert-reward}).}
            \vspace{-1em}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{c|c}
                \hline
                Protocol & $A(K)$ \\
                \hline
                \rlalgo & $\left\{
                    a \in \gA 
                    \,\Big\lvert\,
                    \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a'<a], 0\} \le K
                \right\}$ \\
                % \hline
                \rlalgotmp & $\left\{ a \in \gA 
                    \,\Big\lvert\,
                    \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
                \right\}$ \\
                % \hline
                \rlalgodyntmp & $ \displaystyle
                % \begin{aligned}
                    \{a_t\} \cup 
                    \left\{ 
                    a' \in \gA
                    \,\Big\lvert\,
                        \min_{1\le W^*\le \min\{W_{\max}, t+1\}, W^* \neq W', a''\neq a_t} L_{a',a''}^{W^*,W'} \le K
                    \right\} %\\
                    \cup
                    \left\{
                    a \in \gA
                    \,\Big\lvert\,
                        \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
                    \right\}
                % \end{aligned}
                $ \\
                \bottomrule
            \end{tabular}
            }
            \label{tab:AK-expressions}
        \end{table}
        
        For all three aggregation protocols, we summarize the expressions used for computing the possible action set $A(K)$ given tolerable poisoning threshold $K$ in \Cref{tab:AK-expressions}.
        
        % In this section, we present our robustness certification methods for \textit{cumulative reward bound}.
        % We assume that the RL environment is deterministic throughout the cumulative reward certification for convenience, \ie, the transition function is $P: \gS \times \gA \to \gS$
        % % instead of $P: \gS \times \gA \to \gP(\gS)$ 
        % and the initial state is a fixed $s_0 \in \gS$.
        % % rather than $d_0 \in \gP(\gS)$.
        % The certification goal, as listed in \Cref{def:cum-reward}, is to obtain a lower bound of cumulative reward under  poisoning attacks, as long as the poisoning size is within $K$.
        % Our cumulative reward certification is based on a novel adaptive tree search algorithm \adasearch.
        
        % \paragraph{\adasearch Algorithm Description.}
        % The pseudocode is in \Cref{alg:tree-search}~(\Cref{adxsubsec:alg-reward}).
        % The method starts from the base case: when the poisoning threshold $K_{\mathrm{cur}} = 0$, the lower bound of cumulative reward $\uj_{K_{\mathrm{cur}}}$ is exactly the reward without poisoning.
        % The method then gradually increases the poisoning threshold $K_{\mathrm{cur}}$, by finding the immediate larger $K' > K_{\mathrm{cur}}$ that can expand the possible action set along the trajectory.
        % With the increase of $K_{\mathrm{cur}} \gets K'$, the attack may cause the poisoned policy $\tpi$ to take different actions at some states, thus resulting in new trajectories.
        % We need to figure out \emph{a set of all possible actions} to exhaustively traverse all possible trajectories.
        % We will introduce theorems to compute this set of possible actions.
        % With this set, the method effectively explores these new trajectories by formulating them as expanded branches of a trajectory tree.
        % Once all new trajectories are explored, the method examines all leaf nodes of the tree and figures out the minimum reward among them, which is the new lower bound of cumulative reward $\uj_{K'}$ under new poisoning size $K'$.
        % We then repeat this process of increasing poisoning size from $K'$ and expanding with new trajectories until we reach a predefined threshold for poisoning size $K$.

        
        % % As we can see, the core of \adasearch is figuring out the \emph{possible action set}.
        % \begin{definition}[Possible Action Set]
        %     \label{def:possible-action-set}
        %     Given previous states $s_{0:t}$, the subpolicies $\{\pi_i\}_{i=0}^{u-1}$, the aggregation protocol~(\rlalgo, \rlalgotmp, or \rlalgodyntmp), and the poisoning size $K$, the \emph{possible action set} $A$ at step $t$ is a subset of action space: $A \subseteq \gA$, such that for any poisoned policy $\wtilde \pi$, as long as the poisoning size is within $K$, the chosen action at step $t$ will always be in $A$, \ie, $a_t = \wtilde \pi(s_{0:t}) \in A$.
        % \end{definition}
        
        % \paragraph{Possible Action Set for \rlalgo.}
        % The following theorem gives the possible action set for \rlalgo.
        
        % \begin{theorem}[Tight \rlalgo Action Set]
        %     \label{thm:action-set-ppa}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
        %     then the \emph{possible action set} at step $t$
        %     \begin{small}
        %     \begin{equation}
        %         A^T(K) = \left\{
        %             a \in \gA 
        %             \,\Big\lvert\,
        %             \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a'<a], 0\} \le K
        %         \right\}.
        %         \label{eq:action-set-ppa}
        %     \end{equation}
        %     \end{small}
        % \end{theorem}
        
        % \begin{proof}[Proof sketch.]
        %     Within poisoning size $K$, the optimal attack strategy towards making $a \in \gA$  the chosen action is to let some subpolicies flip their action to $a$.
        %     Then the problem is what subpolicies need to be selected to flip.
        %     It turns out to be all subpolicies whose current action $a'$ has votes $\ge n_a(s_t) + K + 1 - \1[a' < a]$, which completes the proof.
        %     Detailed proof is in \Cref{adxsubsec:proof-C61}.
        % \end{proof}
        
        % \begin{remark}
        % In \Cref{adxsubsec:proof-C62} we prove that   \Cref{thm:action-set-ppa} is  theoretically tight in \Cref{thm:compare-tight-loose-action-set-ppa}. In addition, we show that a direct extension of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) can also yield possible action set~(\Cref{cor:loose-action-set-ppa} in \Cref{adxsubsec:proof-C61}), which is loose than \Cref{thm:action-set-ppa} as proved in \Cref{thm:compare-tight-loose-action-set-ppa}.
        % In other words, a theoretically tight possible action set combined with the proposed \adasearch leads to a theoretically tight certification of cumulative reward bound. 
        %     % In \Cref{adxsubsec:proof-C61},
        %     % we show that a direct extension of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) can also yield possible action set~( \Cref{cor:loose-action-set-ppa}), and in \Cref{adxsubsec:proof-C62} we prove \Cref{thm:compare-tight-loose-action-set-ppa} stating that \Cref{thm:action-set-ppa} is tighter than \Cref{cor:loose-action-set-ppa}, and \Cref{thm:action-set-ppa} is also theoretically tight.
        % \end{remark}
        
        % % In contrast, a generalization of \rlalgo's per-state certification~(\Cref{thm:ppa-radius}) yields a loose action set.
        % % \begin{corollary}[Loose \rlalgo Action Set]
        % %     \label{cor:loose-action-set-ppa}
        % %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
        % %     then the \emph{possible action set} at step $t$
        % %     \begin{equation}
        % %         A^L(K) = \left\{
        % %             a \in \gA
        % %             \,\Big\lvert\,
        % %             \max_{a'\in \gA} n_{a'}(s_t) - n_a(s_t) \le 2K - \1[a > \argmax_{a'\in \gA} n_{a'}(s_t)]
        % %         \right\}.
        % %         \label{eq:loose-action-set-ppa}
        % %     \end{equation}
        % % \end{corollary}
        
        % % As the following theorem show, the \Cref{cor:loose-action-set-ppa} is typically looser than \Cref{thm:action-set-ppa}, and indeed \Cref{thm:action-set-ppa} is theoretically tight.
        % % We also compare \Cref{thm:action-set-ppa} and \Cref{cor:loose-action-set-ppa} in practice in \TODO.
        
        % % \begin{theorem}
        % %     \label{thm:compare-tight-loose-action-set-ppa}
        % %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
        % %     $A^T(K), A^L(K)$ are defined according to \Cref{eq:action-set-ppa,eq:loose-action-set-ppa} accordingly, then
        % %     \begin{enumerate}[leftmargin=*]
        % %         \item $A^T(K) \subseteq A^L(K)$; and there are subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$ such that $A^T(K) \subsetneq A^L(K)$.
                
        % %         \item Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$, for any $a \in A^T(K)$, there exists a poisoned training set $\wtilde D$ whose poisoning size $|D \ominus \wtilde D| \le K$ and some RL training mechanism, such that $\wtilde \rlalgopolicy(s_t) = a$ where $\wtilde \rlalgopolicy$ is the poisoned \rlalgo policy trained on $\wtilde D$.
        % %     \end{enumerate}
        % % \end{theorem}
        
        % % We defer the proofs of \Cref{cor:loose-action-set-ppa} and \Cref{thm:compare-tight-loose-action-set-ppa} to \Cref{adxsubsec:proof-C62}.
        
        % % \begin{remark}
        % %     Specifically, the first point in \Cref{thm:compare-tight-loose-action-set-ppa} shows that the certification from \Cref{cor:loose-action-set-ppa} is usually looser than that from \Cref{thm:action-set-ppa}; and the second point shows the theoretical tightness of \Cref{thm:action-set-ppa}.
        % %     Indeed, a theoretically tight possible action set combined with the proposed \adasearch leads to a theoretically tight certification of cumulative reward.
        % % \end{remark}
        
        % \paragraph{Possible Action Set for \rlalgotmp.}
        % The following theorem gives the possible action set for \rlalgotmp.
        % \begin{theorem}
        %     \label{thm:action-set-tpa}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgotmp as defined in \Cref{def:tpa-agg},
        %     then the \emph{possible action set} at step $t$
        %     \begin{small}
        %     \begin{equation}
        %         A(K) = \left\{ a \in \gA 
        %             \,\Big\lvert\,
        %             \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
        %         \right\},
        %         \label{eq:action-set-tpa}
        %     \end{equation}
        %     \end{small}
        %     where $h_{a',a}^{(i)}$ and $\delta_{a',a}$ follow the definition in \Cref{thm:tpa-radius}.
        % \end{theorem}
        
        % \begin{proof}[Proof sketch.]
        %     We first show that any possible action $a$ must be able to be poisoned to achieve higher votes than any other actions $a'$.
        %     Therefore, a necessary condition is that, after applying the greedy selection strategy to shrink the vote margin between $a'$ and $a$, the votes of $a$ is higher than the votes of $a'$, \ie, $\sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}$.
        %     The detailed proof is in \Cref{adxsec:proofs}.
        % \end{proof}
        
        % The possible action set given by \Cref{thm:tpa-radius} is no longer theoretically tight.
        % In other words, there may exist a possible action set with fewer elements than that given by \Cref{eq:action-set-tpa}.
        % Indeed, the problem of computing a possible action set with minimum cardinality for \rlalgotmp is $\NP$-complete.
        
        % \begin{theorem}
        %     \label{thm:np-complete-tpa-action-set}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgotmp as defined in \Cref{def:tpa-agg}, then computing a possible action set $A(K)$ such that any possible action set $S$ satisfies $|A(K)| \le |S|$ is  $\NP$-complete.
        % \end{theorem}
        
        % We prove the theorem by a reduction to set cover problem~\citep{karp1972reducibility}, with proofs in \Cref{adxsec:proofs}.
        
        % \begin{remark}
        %     This theorem shows a counter-intuitive property of \rlalgotmp aggregated policy.
        %     From \Cref{thm:tpa-radius}, \rlalgotmp has a theoretically tight certification of per-state action, which can be computed in $O(|\gA|u(W+\log u))$ time.
        %     From the proof, we can  craft an optimal attack that deviates the chosen action from the clean policy's choice, which can be viewed as untargeted attack.
        %     In contrast, from \Cref{thm:np-complete-tpa-action-set}, \rlalgotmp \emph{cannot} determine whether a particular action $a'$ can be chosen with a poisoning attack unless $\NP = \mathsf{P}$.
        %     This can be viewed as the hardness of targeted attack.
        %     In other words, the optimal \emph{untargeted} attack on \rlalgotmp can be found in polynomial time, while the optimal \emph{targeted} attack on \rlalgotmp is $\NP$-complete, which indicates the robustness property of proposed \rlalgotmp. 
        % \end{remark}
        
        % \paragraph{Possible Action Set for \rlalgodyntmp.}
        % The following theorem gives the possible action set for \rlalgodyntmp.
        % \begin{theorem}
        %     \label{thm:action-set-dtpa}
        %     Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgotmp as defined in \Cref{def:dtpa-agg},
        %     then the \emph{possible action set} at step $t$
        %     \begin{small}
        %     \begin{equation}
        %         \label{eq:action-set-dtpa}
        %         \begin{aligned}
        %             A(K) = \{a_t\} & \cup 
        %             \left\{ 
        %             a' \in \gA
        %             \,\Big\lvert\,
        %                 \min_{1\le W^*\le \min\{W_{\max}, t+1\}, W^* \neq W', a''\neq a_t} L_{a',a''}^{W^*,W'} \le K
        %             \right\} \\
        %             & \cup
        %             \left\{
        %             a \in \gA
        %             \,\Big\lvert\,
        %                 \sum_{i=1}^K h_{a',a}^{(i)} > \delta_{a',a}, \forall a' \neq a
        %             \right\}
        %         \end{aligned}
        %     \end{equation}
        %     \end{small}
        %     where
        %     $a_t = \rlalgodyntmppolicy(s_{\max\{t - W_{\max} + 1,0\}:t})$ is the clean policy's chosen action,
        %     $W'$ is defined by \Cref{eq:dtpa-agg-1},
        %     $L_{a',a''}^{W^*,W'}$ is defined by \Cref{def:L} with $a$ being replaced by $a_t$,
        %     and $h_{a',a}^{(i)}, \delta_{a',a}$ is defined in \Cref{thm:tpa-radius} with $W$ replaced by $W'$.
        % \end{theorem}
        
        % \begin{proof}[Proof sketch.]
        %     The possible action set given by \Cref{eq:action-set-dtpa} is composed of three parts that encode the possible actions:
        %     (1)~the actions chosen by the aggregated policy without poisoning;
        %     (2)~the actions that may be chosen if the poisoning attack shifts the chosen window size;
        %     (3)~the actions that may be chosen if the poisoning attack does not shift the chosen window size.
        %     For each category, we show that the given set includes all possible actions.
        %     A detailed proof is in \Cref{adxsec:proofs}.
        % \end{proof}
        
        % \begin{remark}[Open problem]
        %     For two aggregation protocols~(\rlalgo and \rlalgotmp), we either provide theoretically tight certification or show they are $\NP$-complete.
        %     In contrast,
        %     for the \rlalgodyntmp aggregation protocol,  we only prove the theoretically tight certification for per-state action~(\Cref{thm:dtpa-radius}). For cumulative reward~(via possible action set given by \Cref{thm:action-set-dtpa}) we do not prove its theoretical tightness in polynomial time (in exponential time we can provide theoretically tight certification by enumerating all $|\gA|^{uW_{\max}}$ possible assignments)).
        %     % nor we show whether theoretically tight certification in polynomial time exists~(in exponential time we can have theoretically tight certification by enumerating all $|\gA|^{uW_{\max}}$ possible assignments).
        %     We conjecture that the theoretically tight certification for \rlalgodyntmp is an $\NP$-complete problem, and leave it as an interesting future exploration.
        % \end{remark}
        
        % % \linyi{Deleted the NP-complete statement of cumulative reward certification, since with finite state space, the problem is not NP-complete. It is just the state space is exponentially large for current problems so the reward certification also needs exponential time. I will do a global search to make other parts consistent.}
        
        % % \paragraph{General Hardness of Cumulative Reward Certification.}
        % % To this point, we have introduced the theorems for computing possible action sets for \rlalgo, \rlalgotmp, and \rlalgodyntmp aggregation protocols.
        % % They can be combined with \adasearch to provide robustness certification for cumulative reward.
        % % In the worst case, \adasearch needs to explore a superset of all trajectories of possible poisoned policies, which seems to be costly~(though performs good in practice as shown in \TODO).
        % % One may think that whether more efficient and tighter certification method exists.
        % % However, the following result implies that theoretically tight certification may need inevitably high computational cost.
        % % \begin{theorem}
        % %     \label{thm:general-hardness-reward}
        % %     The problem of computing $\max \uj_K$ defined by \Cref{def:cert-cum-reward} given general deterministic environment $\gE=(\gS, \gA, R, P, H, d_0)$, subpolicies $\{\pi_i\}_{i=0}^{u-1}$, poisoning size $K$, and aggregation protocols belonging to \rlalgo, \rlalgotmp, and \rlalgodyntmp is $\NP$-complete.
        % % \end{theorem}
        
        % % \begin{proof}[Proof sketch.]
        % %     We prove the theorem by encoding the classical \textsf{3-SAT} problem with a sequential decision making environment.
        % %     The detailed proof is in \Cref{adxsec:proofs}.
        % % \end{proof}



\section{Algorithm Pseudocode and Discussion}

    \label{adxsec:alg}
    
    \subsection{\sysname Training Protocol}
    \label{adxsubsec:algo-train}
    
        \input{algos-training}
    
    \subsection{\sysname Per-State Action Certification}
        \label{adxsec:alg-perstate}
        
        \paragraph{\rlalgofullname~(\rlalgo).}\hfill
        
        \input{algos-PPA-radius}
        
        \paragraph{\rlalgotmpfullname~(\rlalgotmp).}\hfill
        
        \input{algos-TPA-radius}
        
        \paragraph{\rlalgodyntmpfullname~(\rlalgodyntmp).}\hfill
        
        \input{algos-DTPA-radius}
    
    \subsection{\sysname Cumulative Reward Certification}
        \label{adxsubsec:alg-reward}
        
        
        \looseness=-1
        \adasearch alternately executes the procedure of \emph{trajectory exploration and expansion} and \emph{poisoning threshold growth}. 
        In trajectory exploration and expansion, \adasearch organizes all possible trajectories in the form of a search tree and progressively grows it. 
        For each node (representing a state), we leverage \Cref{thm:action-set-ppa,thm:action-set-tpa,thm:action-set-dtpa} to compute the Possible Action Set. We then expand the tree branches corresponding to the actions in the derived set. 
        In poisoning threshold growth, when all trajectories for the current poisoning threshold are explored, we increase $K’$ to seek certification under larger poisoning sizes, via maintaining a priority queue of all poisoning sizes during the expansion of the tree. 
        The iterative procedures end when the priority queue becomes empty.
        
        The \textcolor{blue}{highlighted line} in the following algorithm needs to inject different algorithms based on the aggregation protocol:
        for \rlalgo~($\rlalgopolicy$), use \Cref{thm:action-set-ppa};
        for \rlalgotmp~($\rlalgotmppolicy$), use \Cref{thm:action-set-tpa};
        for \rlalgodyntmp~($\rlalgodyntmppolicy$), use \Cref{thm:action-set-dtpa}.
        
        \input{algos-treesearch}
        
        
        \paragraph{Time Complexity.}
        The complexity of \adasearch is $O(H |\gS_{\mathrm{explored}}|(\log |\gS_{\mathrm{explored}}| + |\gA| T))$, where $|\gS_{\mathrm{explored}}|$ is the number of explored states throughout the search procedure, which is no larger than cardinality of state set $\gS$, $H$ is the horizon length, $|\gA|$ is the cardinality of action set, and $T$ is the time complexity of per-state action certification. 
        The main bottleneck of the algorithm is the large number of possible states, which is in the worse case exponential to state dimension. However, to provide a deterministic worst-case certification agnostic to environment properties, exploring all possible states may be inevitable.
        
        
        \paragraph{Relation with \citet{wu2022crop}.}
        The \adasearch algorithm is inspired from \citet[Algorithm 3]{wu2022crop}, which also leverages tree search to explore all possible states and thus derive the robustness guarantee.
        However, the major distinction is that their algorithm tries to derive a probabilistic guarantee of RL robustness against state perturbations, while \adasearch derives deterministic guarantee of RL robustness against poisoning attacks.
        We think this general tree search methodology can be further extended to provide certification beyond evasion attack~\citep{wu2022crop} and poisoning attack~(our work) and we leave it as future work.
        
        \paragraph{Extension to stochastic MDPs.}
        In the current version of \adasearch, the exhaustive search is enabled by the deterministic MDP assumption. However, we foresee  the potential of conveniently extending \adasearch to stochastic MDPs and will discuss one concrete method below.
        In contrast to interacting with the environment for one time to obtain the \textit{deterministic} next state transition in the deterministic MDP case, in the case of stochastic MDPs, 
        we can leverage \textit{sampling} (\ie, by repeatedly taking the same action at the same state) to obtain the set of high probability next state transitions with high confidence. In this way, our \adasearch will be able to yield a \textit{probabilistic bound}, in comparison with the \textit{deterministic bound} achieved in this paper enabled by the deterministic MDP assumption.
        

\section{Proofs}
    
    \label{adxsec:proofs}
    
    \subsection{Tightness of Per-State Action Certification in \rlalgo}
        
        \label{adxsubsec:proof-C1}
        \begin{proof}[Proof of \Cref{prop:ppa-radius-tightness}]
            We prove by construction.
            Given the state $s_t$, we first locate the subpolicies whose chosen action is $a$, and denote the set of them as 
            $$
                B = \{ i \in [u]
                \,\mid\,
                \pi_i(s_t) = a = \rlalgopolicy(s_t)
                \}.
            $$
            We also denote $a' = \argmax_{a'\neq a} n_{a'}(s_t) + \1[a' < a]$.
            According to $\wbar K_t$'s definition~(\Cref{eq:ppa-radius}), 
            $$
                |B| = n_a(s_t) > n_a(s_t)/2 \ge \wbar K_t.
            $$
            We now pick an arbitrary subset $B' \subseteq B$ such that $|B'| = \wbar K_t + 1$.
            For each $i \in B'$, we locate its corresponding parititioned dataset $D_i$ for training subpolicy $\pi_i$.
            We insert one point $p_i$ to $D_i$, such that our chosen learning algorithm $\gM_0$ can train a subpolicy $\tpi_i = \gM_0(D_i \cup \{p_i\})$ that satisfies $\tpi_i(s_t) = a'$.
            For example, the point could be $p_i = \{(s_t, a', s', \infty)\}$ and $\gM_0$ learns the action with maximum reward for the memorized nearest state, where $s'$ can be adjusted to make sure the point is hashed to parition $i$.\footnote{Strictly speaking, we need to choose a determinisitc hash function $h$ for dataset partitioning such that adjustment on $s'$ and reward~(currently $\infty$, but can be an arbitrary large enough number) can make the point being partitioned to $i$, \ie, $h(p_i) \equiv i\ ({\rm mod\ } u)$. Since our adjustment space is infinite due to infinite number of large enough reward, such assumption can be easily achieved. Same applies to other attack constructions in the following proofs.}
            Then, we construct the poisoned dataset 
            $$
                \wtilde D = \left(\bigcup_{i \in B'} D_i \cup \{p_i\}\right) \cup \left(\bigcup_{i \in [u] \setminus B'} D_i\right).
            $$
            Therefore, we have $\wtilde D \ominus D = \cup_{i\in B'} p_i = |B'| = \wbar K_t+1$.
            
            On this poisoned dataset, we train subpolicies $\{\tpi_i\}_{i=0}^{u-1}$ and get the aggregated policy $\wtilde \rlalgopolicy$.
            To study $\wtilde \rlalgopolicy (s_t)$, we compute the aggregated action count $\wtilde n_a$ on these poisoned subpolicies.
            We found that $\wtilde n_{a}(s_t) = n_a(s_t) - |B'|$ and $\wtilde n_{a'}(s_t) = n_{a'}(s_t) + |B'|$.
            Therefore,
            $$
            \begin{aligned}
                \wtilde n_a(s_t) - \wtilde n_{a'}(s_t) & = n_a(s_t) - n_{a'}(s_t) - 2(\wbar K_t + 1) \\
                & = n_a(s_t) - n_{a'}(s_t) - 2
                \left(
                \Big\lfloor
                \dfrac{n_a(s_t) - n_{a'}(s_t) - \1[a'<a]}{2}
                \Big\rfloor
                +1
                \right) \\
                & <
                n_a(s_t) - n_{a'}(s_t) - (n_a(s_t) - n_{a'}(s_t) - \1[a'<a])
                = \1[a' < a].
            \end{aligned}
            $$
            Therefore, if $a' < a$, $\wtilde n_a(s_t) \le \wtilde n_{a'}(s_t)$, and $a'$ has higher priority to be chosen than $a$;
            if $a' > a$, $\wtilde n_a(s_t) \le \wtilde n_{a'}(s_t) - 1$, and $a'$ still has higher priority to be chosen than $a$.
            Hence, $\wtilde \rlalgopolicy(s_t) \neq a = \rlalgopolicy(s_t)$.
            To this point, we conclude the proof with a feasible construction.
        \end{proof}
        
    \subsection{Per-State Action Certification in \rlalgotmp}
        
        \label{adxsubsec:proof-C2}
        \begin{proof}[Proof of \Cref{thm:tpa-radius}]
            For ease of notation, we let $w = \min\{W,t+1\}$ so $w$ is the actual window size used at step $t$.
            We let $t_0 = t - w + 1$, \ie, $t_0$ is the actual start time step for \rlalgotmp aggregation at step $t$.
            Now we can write the chosen action at step $t$ without poisoning as $a = \rlalgotmppolicy(s_{t_0:t})$.
            
            We prove the theorem by contradiction:
            We assume that there is a poisoning attack whose poisoning size $K \le \wbar K_t$ where $\wbar K_t$ is defined by \Cref{eq:tpa-radius-1} in the theorem, and after poisoning, the chosen action is $a^T \neq a$.
            We denote $\{\tpi_i\}_{i=0}^{u-1}$ to the poisoned subpolicies and $\wtilde \rlalgotmppolicy$ to the poisoned \rlalgotmp aggregated policy.
            From the definition of $\wbar K_t$, we have
            \begin{equation}
                \sum_{i=1}^{K} h_{a,a^T}^{(i)} \le \sum_{i=1}^{\wbar K_t} h_{a,a^T}^{(i)} \le \delta_{a,a^T},
                \label{adxeq:3-1}
            \end{equation}
            since $K \le \wbar K_t$, and each $h_{a,a^T}^{(i)}$ is an element of $h_{i',a,a^T}$ for some $i'$ where
            $$
                h_{i',a,a^T} = 
                \sum_{j=0}^{w-1} \1_{i',a}(s_{t-j}) + w - \sum_{j=0}^{w-1} \1_{i',a^T}(s_{t-j})
                \ge 0
            $$
            by \Cref{eq:tpa-radius-2} in the theorem.
            Since the poisoning attack within threshold $K$ can at most affect $K$ subpolicies, we let $B$ be the set of affected policies and assume $|B| = K$ without loss of generality. 
            Formally, $B = \{i \in [u] \,\mid\, \exists t' \in [t_0,t], \tpi_i(s_{t'}) \neq \pi_i(s_{t'}) \}$.
            Therefore, according to the monotonicity of $h_{a,a^T}^{(i)}$, from \Cref{adxeq:3-1},
            \begin{equation}
                \sum_{i\in B} h_{i,a,a^T} \le \sum_{i=1}^{K} h_{a,a^T}^{(i)} \le \delta_{a,a^T}.
                \label{adxeq:3-2}
            \end{equation}
            
            According to the assumption of successfully poisoning attack,
            after attack, the sum of aggregated vote for $a^T$ plus $\1[a^T < a]$ should be larger then that of $a$.
            Formally, after the poisoning, 
            $$
                \wtilde n_{a^T}(s_{t_0:t}) + \1[a^T < a] > \wtilde n_{a}(s_{t_0:t})
            $$
            or equivalently
            $$
                 \wtilde n_{a}(s_{t_0:t}) - (\wtilde n_{a^T}(s_{t_0:t}) + \1[a^T < a]) < 0.
            $$
            From the statement of \Cref{thm:tpa-radius},
            $$
                \delta_{a,a^T} = n_a(s_{t_0:t}) - (n_{a^T}(s_{t_0:t}) + \1[a^T < a]).
            $$
            Take the difference of the above two equations, we know that
            the attack satisfies
            \begin{equation}
                n_a(s_{t_0:t}) - \wtilde n_a(s_{t_0:t}) - (n_{a^T}(s_{t_0:t}) - \wtilde n_{a^T}(s_{t_0:t})) > \delta_{a,a^T}.
                \label{adxeq:3-3}
            \end{equation}
            Since the attack only changes the subpolicies in $B$,
            we have
            $$
            \begin{aligned}
                n_a(s_{t_0:t}) - \wtilde n_a(s_{t_0:t}) & = \sum_{i\in B} \left( \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j}) = a] - \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j}) = a] \right) \\
                & \le \sum_{i\in B} \sum_{j=0}^{w-1} \1_{i,a}(s_{t-j}), \\
            % $$
            % $$
                n_{a^T}(s_{t_0:t}) - \wtilde n_{a^T}(s_{t_0:t}) & = \sum_{i\in B} \left(
                \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j}) = a^T] - \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j}) = a^T] \right) \\
                & \ge \sum_{i\in B} \left(\sum_{j=0}^{w-1} \1_{i,a^T}(s_{t_j}) - w\right). \\
            \end{aligned}
            $$
            Inject them into \Cref{adxeq:3-3} yields
            $$
                \sum_{i\in B} \underbrace{\left( \sum_{j=0}^{w-1} \1_{i,a}(s_{t-j}) + w - \sum_{j=0}^{w-1} \1_{i,a^T}(s_{t-j}) \right)}_{h_{i,a,a^T}} > \delta_{a,a^T}
            $$
            which contradicts \Cref{adxeq:3-2} and thus concludes the proof.
        \end{proof}
    
    \subsection{Tightness of Per-State Action Certification in \rlalgotmp}
    
        \label{adxsubsec:proof-C3}
        \allowdisplaybreaks
        
        
        % \begin{proposition}
        %     \label{prop:tpa-radius-tightness}
        %     Under the same condition as \Cref{thm:tpa-radius}, for any time step $t$,
        %     there exists an RL learning algorithm $\gM_0$, and a poisoned dataset $\wtilde D$, such that $| D \ominus \wtilde D | = \wbar K_t + 1$, and $\wtilde \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t}) \neq \rlalgotmppolicy(s_{\max\{t-W+1,0\}:t})$.
        % \end{proposition}
        
        \begin{proof}[Proof of \Cref{prop:tpa-radius-tightness}]
            For ease of notation, we let $w = \min\{W,t+1\}$ so $w$ is the actual window size used at step $t$.
            We let $t_0 = t - w + 1$, \ie, $t_0$ is the actual start time step for \rlalgotmp aggregation at step $t$.
            Now we can write the chosen action at step $t$ without poisoning as $a = \rlalgotmppolicy(s_{t_0:t})$.
            
            We prove by construction, \ie, we construct an poisoning attack with poisoning size $\wbar K_t + 1$ that deviates the prediction of the poisoned policy.
            Specifically,
            we aim to craft a poisoned dataset $\wtilde D$ with poisoning size $|D \ominus \wtilde D| = \wbar K_t + 1$,
            such that for certain learning algorithm $\gM_0$, after partitioning and learning on the poisoned dataset, the poisoned subpolicies $\tpi_i = \gM_0(\wtilde D_i)$ can be aggregated to produce different action prediction: $\wtilde \rlalgotmppolicy(s_{t_0:t}) \neq a$.
            
            Before construction, we first show that $\wbar K_t$ given by \Cref{eq:tpa-radius-1} satisfies $\wbar K_t < u$.
            If $\wbar K_t = u$, it means that for arbitrary $a' \neq a$,
            $$
            \begin{aligned}
                & \sum_{i=1}^u h_{a,a'}^{(i)} = \sum_{i=0}^{u-1} h_{i,a,a'}
                = \sum_{i=0}^{u-1} \left(\sum_{j=0}^{w-1} \1_{i,a}(s_{t-j}) + w - \sum_{j=0}^{w-1} \1_{i,a'}(s_{t-j})\right) = n_a(s_{t_0:t}) + uw - n_{a'}(s_{t_0:t}) \\
                & \le \delta_{a,a'} = n_a(s_{t_0:t}) - n_{a'}(s_{t_0:t}) - \1[a'<a],
            \end{aligned}
            $$
            which implies $uw \le 0$ contracting $uw > 0$.
            Now, we know $\wbar K_t < u$, so $\wbar K_t + 1$, our poisoning size, is smaller or equal to $u$.
            
            We start our construction by choosing an action $a^T$:
            $$
                a^T = \argmin_{a'\neq a, a'\in \gA}
                \argmax_{\sum_{i=1}^p h_{a,a'}^{(i)} \le \delta_{a,a'}} p.
            $$
            According to the definition of $\wbar K_t$ in \Cref{eq:tpa-radius-1}, for $a^T$ we have
            \begin{equation}
                \sum_{i=1}^{\wbar K_t + 1} h_{a,a^T}^{(i)} > \delta_{a,a^T}.
                \label{adxeq:4-1}
            \end{equation}
            We locate the subpolicies to poison as 
            \begin{equation}
                B = \{ i \in [u] \,\mid\,
                h_{a,a^T}^i \text{ is } h_{a,a^T}^{(j)} \text{ in the nonincreasing permutation in \Cref{eq:tpa-radius-2}}, j \le \wbar K_t + 1
                \}
                \label{adxeq:4-2}
            \end{equation}
            Therefore, $|B| = \wbar K_t + 1$ and 
            \begin{equation}
                \sum_{i \in B} h_{i,a,a^T} > \delta_{a,a^T}
                \label{adxeq:4-3}
            \end{equation}
            by \Cref{adxeq:4-1}.
            For each of these subpolicies $i \in B$, we locate its corresponding partitioned dataset $D_i$ for training subpolicy $\pi_i$, and insert one trajectory $p_i$ to $D_i$, such that our chosen learning algorithm $\gM_0$ can train a subpolicy $\tpi_i = \gM(D_i \cup \{p_i\})$ satisfying $\tpi_i(s_{t'}) = a^T$ for any $t' \in [t_0,t]$.
            For example, the trajectory could be $p_i = \{(s_{t'}, a^T, s', \infty)\}_{t'=t_0}^t$ and $\gM_0$ learns the action with maximum reward for the memorized nearest state, where $s'$ can be adjusted to make sure the trajectory is hashed to partition $i$.
            Then, we construct the poisoned dataset
            $$
                \wtilde D = \left(\bigcup_{i \in B'} D_i \cup \{p_i\}\right) \cup \left(\bigcup_{i \in [u] \setminus B'} D_i\right).
            $$
            Therefore, we have $\wtilde D \ominus D = \cup_{i\in B'} p_i = |B'| = \wbar K_t+1$.
            Now, we compare the aggregated votes for $a$ and $a^T$ before and after poisoning:
            \begin{align*}
                \wtilde n_a(s_{t_0:t}) - n_a(s_{t_0:t}) & = \sum_{i\in B} \left(\sum_{j=0}^{w-1} \1[\wtilde \pi_i(s_{t-j})=a] - \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a]\right) \\
                & = - \sum_{i\in B} \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a], \\
                \wtilde n_{a^T}(s_{t_0:t}) - n_{a^T}(s_{t_0:t}) & = \sum_{i\in B} \left(\sum_{j=0}^{w-1} \1[\wtilde \pi_i(s_{t-j})=a^T] - \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a^T]\right)  \\
                & = \sum_{i\in B} \left(w - \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a^T]\right).
            \end{align*}
            Now we compare the margin between aggregated votes for $a$ and $a^T$ after poisoning:
            \begin{align*}
                & \wtilde n_{a^T}(s_{t_0:t}) - \wtilde n_a(s_{t_0:t}) + \1[a^T < a] \\
                = &
                n_{a^T}(s_{t_0:t}) - n_a(s_{t_0:t}) + \1[a^T < a] + \wtilde n_{a^T}(s_{t_0:t}) - n_{a^T}(s_{t_0:t}) - \left( \wtilde n_a(s_{t_0:t}) - n_a(s_{t_0:t}) \right) \\
                = & -\delta_{a,a^T} + \sum_{i\in B}
                \left(
                    \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a]
                    + w - \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a^T]
                \right) \\
                = & -\delta_{a,a^T} + \sum_{i\in B} h_{i,a,a^T} > 0.
            \end{align*}
            As a result, after poisoning, $a^T$ has higher priority to be chosen than $a$, \ie, $\wtilde \rlalgotmppolicy(s_{t_0:t}) \neq a = \rlalgotmppolicy(s_{t_0:t})$.
            To this point, we conclude the proof with a feasible attack construction.
        \end{proof}
        
    \subsection{Loose Per-State Action Certification in \rlalgotmp and Comparision with Tight One}
        \label{adxsubsec:loose-tpa-and-compare}
        \label{adxsubsec:proof-C4}
        
        The following corollary of \Cref{thm:ppa-radius} states a loose per-state action certification.
        \begin{corollary}
            \label{cor:tpa-radius-2}
            Under the same condition as \Cref{thm:tpa-radius},
            \begin{equation}
        	    \wbar K_t = \left\lfloor\frac{n_{a}(s_{\max\{t-W+1,0\}:t})-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}(s_{\max\{t-W+1,0\}:t})+\1[a^{\prime}<a]\right)}{2\min\{W,t+1\}}\right\rfloor
        	    \label{eq:rpa-radius-2}
        	\end{equation}
        	is a \emph{tolerable poisoning threshold} at time step $t$ in \Cref{def:per-state}, where $W$ is the window size.
        \end{corollary}
        
        \begin{proof}[Proof of \Cref{cor:tpa-radius-2}]
            We let $w = \min\{t+1, W\}$ to be the actual aggregation window size at time step $t$.
            After poisoning with size $K$, 
            at most $K$ subpolicies are affected and each affected policy can only make $\pm w$ changes to the aggregated action count.
            This implies that, after poisoning, for any action $a' \in \gA$, the aggregated vote count $\wtilde n_{a'}(s_{t-w+1:t}) \in [n_{a'}(s_{t-w+1:t}) - uw, n_{a'}(s_{t-w+1:t}) + uw]$.
            Thus, when $K \le \wbar K_t$ where $\wbar K_t$ is defined in \Cref{thm:tpa-radius}, for any $a' \neq a$, we have
            $$
            \begin{aligned}
                & \tilde n_{a}(s_{t-w+1:t}) - \tilde n_{a'}(s_{t-w+1:t}) - \1[a' < a] \\
                = & n_{a}(s_{t-w+1:t}) - n_{a'}(s_{t-w+1:t}) - \1[a' < a] - 2Kw \\
                \ge & n_{a}(s_{t-w+1:t}) - n_{a'}(s_{t-w+1:t}) - \1[a' < a] - 2w \cdot \wbar K_t \\
                \ge & n_{a}(s_{t-w+1:t}) - n_{a'}(s_{t-w+1:t}) - \1[a' < a] - \left( n_{a}(s_{t-w+1:t}) - \max_{a''\neq a} (n_{a''}(s_{t-w+1:t}) + \1[a''< a]) \right) \\
                = & \max_{a''\neq a} (n_{a''}(s_{t-w+1:t}) + \1[a''< a]) - \left( n_{a'}(s_{t-w+1:t}) + \1[a' < a] \right)
                \ge 0.
            \end{aligned}
            $$
            From the definition of \rlalgotmp protocol, the poisoned policy still chooses action $a$, which implies $\wbar K_t$ is a tolerable poisoning threshold.
        \end{proof}
        
        In the main text, we mention that the certification from \Cref{cor:tpa-radius-2} is looser than that from \Cref{thm:tpa-radius}.
        This assertion is based on the following two facts:
        \begin{enumerate}[leftmargin=*]
            \item According to \Cref{prop:tpa-radius-tightness}, the certification given by \Cref{thm:tpa-radius} is theoretically tight, which means that any other certification can only be as tight as \Cref{thm:tpa-radius} or looser than it.
            
            \item There exists examples where the computed $\wbar K_t$ from \Cref{thm:tpa-radius} is larger than that from \Cref{cor:tpa-radius-2}. \\
            For instance, suppose $W = 5$, action set $\gA = \{a_1, a_2\}$, and there are three subpolicies. 
            At time step $t = 4$, $\pi_i$ for $s_{0}$ to $s_{4}$ are $[a_1,a_1,a_1,a_1,a_2]$ for all subpolicies~(\ie, $i\in [3]$).
            Thus, the benign policy $\rlalgotmppolicy(s_{0:4}) = a_1$.
            By computation, the $\wbar K_t$ from \Cref{thm:tpa-radius} is $1$; 
            while the $\wbar K_t$ from \Cref{cor:tpa-radius-2} is $0$.
        \end{enumerate}
        
        Indeed, \Cref{cor:tpa-radius-2} can be viewed as using $2w$ to upper bound $h_{i,a,a'} = w + \sum_{j=0}^{w-1} \1_{i,a}(s_{t-j}) - \sum_{j=0}^{w-1} \1_{i,a'}(s_{t-j})$.
        Intuitively, \Cref{cor:tpa-radius-2} assumes every subpolicy can provide $2w$ vote margin shrinkage, and \Cref{thm:tpa-radius} uses $h_{i,a,a'}$ to capture the precise worse-case margin shrinkage and thus provides a tighter certification.
        
    \subsection{Per-State Action Certification in \rlalgodyntmp}
    
        \label{adxsubsec:proof-C5}
        \begin{proof}[Proof of \Cref{thm:dtpa-radius}]
            Without loss of generality, we assume $W_{\max} \le t+1$ and otherwise we let $W_{\max} \gets \min\{W_{\max}, t+1\}$.
            We let $t_0 = \max\{t - W_{\max} + 1,0\}$ be the start time step of the maximum possible window.
            To prove the theorem, our general methodology is to enumerate all possible cases of a successful attack, and derive the tolerable poisoning threshold for each case respectively.
            Taking a minimum over these tolerable poisoning thresholds gives the required result.
            
            Specifically, we denote $\gP$ to the predicate of robustness under poisoning attack: $\gP = [\wtilde \rlalgodyntmppolicy(s_{t_0:t}) = a]$, and denote $K$ to the poisoning attack size.
            Therefore, we can decompose $\gP$ as such:
            \begin{equation}
                \gP = \gP(W') \wedge  \bigwedge_{\substack{1\le W^* \le W_{\max}, W^* \neq W'\\ a'\neq a}} \neg \gQ(W^*,a').
                \label{adxeq:6-1}
            \end{equation}
            Recall that $W'$ is the chosen window size by the protocol \rlalgodyntmp with unattacked subpolicies $\rlalgodyntmppolicy$ (\Cref{eq:dtpa-agg-1}).
            In \Cref{adxeq:6-1}, the predicate $\gP(W')$ means that after poisoning attack, whether the prediction under window size $W'$ is still $a$;
            the predicate $\gQ(W^*, a')$ means that after poisoning attack, whether the chosen action is $a'$ at window size $W^*$ and average vote margin is larger~(or equal if $a' < a$) at window size $W^*$ compared to $W'$.
            Formally, let $\wtilde n_a$ be the aggregated action count after poisoning and $\wtilde \Delta_t^W$ be the average vote margin after poisoning at window $W$~(see \Cref{eq:dtpa-agg-2}),
            \begin{equation}
                \begin{aligned}
                    \gP(W') = & \left(\argmax_{a\in \gA} \wtilde n_a(s_{t-W'+1:t}) = a\right), \\
                    \gQ(W^*,a') = & \left(\argmax_{a\in \gA} \wtilde n_a(s_{t-W^*+1:t}) = a'  \right) \wedge \\
                    & \left( \left(\left( \wtilde \Delta_t^{W^*} \ge \wtilde \Delta_t^{W'} \right) \wedge (a' < a)\right) \vee \left( \left( \wtilde \Delta_t^{W^*} > \wtilde \Delta_t^{W'} \right) \wedge (a' > a) \right) \right).
                \end{aligned}
                \label{adxeq:6-2}
            \end{equation}
            According to \Cref{thm:tpa-radius},
            \begin{equation*}
                K \le \wbar K_t \Longrightarrow \gP(W')
            \end{equation*}
            where $\wbar K_t$ is defined by \Cref{eq:tpa-radius-1} with $W$ replaced by $W'$.
            The following \Cref{adxlem:6-1} shows a sufficient condition for $Q(W^*,a')$.
            We then aggregate these conditions together with minimum to obtain a sufficient condition for $\gP$:
            $$
                K \le \min\left\{ \wbar K_t,\, \min_{1\le W^* \le \min\{W_{\max}, t+1\}, W^* \neq W', a'\neq a, a''\neq a} L_{a',a''}^{W^*, W'} \right\}
            $$
            and thus conclude the proof.
        \end{proof}
        
        
        \begin{lemma}
            \label{adxlem:6-1}
            Let $\gQ(W^*, a')$, $K$, $W'$ be the same as defined in proof of \Cref{thm:dtpa-radius}, then
            \begin{equation}
                K \le \min_{a''\neq a} L_{a',a''}^{W^*,W'} \Longrightarrow \neg \gQ(W^*,a'),
                % \label{eq:adxlem:6-1}
            \end{equation}
            where $L_{a',a''}^{W^*,W'}$ is defined in \Cref{def:L}.
        \end{lemma}
        
        \begin{proof}
            We prove the equivalent form:
            \begin{equation}
                \gQ(W^*,a') \Longrightarrow K > \min_{a''\neq a} L_{a',a''}^{W^*,W'}.
                \label{adxeq:6-3}
            \end{equation}
            Suppose a poisoning attack can successfully achieve $Q(W^*, a')$, we now induce the requirement on its poisoning size $K$.
            First, we notice that
            \begin{equation}
                \begin{aligned}
                    & \left(\left( \wtilde \Delta_t^{W^*} \ge \wtilde \Delta_t^{W'} \right) \wedge (a' < a)\right) \vee \left( \left( \wtilde \Delta_t^{W^*} > \wtilde \Delta_t^{W'} \right) \wedge (a' > a) \right) \\
                    \iff & W^*W' \wtilde \Delta_t^{W^*} \ge W^*W' \wtilde \Delta_t^{W'} + \1[a' > a]
                \end{aligned}
                \label{adxeq:6-4}
            \end{equation}
            since $W^*W'\wtilde \Delta_t^{W*/W^*}$ is an integer by definition.
            According to the definition and $\gQ(W^*,a')$'s assumption that $\argmax_{a\in \gA} \wtilde n_a(s_{t-W^*+1:t}) = a'$, 
            $$
                W^* W' \wtilde \Delta_t^{W^*} \le W' \left( \wtilde n_{a'}(s_{t-W^*+1:t}) - \wtilde n_{a^\#}(s_{t-W^*+1:t}) \right),
            $$
            where ``$\le$'' comes from the fact that the margin in $\wtilde \Delta_t^{W^*}$ should be with respect to the runner-up class after poisoning, and computing with respect to any other class provides an upper bound.
            Here we choose $a^\# = \argmax_{a_0\neq a', a_0\in \gA} n_{a_0}(s_{t-W^*+1:t})$~(see \Cref{def:L}), the runner-up class before poisoning, to empirically shrink the gap between the bound and actual margin.
            On the other hand,
            $$
                W^*W'\wtilde \Delta_t^{W'} \ge W^* \left(\wtilde n_a (s_{t-W'+1:t}) - \max_{a''\neq a} \wtilde n_{a''}(s_{t-W'+1:t}) \right),
            $$
            where ``$\ge$'' comes from the fact that the margin in $\wtilde \Delta_t^{W'}$ should use the top class after poisoning, and computing with any other class provides a lower bound.
            Thus, from \Cref{adxeq:6-4} and the above two relaxations, we get
            \begin{equation*}
                \begin{aligned}
                    & Q(W^*,a') \\
                    \Longrightarrow &
                    W' \left( \wtilde n_{a'}(s_{t-W^*+1:t}) - \wtilde n_{a^\#}(s_{t-W^*+1:t}) \right)
                    \ge W^* \left(\wtilde n_a (s_{t-W'+1:t}) - \max_{a''\neq a} \wtilde n_{a''}(s_{t-W'+1:t}) \right) + \1[a' > a]  \\
                    \Longrightarrow &
                    \exists a'' \neq a, \\
                    & W' \left( \wtilde n_{a'}(s_{t-W^*+1:t}) - \wtilde n_{a^\#}(s_{t-W^*+1:t}) \right)
                    \ge W^* \left(\wtilde n_a (s_{t-W'+1:t}) - \wtilde n_{a''}(s_{t-W'+1:t}) \right) + \1[a' > a].
                \end{aligned}
            \end{equation*}
            For each $a'' \neq a$, now we use the last equation as the condition, and show that $K > L_{a',a''}^{W^*,W'}$ is a necessary condition.
            This proposition is equivalent to
            \begin{equation}
                \begin{aligned}
                    & K \le L_{a',a''}^{W^*,W'} \\
                    \Longrightarrow & 
                    W' \left( \wtilde n_{a'}(s_{t-W^*+1:t}) - \wtilde n_{a^\#}(s_{t-W^*+1:t}) \right)
                    < W^* \left(\wtilde n_a (s_{t-W'+1:t}) - \wtilde n_{a''}(s_{t-W'+1:t}) \right) + \1[a' > a].
                \end{aligned}
                \label{adxeq:6-5}
            \end{equation}
            
            Suppose a poisoning attack within poisoning size $K$ changes the subpolicies in set $B \subseteq [u]$.
            Note that $|B| \le K$.
            We inspect the objective in \Cref{adxeq:6-5}:
            \begingroup
            \allowdisplaybreaks
            \begin{align*}
                \small
                    & W' \left(\wtilde n_{a'}(s_{t-W^*+1:t}) - \wtilde n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left(\wtilde n_a (s_{t-W'+1:t}) - \wtilde n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] \\
                    = &  W' \left( n_{a'}(s_{t-W^*+1:t}) -  n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left( n_a (s_{t-W'+1:t}) -  n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] \\
                    & + \sum_{i \in B} \left( W' \sum_{w=0}^{W^*-1} \1[\tpi_i(s_{t-w+1})=a'] - W' \sum_{w=0}^{W^*-1} \1[\tpi_i(s_{t-w+1})=a^\#] \right. \\
                    & \hspace{3em} \left. - W^* \sum_{w=0}^{W'-1} \1[\tpi_i(s_{t-w+1})=a] + W^* \sum_{w=0}^{W'-1} \1[\tpi_i(s_{t-w+1})=a''] \right) \\
                    & - \sum_{i \in B} \left( W' \sum_{w=0}^{W^*-1} \1[\pi_i(s_{t-w+1})=a'] - W' \sum_{w=0}^{W^*-1} \1[\pi_i(s_{t-w+1})=a^\#] \right. \\
                    & \hspace{3em} \left. - W^* \sum_{w=0}^{W'-1} \1[\pi_i(s_{t-w+1})=a] + W^* \sum_{w=0}^{W'-1} \1[\pi_i(s_{t-w+1})=a''] \right) \\
                    = & W' \left( n_{a'}(s_{t-W^*+1:t}) -  n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left( n_a (s_{t-W'+1:t}) -  n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] \\
                    & + \sum_{i\in B} \sum_{w=0}^{\max\{W^*, W'\}}
                    \sigma^w(\tpi_i(s_{t-w})) - \sigma^w(\pi_i(s_{t-w})) \\
                    \le & W' \left( n_{a'}(s_{t-W^*+1:t}) -  n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left( n_a (s_{t-W'+1:t}) -  n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] \\
                    & + \sum_{i\in B} \underbrace{\sum_{w=0}^{\max\{W^*, W'\}} \max_{a_0\in \gA} \sigma^w(a_0) - \sigma^w(\pi_i(s_{t-w}))}_{g_i} \\
                    \overset{(a)}{\le} & W' \left( n_{a'}(s_{t-W^*+1:t}) -  n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left( n_a (s_{t-W'+1:t}) -  n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] %\\
                    % & 
                    + \sum_{i=1}^{K} g^{(i)} \\ 
                    \overset{(b)}{\le} & W' \left( n_{a'}(s_{t-W^*+1:t}) -  n_{a^\#}(s_{t-W^*+1:t}) \right) - W^* \left( n_a (s_{t-W'+1:t}) -  n_{a''}(s_{t-W'+1:t}) \right) - \1[a' > a] %\\
                    % & 
                    + \sum_{i=1}^{L^{W^*,W'}_{a',a''}} g^{(i)} \\
                    \overset{(c)}{<} & 0. \\ 
            \end{align*}
            \endgroup
            Thus, \Cref{adxeq:6-5} is proved.
            Therefore, $K > L_{a',a''}^{W^*,W'}$ is a necessary condition for $Q(W^*,a')$, \ie, \Cref{adxeq:6-3}.
            
            In the above deriviation, the definitions of $g^i$, $g^{i}$, and $\sigma^w$ are from \Cref{eq:L-2}.
            $(a)$ comes from the facts that $\{g^{(i)}\}_{i=1}^u$ is a nondecreasing permutation of $\{g_i\}_{i=0}^{u-1}$, $g_i \ge 0$, and $|B| \le K$.
            $(b)$ comes from the assumption $K \le L_{a,a''}^{W^*,W'}$ and also $g^{(i)} \ge 0$.
            $(c)$ comes from the definition in \Cref{eq:L-1}.
        \end{proof}
        
    \subsection{Possible Action Set in \rlalgo and Comparison}
    
        \label{adxsubsec:proof-C6}
        \subsubsection{Certification}
        \label{adxsubsec:proof-C61}
        \begin{proof}[Proof of \Cref{thm:action-set-ppa}]
            According to the definition of possible action set, we only need to prove the contrary: for any $a \in \gA \setminus A^T(K)$, within poisoning size $K$, the poisoned policy cannot choose $a$: $\wtilde \rlalgopolicy(s_t) \neq a$.  
    
            According to \Cref{eq:action-set-ppa}, any $a \in \gA \setminus A^T(K)$ satisfies
            \begin{equation}
                \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a' < a], 0\} > K.
                \label{adxeq:7-1}
            \end{equation}
            Given poisoning size $K$, since each poisoning size can affect only one subpolicy, we know
            $$
                \wtilde n_a(s_t) \le n_a(s_t) + K
            $$
            where $\wtilde n_a$ denotes to the poisoned aggregated action count.
            We suppose the attack could be successful, then
            for $a' < a$, $\wtilde n_{a'}(s_t) \le \wtilde n_{a}(s_t) - 1$, and thus $n_{a'}(s_t) - \wtilde n_{a'}(s_t) \ge n_{a'}(s_t) - n_a(s_t) - K + 1$.
            Similarly, for $a' > a$, $\wtilde{a'}(s_t) \le \wtilde n_a(s_t)$, and thus $n_{a'}(s_t) - \wtilde n_{a'}(s_t) \ge n_{a'}(s_t) - n_a(s_t) - K$.
            Also, for any $a' \neq a$ after poisoning $n_{a'}(s_t) - \wtilde n_{a'}(s_t) \ge 0$; otherwise deviating the difference subpolicies' decisions' from $a'$ to $a$ is strictly no-worse.
            Given these facts, the amount of votes that need to be reduced is the LHS of \Cref{adxeq:7-1} which is larger than $K$.
            However, we only have $K$ poisoning size, \ie, $K$ votes that can be reduced.
            As a result, our assumption that the attack could be successful is falsified and the poisoned policy cannot choose $a$.
        \end{proof}
        
        \begin{corollary}[Loose \rlalgo Action Set]
            \label{cor:loose-action-set-ppa}
            Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
            then the \emph{possible action set} at step $t$
            \begin{equation}
                A^L(K) = \left\{
                    a \in \gA
                    \,\Big\lvert\,
                    \max_{a'\in \gA} n_{a'}(s_t) - n_a(s_t) \le 2K - \1[a > \argmax_{a'\in \gA} n_{a'}(s_t)]
                \right\}.
                \label{eq:loose-action-set-ppa}
            \end{equation}
        \end{corollary}
        
        \begin{proof}[Proof of \Cref{cor:loose-action-set-ppa}]
            Again, we prove the contrary, for any $a \in \gA \setminus A^L(K)$, within poisoning size $K$, the poisoned policy cannot choose $a$: $\wtilde \rlalgopolicy(s_t) \neq a$.
            
            According to \Cref{eq:loose-action-set-ppa}, let $a_m = \argmax_{a'\in \gA} n_{a'}(s_t)$, then any $a \in \gA \setminus A^L(K)$ satisfies
            $$
                n_{a_m}(s_t) - n_a(s_t) > 2K - \1[a > a_m].
            $$
            After poisoning, we thus have
            $$
                n_{a_m}(s_t) - n_a(s_t) > -\1[a > a_m] 
                \Longrightarrow
                n_{a_m}(s_t) - n_a(s_t) \ge 1-\1[a > a_m] 
            $$
            From the definition, $a \notin A^L(K)$ so $a \neq a_m$.
            If $a_m < a$, $n_{a_m}(s_t) \ge n_a(s_t)$; if $a_m > a$, $n_{a_m}(s_t) > n_a(s_t)$.
            In both cases, $a_m$ has higher priority to be chosen than $a$, and thus the poisoned policy cannot choose $a$.
        \end{proof}
        
        \subsubsection{Comparison}
        \label{adxsubsec:proof-C62}
        
        \begin{theorem}
            \label{thm:compare-tight-loose-action-set-ppa}
            Under the condition of \Cref{def:possible-action-set}, suppose the aggregation protocol is \rlalgo as defined in \Cref{def:ppa-agg},
            $A^T(K), A^L(K)$ are defined according to \Cref{eq:action-set-ppa,eq:loose-action-set-ppa} accordingly, then
            \begin{enumerate}[leftmargin=*]
                \item $A^T(K) \subseteq A^L(K)$; and there are subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$ such that $A^T(K) \subsetneq A^L(K)$.
                
                \item Given subpolicies $\{\pi_i\}_{i=0}^{u-1}$ and state $s_t$, for any $a \in A^T(K)$, there exists a poisoned training set $\wtilde D$ whose poisoning size $|D \ominus \wtilde D| \le K$ and some RL training mechanism, such that $\wtilde \rlalgopolicy(s_t) = a$ where $\wtilde \rlalgopolicy$ is the poisoned \rlalgo policy trained on $\wtilde D$.
            \end{enumerate}
        \end{theorem}
        \begin{proof}[Proof of \Cref{thm:compare-tight-loose-action-set-ppa}]
            We prove the two arguments separately.
            \begin{enumerate}[leftmargin=*]
                \item We first prove $A^T(K) \subseteq A^L(K)$.
                For any $a \in A^T(K)$, let $a_m = \argmax_{a'\in \gA} n_{a'}(s_t)$, then
                $$
                \begin{aligned}
                    & \sum_{a'\in \gA} \max\{ n_{a'}(s_t) - n_a(s_t) - K + \1[a' < a], 0\} \le K \\
                    \Longrightarrow & n_{a_m}(s_t) - n_a(s_t) - K + \1[a_m < a] \le K \\
                    \Longrightarrow & n_{a_m}(s_t) - n_a(s_t) \le 2K - \1[a > a_m]
                \end{aligned}
                $$
                where the last proposition is exactly the set selector of $A^L(K)$ so $a \in A^L(K)$.
                
                We then prove that $A^T(K) \subsetneq A^L(K)$ can happen by construction.
                Suppose that there are three actions in the action space: $\gA = \{a_1, a_2, a_3\}$.
                We construct subpolicies for current state $s_t$ such that the aggregated action counts are 
                $$
                    n_{a_1}(s_t) = 10, n_{a_2}(s_t) = 9, n_{a_3}(s_t) = 1.
                $$
                Given poisoning size $K=5$, we find that
                $$
                \begin{aligned}
                    & n_{a_1}(s_t) - n_{a_3}(s_t) = 9 \le 10 - \1[a_3 \ge a_1] = 9 & \Longrightarrow a_3 \in a^L(K), \\
                    & \left(n_{a_1}(s_t) - n_{a_3}(s_t) - K + \1[a_1<a_3]\right)  + & \\
                    & \left(n_{a_2}(s_t) - n_{a_3}(s_t) - K + \1[a_2<a_3]\right) = 9 > K = 5 & \Longrightarrow a_3 \notin a^T(K).
                \end{aligned}
                $$
                Therefore, $A^T(K) \subsetneq A^L(K)$ for these subpolicies and state $s_t$.
                
                \item 
                We prove by construction.
                For any $a\in A^T(K)$, we construct the set of subpolicies to poison $B^a \subseteq [u]$ such that $|B^a| \le K$, then describe the corresponding poisoned dataset $\wtilde D^a$, and finally prove that the poisoned policy $\wtilde \rlalgopolicy^a(s_t) = a$. 
                
                For $a \in A^T(K)$, by definition~(\Cref{eq:action-set-ppa}), we know
                \begin{equation}
                    \sum_{a'\in \gA} \max\{ \underbrace{n_{a'}(s_t) - n_a(s_t) - K + \1[a' < a]}_{:= t_{a,a'}}, 0\} \le K.
                    \label{adxeq:9-1}
                \end{equation}
                We now define a set of actions $C^a \subseteq \gA$ such that
                $$
                    C^a = \{ a' \in \gA
                    \,\mid\,
                    t_{a,a'} > 0
                    \}.
                $$
                According to this definition, $a \notin C^a$ since $t_{a,a} \le 0$.
                
                \begin{fact}
                    For $a\in A^T(K)$ and any $a'\in \gA$, $n_a(s_t) + K - \1[a'<a] \ge 0$.
                    \label{fact:c-1}
                \end{fact}
                \begin{proof}[Proof of \Cref{fact:c-1}.]
                    Suppose $n_a(s_t) + K - \1[a'<a] \le 0$, then $n_a(s_t) = K = 0$ and $a' < a$.
                    Then 
                    $$
                    \sum_{a'\in \gA} \max\{n_{a'}(s_t) - n_a(s_t) - K + \1[a'<a], 0\}
                    \ge \sum_{a' \in \gA} n_{a'}(s_t) - n_a(s_t) - K
                    = \sum_{a'\in \gA} n_{a'}(s_t)
                    = u > 0
                    $$
                    which contradicts the requirement that the LHS of the above inequality should be $\le K = 0$.
                \end{proof}
                Give \Cref{fact:c-1}, for any $a' \in C^a$, $n_{a'}(s_t) \ge t_{a,a'}$.
                Notice that $n_{a'}(s_t)$ is the number of subpolicies that vote for action $a'$ at state $s_t$.
                Therefore, we can pick an arbitrary subset of those subpolicies whose cardinality is $t_{a,a'}$.
                We denote $B_{a'}^a$ to such subset:
                $$
                    B_{a'}^a \subseteq \{ i\in [u] \,\mid\, \pi_i(s_t) = a' \},
                    \,
                    |B_{a'}^a| = t_{a,a'}.
                $$
                Now define $B^a_{\alpha}$: $B^a_{\alpha} = \bigcup_{a'\in C^a} B^a_{a'}$.
                We construct $B^a_{\beta}$ to be an arbitrary subset of those subpolicies whose prediction is not $a$ and who are not in $B^a_{\alpha}$, and limit the $B^a_{\beta}$'s cardinality:
                $$
                    B^a_{\beta} \subseteq \{i \in [u] \,\mid\, \pi_i(s_t) \neq a \} \setminus B^a_{\alpha},
                    |B^a_{\beta}| = \min \{ K - |B^a_{\alpha}|, u - n_a(s_t) - |B^a_{\alpha}| \}.
                $$
                Such $B^a_{\beta}$ can be selected, because:
                \begin{itemize}
                    \item From definition, $B_{\alpha}^a \subseteq \{i\in [u] \,\mid\, \pi_i(s_t) \neq a\}$, where the cardinality of $\{i\in [u] \,\mid\, \pi_i(s_t) \neq a\}$ is $u - n_a(s_t)$. So $0 \le u - n_a(s_t) - |B_{\alpha}^a|$.
                    
                    \item Since
                    $$
                        |B^a_{\alpha}|\le 
                        \sum_{a'\in C^a} |B_{a'}^a| = \sum_{a'\in C^a} t_{a,a'} = \sum_{a'\in \gA, t_{a,a'} > 0} t_{a,a'} \overset{(*)}{\le} K,
                    $$
                    $K - |B^a_{\alpha}| \ge 0$, and thus $|B^a_{\beta}| \ge 0$.
                    Here $(*)$ is due to \Cref{adxeq:9-1}.
                    
                    \item The superset $\{i\in [u] \,\mid\, \pi_i(s_t) \neq a\} \setminus B_{\alpha}^a$ has cardinality $u - n_a(s_t) - |B_{\alpha}^a|$ and $|B^a_{\beta}| \le u - n_a(s_t) - |B_{\alpha}^a|$.
                \end{itemize}
                
                To this point, we can define the set of subpolicies to poison:
                $$
                    B^a := B^a_{\alpha} \cup B^a_{\beta},
                $$
                and $|B^a| = |B^a_{\alpha}| + |B^a_{\beta}| \le K$.
                
                In a similar fashion as the attack construction in proof of \Cref{prop:ppa-radius-tightness}, for each $i \in B^a$, we locate its corresponding partitioned dataset $D_i$ for training subpolicy $\pi_i^a$.
                We inset one trajectory $p_i^a$ to $D_i$ such that our chosen learning algorithm $\gM_0$ can train a subpolicy $\tpi_i^a = \gM_0(D_i \cup \{p_i^a\})$ such that $\tpi_i^a(s_t) = a$.
                For example, the trajectory could be $p_i^a = \{(s_t,a,s',\infty)\}$ where $s'$ is an arbitrary state that guarantees $p_i^a$ is hashed to partition $i$;
                and $\gM_0$ learns the action with maximum reward for the memorized nearest state.
                Then, the poisoned dataset
                $$
                    \wtilde D^a = \left( \bigcup_{i \in B^a} D_i \cup \{p_i^a\} \right) \cup \left( \bigcup_{i\in [u] \setminus B'} D_i \right).
                $$
                Thus, $\wtilde D^a$ is $|D \ominus \wtilde D^a| = |B^a| \le K$, \ie, the constructed attack's poisoning size is within $K$.
                
                We now analyze the action prediction of the poisoned policy $\wtilde \rlalgopolicy$.
                For action $a$, after poisoning, $\wtilde n_{a}(s_t) = n_{a}(s_t) + |B^a| = n_a(s_t) + \min\{K, u - n_a(s_t)\} = \min\{ n_a(s_t) + K, u\}$.
                If $\wtilde n_a(s_t) = u$, then all subpolicies vote for $a$, apparently $\wtilde \rlalgopolicy^a(s_t) = a$;
                otherwise, $\wtilde n_a(s_t) = n_a(s_t) + K$.
                In this case,
                for any action $a' \in C^a$, since we at least choose subpolicies in $B_{a'}^a$ and change their action prediction to $a$, the aggregated action count after poisoning is $\wtilde n_{a'}(s_t) \le n_{a'}(s_t) - |B_{a'}^a| = n_{a'}(s_t) - t_{a,a'} = n_{a'}(s_t) - n_{a'}(s_t) + n_a(s_t) + K - \1[a' < a] = n_a(s_t) + K - \1[a'< a] = \tilde n_a(s_t) - \1[a' < a]$.
                Thus, $a'$ has lower priority to be chosen than $a$.
                For any action $a' \notin C^a$ and $a' \neq a$, by the definition of $C^a$, $t_{a,a'} = n_{a'}(s_t) - n_a(s_t) - K + \1[a' < a] \le 0$.
                After poisoning, the vote of $a'$ does not increase, \ie, 
                $\wtilde n_{a'}(s_t) \le n_{a'}(s_t) \le n_a(s_t) + K - \1[a' < a] = \wtilde n_{a}(s_t) - \1[a' < a]$.
                Thus, $a'$ also has lower priority to be chosen than $a$.
                In conclusion, we have $\wtilde \rlalgopolicy^a(s_t) = a$.
                
                To this point, for any $a\in A^T(K)$, we successfully construct the corresponding poisoned dataset $\wtilde D^a$ within poisoning size $K$ such that $\wtilde \rlalgopolicy^a(s_t)=a$, thus concludes the proof.
            \end{enumerate}
        \end{proof}
    
    \subsection{Possible Action Set in \rlalgotmp}
        \label{adxsubsec:proof-C7}
        \begin{proof}[Proof of \Cref{thm:action-set-tpa}]
            For ease of notation, we let $w = \min\{W, t+1\}$, so $w$ is the actual window size used at step $t$.
            We let $t_0 = t-w+1$, \ie, $t_0$ is the actual start time step for \rlalgotmp aggregation at our current step $t$.
            Now we can write chosen action at step $t$ without poisoning as $\rlalgotmppolicy(s_{t_0:t})$.
        
            We only need to prove the contrary: for any $a \in \gA \setminus A(K)$, within poisoning size $K$, the poisoned policy cannot choose $a$: $\wtilde \rlalgotmppolicy(s_{t_0:t}) \neq a$.
            
            According to \Cref{eq:action-set-tpa}, for such $a$, there exists $a' \neq a$ such that
            \begin{equation}
                \sum_{i=1}^K h_{a',a}^{(i)} \le \delta_{a',a} = n_{a'}(s_{t_0:t}) - n_a(s_{t_0:t}) - \1[a < a'].
                \label{adxeq:10-1}
            \end{equation}
            Suppose there exists such poisoning attack that lets $\wtilde \rlalgotmppolicy(s_{t_0:t}) = a$.
            This implies that for $a'$, after poisoning, we have
            \begin{equation}
                \wtilde n_{a'}(s_{t_0:t}) - \wtilde n_{a'}(s_{t_0:t}) - \1[a' < a] < 0,
                \label{adxeq:10-2}
            \end{equation}
            where $\wtilde n_a$ is the aggregated action count after poisoning.
            Since the poisoning size is within $K$, it can affect at most $K$ subpolicies.
            We let $B \subseteq [u], |B| \le K$ to represent the affected subpolicy set.
            Therefore,
            \begin{align*}
                & \wtilde n_{a'}(s_{t_0:t}) - \wtilde n_{a}(s_{t_0:t}) - \1[a' < a] \\
                = & \underbrace{n_{a'}(s_{t_0:t}) - n_{a}(s_{t_0:t}) - \1[a' < a]}_{\delta_{a',a}} + (\wtilde n_{a'}(s_{t_0:t}) - n_{a'}(s_{t_0:t})) - (\wtilde n_{a}(s_{t_0:t}) - n_{a}(s_{t_0:t})) \\
                = & \delta_{a',a} + \sum_{i\in B} \left(
                    \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})=a', \pi_i(s_{t-j}) \neq a'] - \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})\neq a', \pi_i(s_{t-j}) = a']
                \right) \\
                & - \sum_{i\in B} \left(
                    \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})=a, \pi_i(s_{t-j}) \neq a] - \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})\neq a, \pi_i(s_{t-j}) = a]
                \right) \\
                \ge & \delta_{a',a} - \sum_{i \in B} \left( \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})\neq a', \pi_i(s_{t-j})=a'] + \sum_{j=0}^{w-1} \1[\tpi_i(s_{t-j})=a, \pi_i(s_{t-j}) \neq a] \right) \\
                \ge & \delta_{a',a} - \sum_{i \in B} \left( \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})=a'] + \sum_{j=0}^{w-1} \1[\pi_i(s_{t-j})\neq a] \right) \\
                = & \delta_{a',a} - \sum_{i \in B} \left( \sum_{j=0}^{w-1} \1_{i,a'}(s_{t-j}) + w - \sum_{j=0}^{w-1} \1_{i,a}(s_{t-j}) \right) \\
                = & \delta_{a',a} - \sum_{i \in B} h_{i,a',a} %\\
                \overset{(a)}{\ge} \delta_{a',a} - \sum_{i=1}^{|B|} h_{a',a}^{(i)} %\\
                \overset{(b)}{\ge}  \delta_{a',a} - \sum_{i=1}^{K} h_{a',a}^{(i)} %\\
                \overset{(c)}{\ge}  0.
            \end{align*}
            This contradicts with \Cref{adxeq:10-2}, and thus the assumption is falsified, \ie, there is no such poisoning attack that let $\wtilde \rlalgotmppolicy(s_{t_0:t}) = a$.
            In the above equations, $(a)$ is due to the fact that $h_{a',a}^{(i)}$ is a nonincreasing permutation of $\{h_{i,a',a}\}_{i=0}^{u-1}$.
            $(b)$ is due to the facts that $|B| \le K$ and $h_{a',a}^{(i)} \ge 0$.
            $(c)$ comes from \Cref{adxeq:10-1}.
        \end{proof}
        
    \subsection{Hardness for Computing Tight Possible Action Set in \rlalgotmp}
        \label{adxsubsec:proof-C8}
        \begin{proof}[Proof of \Cref{thm:np-complete-tpa-action-set}]
            By \Cref{def:possible-action-set}, the possible action set with minimum cardinality~(called minimal possible action set hereinafter) is unique.
            Otherwise, suppose $A$ and $B$ are both minimal possible action set, but $A \neq B$, then $A \cap B$ is a smaller and valid possible action set.
            Therefore, the oracle that returns the minimal possible action set, denoted by \textsf{MINSET}, can tell whether any action $a \in \mathsf{MINSET}$ and thus whether any action $a$ can be chosen by some poisoned policy $\wtilde \pi$ whose poisoning size is within $K$.
            In other words, the problem of determining whether an action $a$ can be chosen by some poisoned policy $\tpi$ whose poisoning size is within $K$, denoted by \textsf{ATTKACT}, is polynomially equivalent to \textsf{MINSET}: $\mathsf{MINSET} \equiv_P \mathsf{ATTKACT}$.
            Now, we show a polynomial reduction from the set cover problem to \textsf{ATTKACT}, which implies that our \textsf{MINSET} problem is an $\NP$-complete problem.
            
            The decision version of the set cover problem~\citep{karp1972reducibility}, denoted by \textsf{SETCOVER}, is a well-known $\NP$-complete problem and is defined as follows.
            The inputs are
            \begin{enumerate}[leftmargin=*]
                \item a universal set of $n$ elements: $\gU = \{u_1,u_2,\cdots,u_n\}$;
                \item a set of subsets of $\gU$: $\gV = \{V_1,\cdots,V_m\}, V_i \subseteq \gU, 1\le i\le m, \bigcup_{i=1}^m V_i = \gU$;
                \item a positive number $K \in \sR_+$.
            \end{enumerate}
            The output is a boolean variable $b$, indicating that whether there exists a subset $\gW \subseteq \gV, |\gW| \le K$, such that $\forall u_i\in \gU, \exists V\in \gW, u_i \in V$.
            Given an oracle to \textsf{ATTKACT}, we need to show \textsf{SETCOVER} can be solved in polynomial time, \ie, $\mathsf{SETCOVER} \le_{P} \mathsf{ATTKACT}$.
            
            \begin{itemize}[leftmargin=*]
                \item If $K \ge n$:\\
                We scan all sets $V_i \in \gV$. To being with, we have a record set $S \gets \emptyset$, and an answer set $\gW \gets \emptyset$. Whenever we encounter a set that contains a new element $u_i \notin S$, we put $\gW \gets \gW \cup \{V_j\}$, and record this element $S \gets S \cup \{u_i\}$. After one scan pass, $\gW$ covers all elements of $\gU$~(since $\bigcup_{j=1}^m V_j = \gU$), and $|\gW| \le n \le K$.
                Therefore, $\gW$ is a valid set cover.
                Since we can always find such $\gW$, we can directly answer \texttt{true}.
                
                \item If $K \ge m$:\\
                We can directly return $\gV$ as a valid set cover, since $\bigcup_{j=1}^m V_j = \gU$ and $|\gV| \le m \le K$.
                Thus, we can answer \texttt{true}.
                
                \item If $K < \min\{n, m\}$:\\
                This is the general case which we need to handle.
                Now we construct the \textsf{ATTKACT}$(K)$ problem so that we can trigger its oracle to solve \textsf{SETCOVER}.
                
                \begin{enumerate}
                    \item The poisoning size is $K$.
                    
                    \item The action space $\gA = \gU \cup \{b\} \cup \Gamma$ where $\Gamma := \{\#_1,\dots, \#_{m^2n}\}$. 
                    ($|\gA| = n + 1 + m^2n$.)
                    The sorting of actions is $u_1 < u_2 < \cdots < u_n < b < \#_1 < \cdots < \#_{m^2n}$.
                    
                    \item The subpolicies are $\{\pi^a_j\}_{j=1}^m \cup \{\pi^b_i, \pi^c_{i,j} \,\mid\, 1\le i\le n, 1\le j\le K-1\}$, where $\pi^a_j$ corresponds to $V_j \in \gV$, and $\pi^b_i, \pi^c_{i,j}$ correspond to $u_i \in \gU$.
                    (Number of subpolicies $u = m + Kn \le m + n^2$.)
                    
                    \item The current time step is $t = nm$, and the window size $W = nm$.
                    % For convenience, we let $\pi(t)$ to represent the subpolicy $\pi$'s action prediction for the state $s_t$ at time step $t$.
                    
                    \item The input action is $b$, \ie, asking whether $b$ can be chosen by some poisoned \rlalgotmp policy, \ie, $\wtilde \rlalgotmppolicy(s_{1:t}) = b$, if the poisoning size is within $K$.
                \end{enumerate}
                Now, we construct the states at each step $t$~($1 \le t \le nm$) so that the subpolicies' action predictions at these steps are as follows.
                \begin{enumerate}
                    \item Count the appearing time of each $u_i$ in $\gV$, and denote it by $c_i$: $c_i = \sum_{j=1}^m \1[u_i \in V_j]$.
                    For each $u_i$, select a $V_{j_0}$ that contains $u_i$, and in the corresponding $\pi_{j_0}^a$, assign $m-c_i+1$ steps to predict $u_i$;
                    for all other $V_j$ that contains $u_i$, in the corresponding $\pi_j^a$, assign one step to predict $u_i$.
                    
                    \item After this process, each $\pi_j^a$ at least has one time step whose action prediction is $u_i$ for each $u_i \in V_j$.
                    Among all $\{\pi_j^a\}_{j=1}^m$ and all time steps $1 \le t \le nm$, $mn$ step-action cells are filled, and the remaining $(m^2n-mn)$ cells are filled by $\#_l \in \Gamma$ sequentially.
                    
                    \item For each $\pi_i^b$, arbitrarily select $W-m$ time steps to assign action prediction as $u_i$; and fill in other $m$ time steps by remaining $\#_l \in \Gamma$ sequentially.
                    
                    \item For each $\pi_{i,j}^c$, for all time steps, let the action prediction be $u_i$.
                \end{enumerate}
                As we can observe, the number of actions, the number of subpolicies, and the window size are all bounded by a polynomial of $n$ and $m$.
                Therefore, such construction can be done in polynomial time.
                
                We then show $\mathsf{SETCOVER}=\texttt{true} \iff \exists K', b \in \mathsf{ATTKACT}(K'), 1\le K' \le K$.
                \begin{itemize}
                    \item $\Longrightarrow$: \\
                    Suppose the covering set is $\gW \subseteq \gV$, 
                    we denote $K'$ to $|\gW|$,
                    and construct the \textsf{ATTKACT} problem with poisoning size $K'$ as described above.
                    
                    We can construct a poisoning strategy to let $\wtilde \rlalgotmppolicy(s_{1:nm}) = b$,
                    The poisoning strategy is to find out $\pi_j^a$ for each $V_j \in \gW$, and to let them predict action $b$ throughout all time steps: $\wtilde \pi_j^a(s_t') = b, 1\le t' \le nm$.
                    
                    After poisoning, the aggregated action count $\wtilde n_{b}(s_{1:nm}) = |\gW| \times nm = K'nm$.
                    Since $\gW$ covers every $u_i \in \gU$, for each $u_i\in \gU$ there exists a set $V_j \ni u_i$, whose corresponding $\wtilde \pi_j^a$ is poisoned to predict $b$.
                    Thus, $\wtilde n_{u_i}(s_{1:nm}) < n_{u_i}(s_{1:nm}) = m + (W-m) + W \times (K'-1) = WK' = K'nm$.
                    For any $\#_l \in \Gamma$, $\wtilde n_{\#_l}(s_{1:nm}) \le n_{\#_l}(s_{1:nm}) = 1$.
                    In summary,
                    $$
                        \wtilde n_{u_i}(s_{1:nm}) < K'nm,
                        \wtilde n_b(s_{1:nm}) = K'nm,
                        \wtilde n_{\#_l}(s_{1:nm}) = 1.
                    $$
                    Thus, after \rlalgotmp aggregation, the poisoned policy $\wtilde \rlalgotmppolicy(s_{1:nm}) = b$, and therefore $b \in \mathsf{ATTKACT}(K')$.
                    
                    \item $\Longleftarrow$: \\
                    Suppose it is $K'$ that let $b \in \mathsf{ATTKACT}(K')$, which implies that there exists such a poisoning attack within size $K'$ that misleads the poisoned policy to $b$: $\wtilde \rlalgotmppolicy(s_{1:nm}) = b$.
                    Since the poisoning size is $K'$, after poisoning the aggregated action count 
                    $$
                    \wtilde n_b(s_{1:nm}) \le K'W = K'nm.
                    $$
                    For each $u_i \in \gU$, since $n_{u_i}(s_{1:nm}) = m + (W-m) + W \times (K'-1) = K'nm$, we always have 
                    \begin{equation}
                        \wtilde n_{u_i}(s_{1:nm}) \overset{(*)}{<} \wtilde n_b(s_{1:nm}) \le n_{u_i}(s_{1:nm}),
                        \label{adxeq:11-1}
                    \end{equation}
                    where $(*)$ is due to the condition of successful attack.
                    We denote the set of poisoned subpolicies by $\Pi$~($|\Pi| \le K'$). Therefore, 
                    \Cref{adxeq:11-1} implies that for each $u_i \in \gU$, there exists at least one subpolicy 
                    \begin{equation}
                        \pi_{u_i}' \in \Pi, \pi_{u_i}' \in \{\pi_j^a \,\mid\, u_i\in V_j\} \cup \{\pi_i^b\} \cup \{\pi_{i,j}^c \,\mid\, 1\le j\le K-1\}
                        \label{adxeq:11-2}
                    \end{equation}
                    that is poisoned by the attack, otherwise the aggregated vote $\wtilde n_{u_i}$ cannot change.
                    
                    We partition $\Gamma$ by $\Gamma^a$ and $\Gamma^{bc}$, where
                    $$
                        \Gamma^a = \Gamma \cap \{\pi_j^a\}_{j=1}^m,
                        \Gamma^b = \Gamma \cap \{\pi_i^b, \pi_{i,j}^c \,\mid\, 1\le i\le n, 1\le j\le K-1\}.
                    $$
                    We construct additional poisoning set $\Gamma^a_+$ following this process:
                    In the beginning, $\Gamma^a_+ \gets \emptyset$.
                    For each $u_i \in \gU$, if $\Gamma^a \cap \{\pi_j^a \,\mid\, u_i \in V_j\}$ is not empty, skip.
                    Otherwise, according to \Cref{adxeq:11-2}, $\Gamma^b \cap \{\pi_i^b, \pi_{i,j}^c \,\mid\, 1\le j\le K-1\}$ is not empty.
                    In this case, we find an arbitrary covering set of $u_i$, namely $V_{j_0} \ni u_i$, and put $\pi_{j_0}^a$ into $\Gamma^a_+$.
                    When the process terminates, we find that for each $u_i\in \gU$,
                    \begin{equation}
                        (\Gamma^a \cup \Gamma^a_+) \cap \{\pi_j^a \,\mid\, u_i \in V_j\} \neq \emptyset.
                        \label{adxeq:11-3}
                    \end{equation}
                    Following the mapping $\{\pi_j^a\}_{j=1}^m \longleftrightarrow \{V_j \,\mid\, 1\le j\le m\} = \gV$, the subset $(\Gamma^a \cup \Gamma^a_+) \subseteq \{\pi_j^a\}_{j=1}^m$ can be mapped to $(\gW^a \cup \gW^a_+) \subseteq \gV$.
                    From \Cref{adxeq:11-3}, $(\gW^a \cup \gW^a_+)$ is a valid set cover for $\gU$.
                    We now study the cardinality of this set cover.
                    From the process, we know that every $V_{j_0} \in \gW^a_+$ corresponds to a different set in $\Gamma^b$.
                    Thus, $|\gW^a_+| \le |\Gamma^b|$, which implies that
                    $$
                        |\gW^a \cup \gW^a_+|
                        \le
                        |\gW^a| + |\gW^a_+|
                        \le |\Gamma^a| + |\Gamma^b|
                        = |\Gamma| \le K'.
                    $$
                    To this point, we successfully construct a set cover within cardinally $K' \le K$ that covers $\gU$, so $\mathsf{SETCOVER}=\mathtt{true}$.
                \end{itemize}
                Therefore, we can check whether $\mathsf{SETCOVER}=\mathtt{true}$ by iterating $K'$ from $1$ to $K$~($< \min\{n,m\}$ iterations), constructing the $\mathsf{ATTKACT}(K')$ problem, and querying the oracle.
                The whole process can be done in polynomial time assumping $O(1)$ computation time of the $\mathsf{ATTKACT}(K')$ oracle.
            \end{itemize}
            To this point, we have shown $\mathsf{SETCOVER} \le_{P} \mathsf{ATTKACT}$.
            On the other hand, an undeterminisitic Turing machine can  try different poisoning strategies by branching on whether to poison current subpolicy and what actions to be assigned to each poisoned subpolicy.
            The decision of whether the poisoning is successful can be done in polynomial time and $b\in \mathsf{ATTKACT}(K)$ corresponds to the existence of successfully attacked branches.
            Thus, $\mathsf{ATTKACT} \in \mathsf{NP}$.
            Given that \textsf{SETCOVER} is an $\NP$-complete problem, so does \textsf{ATTKACT} and \textsf{MINSET}~(since $\mathsf{MINSET} \equiv_P \mathsf{ATTKACT}$).
        \end{proof}
        
    \subsection{Possible Action Set in \rlalgodyntmp}
        \label{adxsubsec:proof-C9}
        \begin{proof}[Proof of \Cref{thm:action-set-dtpa}]
            For ease of notation, we assume that $W_{\max} \le t+1$, and otherwise we let $W_{\max} \gets t+1$.
            We let $t_0 = \max\{t - W_{\max} + 1, 0\}$ be the start time step of the maximum possible window.
            
            We only need to prove the contrary: for any $a \in \gA \setminus A(K)$, within poisoning size $K$, the poisoned policy cannot choose $a$: $\wtilde \rlalgodyntmppolicy(s_{t_0:t}) \neq a$.
            We prove by contradiction: we assume that there exists such a poisoning attack within poisoning size $K$ that lets $\wtilde \rlalgodyntmppolicy(s_{t_0:t}) = a$.
            From the expression of $A(K)$~(\Cref{eq:action-set-dtpa}), $a \neq a_t = \rlalgodyntmppolicy(s_{t_0:t})$.
            Suppose the selected time window before the attack is $W'$~(selected according to \Cref{eq:dtpa-agg-1} based on $\Delta_t^W$ and $n_a$), and the selected time window after the attack is $\wtilde W'$~(selected according to \Cref{eq:dtpa-agg-1} based on $\wtilde \Delta_t^W$ and $\wtilde n_a$).
            \begin{itemize}[leftmargin=*]
                \item If $\wtilde W' = W'$: \\
                Suppose we use the \rlalgotmp aggregation policy with window size $W = W'$ instead of current \rlalgodyntmp aggregation policy,
                then we will have $\rlalgotmppolicy(s_{t-W'+1:t}) = a_t$ and $\wtilde \rlalgotmppolicy(s_{t-W'+1:t}) = a$.
                Thus, according to the definition of possible action set~(\Cref{def:possible-action-set}), $a \in A(K)$ where $A(K)$ is defined by \Cref{eq:action-set-tpa} in \Cref{thm:action-set-tpa}.
                This implies that $a \in A(K)$ where $A(K)$ is defined by \Cref{eq:action-set-dtpa}, which contradicts the assumption that $a \in \gA \setminus A(K)$.
                
                \item If $\wtilde W' \neq W'$: \\
                According to the definition in \Cref{eq:action-set-dtpa}, 
                $$
                    \min_{1\le W^* \le W_{\max}, W^* \neq W', a'' \neq a_t} L_{a,a''}^{W^*,W'} > K.
                $$
                We define $a_t^\# = \argmax_{a_0 \neq a_t} \wtilde n_{a_0}(s_{t-W'+1:t})$.
                Then, the above equation implies that
                $$
                    L_{a,a_t^\#}^{\wtilde W', W'} > K
                $$
                and thus
                \begin{equation*}
                    \sum_{i=1}^{L_{a,a_t^\#}^{\wtilde W', W'}}
                    g^{(i)}
                    + W'(n_a^{\wtilde W'} - n_{a^\#}^{\wtilde W'}) - \wtilde W'(n_{a_t}^{W'} - n_{a_t^\#}^{W'}) - \1[a > a_t] < 0.
                \end{equation*}
                Since $g^{(i)} \ge 0$ by definition~(\Cref{eq:L-2}),
                \begin{equation}
                    \sum_{i=1}^K
                    g^{(i)}
                    + W'(n_a^{\wtilde W'} - n_{a^\#}^{\wtilde W'}) - \wtilde W'(n_{a_t}^{W'} - n_{a_t^\#}^{W'}) - \1[a > a_t] < 0,
                    \label{adxeq:12-1}
                \end{equation}
                where $a^\# = \argmax_{a_0\neq a', a_0\in \gA} n_{a_0}(s_{t-\wtilde W'+1:t})$ and $n_a^w$ is a shorthand of $n_a(s_{t-w+1:t})$.
                
                Following the derivation from \Cref{adxeq:6-5} to $(a)$, we have
                \begin{equation*}
                    \sum_{i=1}^K
                    g^{(i)}
                    + W'(n_a^{\wtilde W'} - n_{a^\#}^{\wtilde W'}) - \wtilde W'(n_{a_t}^{W'} - n_{a_t^\#}^{W'}) - \1[a > a_t]
                    \ge
                    W'(\wtilde n_a^{\wtilde W'} - \wtilde n_{a^\#}^{\wtilde W'}) - \wtilde W'(\wtilde n_{a_t}^{W'} - \wtilde n_{a_t^\#}^{W'}) - \1[a > a_t].
                \end{equation*}
                Combined with \Cref{adxeq:12-1},
                \begin{equation}
                    W'(\wtilde n_a^{\wtilde W'} - \wtilde n_{a^\#}^{\wtilde W'}) - \wtilde W'(\wtilde n_{a_t}^{W'} - \wtilde n_{a_t^\#}^{W'}) - \1[a > a_t] < 0.
                    \label{adxeq:12-2}
                \end{equation}
                
                On the other hand,
                the successful attack assumption, \ie, $\wtilde \rlalgodyntmppolicy(s_{t_0:t}) = a$ and $\rlalgodyntmppolicy(s_{t_0:t}) = a_t$, implies that
                \begin{equation}
                    \wtilde \Delta_t^{\wtilde W'} = \dfrac{\wtilde n_a^{\wtilde W'} - \wtilde n_{a^{(2)}}^{\wtilde W'}}{\wtilde W'}
                    >
                    \dfrac{\wtilde n_{a_{W'}}^{W'} - \wtilde n_{a_{W'}^{(2)}}^{W'}}{W'} = \wtilde \Delta_t^{W'},
                    \label{adxeq:12-3}
                \end{equation}
                where ``$>$'' is ``$\ge$'' if $a < a_t$.
                In the above equation,
                $$
                    a^{(2)} = \argmax_{a_0\neq a,a_0\in \gA} \wtilde n_{a_0}^{\wtilde W'}, 
                    a_{W'} = \argmax_{a_0\in \gA} \wtilde n_{a_0}^{W'}, 
                    a_{W'}^{(2)} = \argmax_{a_0\neq a_{W'},a_0\in \gA} \wtilde n_{a_0}^{W'}.
                $$
                Intuitively, after poisoning, $a^{(2)}$ is the runner-up action at window $\wtilde W'$, $a_{W'}$ is the action at window $W'$, and $a_{W'}^{(2)}$ is the runner-up action at window $W'$.
                We rewrite \Cref{adxeq:12-3} to
                \begin{equation}
                    W'(\wtilde n_a^{\wtilde W'} - \wtilde n_{a^{(2)}}^{\wtilde W'}) \ge \wtilde W' (\wtilde n_{a_{W'}}^{W'} - \wtilde n_{a_{W'}^{(2)}}^{W'}) + \1[a > a_t].
                    \label{adxeq:12-4}
                \end{equation}
                We have the following two observations:
                \begin{enumerate}
                    \item $
                        \wtilde n_a^{\wtilde W'} - \wtilde n_{a^{\#}}^{\wtilde W'}
                        \ge 
                        \wtilde n_a^{\wtilde W'} - \wtilde n_{a^{(2)}}^{\wtilde W'}$, since $a$ is the top action and $a^{(2)}$ is the runner-up action and their margin should be the smallest.
                    
                    \item $\wtilde n_{a_{W'}}^{W'} - \wtilde n_{a_{W'}^{(2)}}^{W'} \ge \wtilde n_{a_t}^{W'} - \wtilde n_{a_t^{\#}}^{W'}$,
                    because 1)~if $a_t = a_{W'}$, LHS equals to RHS; 2)~if $a_t \neq a_{W'}$, LHS $\ge 0$ and RHS $\le 0$.
                \end{enumerate}
                Plugging these two observations to two sides of \Cref{adxeq:12-4}, we get
                \begin{equation}
                     W'(\wtilde n_a^{\wtilde W'} - \wtilde n_{a^{\#}}^{\wtilde W'}) \ge \wtilde W' (\wtilde n_{a_t}^{W'} - \wtilde n_{a_t^{\#}}^{W'}) + \1[a > a_t].
                    \label{adxeq:12-5}
                \end{equation}
                This contradicts with \Cref{adxeq:12-2}.
            \end{itemize}
            Since in both cases, we find contradictions.
            Now we can conclude that for any $a \in \gA \setminus A(K)$, within poisoning size $K$, the poisoned policy cannot choose $a$: $\wtilde \rlalgodyntmppolicy(s_{t_0:t}) \neq a$.
        \end{proof}
        
    % \subsection{General Hardness of Tight Cumulative Reward Certification}
    %     \begin{proof}[Proof of \Cref{thm:general-hardness-reward}]
    %         \TODO
    %     \end{proof}


\section{Additional Experimental Details}
    \label{adxsec:exp}
    
    \subsection{Details of the Offline RL algorithms and Implementations}
        \label{adxsubsec:rl-algos}
        
        We experimented with three offline RL algorithms: DQN~\citep{mnih2013playing}, QR-DQN~\citep{dabney2018distributional}, and C51~\citep{bellemare2017distributional}. 
        The first one is the standard baseline, while the latter two are distributional RL algorithms which show SOTA results in offline RL tasks.
        We first briefly introduce the algorithm ideas, followed by the implementation details.
        
        \textbf{Algorithm Ideas.}\quad
        The core of Q-learning~\citep{watkins1992q} is the Bellman optimality equation~\citep{bellman1966dynamic}
        \begin{align}
            Q^{\star}(s, a)=\mathbb{E} R(s, a)+\gamma \mathbb{E}_{s^{\prime} \sim P} \max _{a^{\prime} \in \mathcal{A}} Q^{\star}\left(s^{\prime}, a^{\prime}\right),
        \end{align}
        where a parameterized $Q^\theta$ is adopted to approximate the optimal $Q^\star$ and iteratively improved.
        In DQN~\citep{mnih2013playing} specifically, the parameterization is achieved by using a convolutional neural network~\citep{lecun1998gradient}.
        In contrast to estimating the mean action value $Q^\pi(s,a)$ in DQN, distributional RL algorithms estimate a density over the values of the state-action pairs. The distributional Bellman optimality can be expressed as follows:
        \begin{align}
            Z^\star(s, a) \stackrel{D}{=} r +\gamma Z^\star\left(s^{\prime}, \operatorname{argmax}_{a^{\prime} \in \mathcal{A}} Q^{\star}\left(s^{\prime}, a^{\prime}\right)\right) 
             \text { where } r \sim R(s, a), s^{\prime} \sim P(\cdot \mid s, a).
        \end{align}
        Concretely, QR-DQN~\citep{dabney2018distributional} approximates the density $D^\star$ with a uniform mixture of $K$ Dirac delta functions, while C51~\citep{bellemare2017distributional} approximates the density using a categorical distribution over a set of anchor points.
        
        \textbf{Implementation Details.}\quad
        For training the subpolicies using offline RL training algorithms, we use the code base of~\citet{agarwal2020optimistic}.
        The configuration files containing the detailed hyperparameters can be found at their public repository \url{https://github.com/google-research/batch_rl/tree/master/batch_rl/fixed_replay/configs}.
        For the three methods DQN, QR-DQN, and C51, the names of the configuration files are \texttt{dqn.gin}, \texttt{quantile.gin}, and \texttt{c51.gin}, respectively.
        On each partition, we train the subpolicy for $50$ epochs.
        
    \subsection{Concrete Experimental Procedures}
        \label{adxsubsec:exp-proc}
        \looseness=-1
        We conduct experiments on two Atari 2600 games, Freeway and Breakout from OpenAI Gym~\citep{brockman2016openai}, and one autonomous driving environment Highway~\citep{highway-env}, following~\Cref{sec:main}.
        
        Concretely, in the \textbf{training} stage, we first partition the training dataset into $u$ partitions ($u=30$, $50$, or $100$) by using the hash function $h(\tau)$ pre-defined in each environment. 
        Let $s^i$ be the $i$-th value in the state representation and $d$ be the dimensionality of the state.
        In \textit{Atari games} where the state is the game frame, $h(\tau)$ is defined as the sum of all pixel values of all frames in the trajectory $\tau$, \ie, $h(\tau) = \sum_{s \in \tau} \sum_{i \in [d]} s^i$. 
        In \textit{Highway} where the state is a floating point number scalar containing the positions and velocities of all vehicles, we define $h(\tau) = \sum_{s\in \tau}\sum_{i \in [d]} f(s^i)$ where $f: \mathbb{R} \rightarrow \mathbb{Z}$ is a deterministic function that maps the given float value to integer space. Concretely, we take $f(x)$ as the the sum of the higher $16$ bits and the lower $16$ bits of its $32$-bit representation under IEEE $754$ standard~\citep{ieee1985ieee}.
        % for each number in a state, we first calculate the sum of the higher $16$ bits and the lower $16$ bits of its IEEE $754$ $32$-bit representation. Then we define $h(\tau)$ as the sum of all numbers of all states in the trajectory $\tau$.
        We then train the subpolicies on the partitions with offline RL training algorithm $\gM_0 \in $ \{DQN~\citep{mnih2013playing}, QR-DQN~\citep{dabney2018distributional}, C51~\citep{bellemare2017distributional}\}.
        The detailed description of the algorithms can be found in~\Cref{adxsubsec:rl-algos}.
        
        In the \textbf{aggregation} stage, we apply the three proposed aggregation protocols (\rlalgo~(\Cref{thm:ppa-radius}), \rlalgotmp~(\Cref{thm:tpa-radius}), and \rlalgodyntmp~(\Cref{thm:dtpa-radius})) on the trained $u$ subpolicies and derive the aggregated policies $\rlalgopolicy$, $\rlalgotmppolicy$, and $\rlalgodyntmppolicy$ accordingly. 
        
        Finally, in the \textbf{certification} stage, for each aggregated policy, we provide the per-state action and cumulative reward certification following our theorems. 
        When certifying the \textit{per-state action}, we constrain the maximum trajectory length $H=1000$ for Atari games and $H=30$ for Highway (which is the full length in Highway) and report results averaged over $20$ runs;
        for the \textit{cumulative reward} certification, we adopt the trajectory length $H=400$ for evaluating Freeway, $H=75$ for Breakout, and $H=30$ for Highway.
        
        \textbf{Configuration of Trajectory Length $H$.}\quad
        For \textit{Atari games}, we do not evaluate the full episode length (up to tens of thousands steps), since our goal is to compare the relative certified robustness of different RL algorithms, and the evaluation on relatively short trajectory is sufficient under affordable computation cost.
        Moreover, different episodes in Atari games are oftentimes of different lengths; thus it is necessary that we restrict the episode length to enable a fair comparison.
        For \textit{Highway}, we evaluate on the full episode ($H=30$) where we can efficiently achieve effective comparisons. 



\section{Additional Evaluation Results and Discussions}
    \label{adxsec:exp-results}
    
    \subsection{Benign Empirical Performance}
        \label{adxsubsec:emp-reward}
        % \input{tables/tab_empirical_reward}
        
        \input{tables/tab_empirical_reward_full}
        
        We present the benign empirical cumulative rewards of the three aggregation protocols (\rlalgo, \rlalgotmp, and \rlalgodyntmp) applied on subpolicies trained using three offline RL algorithms (DQN, QR-DQN, and C51) in~\Cref{tab:emp-reward-full}.
        The cumulative reward is obtained by running a trajectory of maximum length $H$ and accumulating the reward achieved at each time step. 
        
        We discuss the conclusions on multiple levels.
        We choose $H=1000$ for Atari games and $H=30$ for Highway environment and report results averaged over $20$ runs.
        On the \textbf{RL algorithm} level, we see that QR-DQN achieves the highest score in most cases.
        On the \textbf{aggregation protocol} level, temporal aggregation enhances the performance on Freeway while dampens the performance on Breakout and Highway.
        We particularly note that the results obtained by using temporal aggregation (\rlalgotmp and \rlalgodyntmp) gives significantly smaller variance compared to the single-step aggregation \rlalgo, especially in Breakout. This implies that temporal aggregation can help stabilize the policy.
        However, the conclusion does not hold in Highway, which is an interesting phenomenon that is worth investigating.
        On the \textbf{partition number} level, a larger partition number can give slightly better results.
        On the \textbf{environment} level, Freeway is simpler and more stable than Breakout and Highway.


    \subsection{Comparison of \sysname with Standard Training}
        \label{adxsubsec:cmp-training}
        
        \input{fig_desc/fig_training}
        
        \input{tables/tab_testing_cmp}
        
        We provide additional experimental results on the comparison between the empirical performance of our \sysname and the standard training in terms of the \textit{convergence speed} (\Cref{fig:training-cmp}) and \textit{policy quality} (\Cref{tab:testing-cmp}).
        
        In~\Cref{fig:training-cmp}, we aim to show the comparison of the convergence speed. For \textit{our proposed training}, we plot all training curves of the sampled $5$ subpolicies in blue, where each subpolicy is trained on one partition of the dataset. (We do not plot all $50$ curves for visual clarity.) 
        For \textit{standard training}, we plot the training curve of the standard policy in red, where the single policy is trained on the entire dataset. We see that on \textbf{Freeway}, most subpolicies converge slower than the standard policy, but will reach similar convergence value as the standard training one; while there also exist a few subpolicies that fail to be trained. On \textbf{Breakout}, within $50$ epochs, we observe substantial fluctuation for the training curves of all the policies, as well as large variance for the achieved reward at the last epoch.
        Thus, on these two \textbf{Atari games}, we cannot draw conclusions w.r.t. the convergence. 
        Given more computational resources to run more epochs, we would be able to draw more informative conclusions.
        In contrast, on \textbf{Highway}, all subpolicies display similarly good convergence properties, showing comparable convergence speed and value with the standard training on the entire dataset.
        
        
        In~\Cref{tab:testing-cmp}, we aim to compare the policy quality of the aggregated policy derived in our \sysname framework (\ie, \rlalgo, \rlalgotmp, and \rlalgodyntmp) with the policy obtained from standard training. We see that on \textbf{Freeway}, our three protocols achieve comparable results with the policy obtained by standard training on the entire dataset; on \textbf{Breakout}, although the quality of our obtained policies is lower, our policies are much more stable with significantly lower variance than the standard training; on \textbf{Highway}, only PARL obtains comparable results to the standard training policy, indicating the lack of temporal continuity in this environment.

    
    \subsection{More Analytical Statistics for \rlalgodyntmp}
        \label{adxsubsec:stat-dparl}
        
        \input{tables/tab_ave_window_size}
        \textbf{Selected Window Size.}\quad
        We provide the mean and variance for the selected window sizes in \rlalgodyntmp in~\Cref{tab:ave-window-size}.
        In our experiments, the \textit{maximum window size} $W_{\rm max}=5$, while the \textit{average selected window sizes} are all around half of the maximum value. Thus, the average certification time is expected to be much smaller compared with the worst-case time complexity.
    
        \input{tables/tab_runtime}
        \textbf{Running Time.}\quad
        We provide the running time in~\Cref{tab:runtime}.
        Specifically, we compare the running time of \rlalgodyntmp ($W_{\rm max}=5$) applied on $u=30$ or $50$ subpolicies trained using \textit{offline RL algorithm} DQN with the \textit{normal testing} which tests the runtime of a single trained DQN policy without using our framework. As we have shown in the remark of~\Cref{thm:dtpa-radius} in~\Cref{subsec:cert-radius}, the time complexity of \rlalgodyntmp is $O\left(W_{\max }^{2}|\mathcal{A}|^{2} u+W_{\max }|\mathcal{A}|^{2} u \log u\right)$. In~\Cref{tab:runtime}, we also see that the runtime of \rlalgodyntmp scales roughly quasilinearly with the number of subpolicies $u$, and quadratically with the action set size $|\cal A|$, which is $3$ for Freeway and $4$ for Breakout.
        We omit the runtime for Highway, since the horizon length, the environment type, and the neural network size are all different for Highway and Atari games.
        % \chejianm{and $5$ for Highway}. \chejian{not very clear in Highway?}


        
    \subsection{Maximum Tolerable Poisoning Threshold vs. Total Trajectory Number}
        \label{adxsubsec:cmp-traj-num}
        We provide the total number of trajectories in the offline dataset used for training the environments Freeway, Breakout and Highway below, as well as the corresponding ratio of the maximum tolerable poisoning threshold w.r.t. the total number of trajectories. 
        For \textbf{Freeway}, the total number of trajectories in the entire offline dataset is 121,892, and the ratio ($\max \widebar K_t$ / \# total trajectories) is 0.0002; 
        for \textbf{Breakout}, the number is 209,049, and the ratio is 0.0001.
        % \chejianm{for \textbf{Highway}, the number is $4,532,126$, and the ratio is $0.00001$.}
        We emphasize that, as shown in previous work on probable defense against poisoning in supervised learning~\citep{levine2020deep}, the number of instances they can certify is also not high especially for challenging tasks (\eg, certifying 20 instances on the dataset GTSRB in~\citet{levine2020deep}, attaining the ratio 0.0005), which may imply the intrinsic difficulty of certifying against poisoning attacks. Given such difficulty, we already achieve reasonable certification as the first work on certified robust RL against poisoning, and we hope future works can further improve upon our results.
        
    
    \subsection{Comparison of Freeway, Breakout, and Highway}
        \label{adxsubsec:cmp-games}

        Freeway and Breakout are two typical types of games with distinctive game properties.
        Freeway is a simple game where the agent aims to cross the road and avoid the traffic. In most of the time steps, the agent would take the ``forward'' action; only when there is a need to avoid the traffic will the agent stop and wait.
        In comparison, the game Breakout involves more complicated interactions between the paddle and the environment. The paddle position and velocity both play important roles in order to catch and bounce the ball at an appropriate angle, which requires a frequent switch of the paddle moving direction. Similar to Breakout, as an autonomous driving environment, Highway requires the agent to accurately analyze the rapidly changing environment around it and react quickly, leading to frequent changes in vehicle's actions.
        
        Given the properties of the environments, we note that in Freeway, adjacent time steps may share consistent action selections, which is not necessarily true in the Breakout and Highway.
        Thus, it would be expected to be beneficial to consider the past history for making the current decision in Freeway, while the past history may interfere with the action selection in Breakout and Highway.
        
        \noindent\textbf{Comparisons of Bottleneck states in Atari Games.}\quad
        In Breakout, the game goal is to control the paddle so that the ball is bounced to hit the brick. There are clearly very different stages in the Breakout game, \eg, when the ball is flying towards the paddle and when it is bounced back. An example of the \textit{bottleneck state} is when the ball is approaching the paddle. The poisoning behavior may lead to the disastrous effect that the policy learns to control the paddle to slide in the opposite direction of the ball at such bottleneck states, while other states may not be as vulnerable. In comparison, in Freeway, the game goal is to control the agent to cross the road while avoiding the traffic. The agent is faced with similar traffic conditions everywhere on the road, and can make stable choices regardless of the complex situation. Thus there are very few \textit{bottleneck states}.
        
        \input{tables/tab_action_change}
        \noindent\textbf{A Study on the Frequency of Action Change in Highway.}\quad
        In \Cref{tab:action_change}, we present the action change ratio (\# action changes / trajectory length) in Highway environment. 
        Comparing among the aggregation protocols, we first note that the single-step aggregation policy $\rlalgopolicy$ frequently alters actions as the reaction to the rapidly changing driving environment, while the temporal aggregation protocol $\rlalgotmppolicy$ changes actions less frequently. This is because in \rlalgotmp, the agent is explicitly forced to take stable actions based on a fixed window size.
        Second, comparing the action change ratio with the benign empirical performance in~\Cref{tab:emp-reward-full}, we observe that $\rlalgopolicy$ and $\rlalgotmppolicy$ achieves the highest and lowest empirical performance respectively, which indicates the correlation between action change ratio with the achieved empirical reward. Specifically, in \rlalgotmp, the action change is limited as a result of the enforced window size, leading to the limited benign performance.
        % On the \textbf{aggregation protocol} level, the single-step aggregation \rlalgo is the most active method, frequently reacting to the rapidly changing driving environment, which achieves the highest benign empirical performance as shown in \Cref{tab:emp-reward-full}. In TPARL, on the other hand, the agent is forced to take stable actions based on a fixed window size, which reduces the change ratio and limits the benign performance.
        
        
    \subsection{Full Results of Robustness Certification for Per-State Action Stability}
        \label{adxsubsec:full-action}

        \input{fig_desc/fig_action_full_cum}
        \input{fig_desc/fig_action_full_cum_highway}
        
        \input{tables/tab_ave_poison_size}
        As a complete set of results for per-state action certification apart from~\Cref{fig:statewise} in~\Cref{subsec:eval-action}, we present the entire cumulative histogram of \textit{tolerable poisoning thresholds} in~\Cref{fig:statewise-full} and~\Cref{fig:statewise-full-highway}, together with the \textit{average tolerable poisoning thresholds} in~\Cref{tab:ave-poison-size}.
        % Due to the space limit, we put the partial results of the cumulative histogram in~\Cref{fig:statewise} in~\Cref{subsec:eval-action} and leave a complete presentation of all results here in~\Cref{fig:statewise-full}.
        The definitions of the two metrcis can be found in~\Cref{subsec:eval-action}.

        Basically, the conclusions in terms of the comparisons on the RL algorithm level, the aggregation protocol level, the partition number level, and the game level are all similar to that derived in~\Cref{subsec:eval-action}.
        
    \subsection{Full Results of Robustness Certification for Cumulative Reward Bound}
        \label{adxsubsec:full-reward}
        
        \input{fig_desc/fig_reward}
        In addition to the evaluation results provided in~\Cref{fig:reward} in~\cref{subsec:eval-reward}, we provide a more comprehensive set of evaluation results with more settings of trajectory length $H$ here in~\Cref{fig:reward-full}.
        
        We draw similar conclusions as discussed in~\Cref{subsec:eval-reward}.
        Specifically, in Highway, C51 achieves higher certified lower bounds than other two when the poisoning size is large, which can be explained by the larger portion of states that can tolerate large poisoning sizes as shown in~\Cref{fig:statewise-full-highway}.

        We additionally point out that the value $\uj_K$ achieved at poisoning size $K=0$ (\eg, $\uj_K=4$ for Freeway, $2$ for Breakout, and $28.31$ for Highway under $\rlalgopolicy$ over $u=50$ DQN subpolicies) corresponds to the case where there is no poisoning at all on the training set. Our successive bounds under larger $K$ are non-vacuous compared to this value.

\section{A Broader Discussion on Related Work}
\label{adxsec:related-works}

\subsection{Poisoning Attacks in RL}

% \noindent\textbf{Reward Poisoning Attacks.}\quad

Below, we provide a brief discussion on the related works on policy poisoning and reward poisoning~\citep{ma2019policy,sun2021vulnerabilityaware,huang2019deceptive}.

\citet{ma2019policy} and~\citet{huang2019deceptive} study reward poisoning where the attacker can modify the rewards in an offline dataset or the reward signals during the online interaction. The attacker’s goal is to force learning a particular target policy, or minimize the agent’s reward in the original task. Under this framework,~\citet{ma2019policy} considers two victim learners with specific assumptions on the learner structure and develops attacks for them, while~\citet{huang2019deceptive} provides a theoretical analysis on the conditions for successful attacks against a Q-learning agent. In comparison to only reward poisoning in~\citet{ma2019policy} and~\citet{huang2017adversarial},~\citet{sun2021vulnerabilityaware} focuses on general policy poisoning attacks for policy gradient learners in the online RL setting by using the vulnerability-awareness metric to decide when to poison, and the adversarial critic to guide the poisoning.~\citet{sun2021vulnerabilityaware} achieve successful poisoning against policy-based agents in various complex environments in online RL, but it remains an interesting open problem as to how to poison the offline RL dataset which is agnostic to the learning algorithm.



\subsection{Empirically Robust RL}

\noindent\textbf{Robust RL against Evasion Attacks.}\quad
We briefly review several categories of RL methods that demonstrate empirical  robustness against evasion attacks.
% , representatives of which have been evaluated in this paper.

\textit{Randomization methods}~\citep{tobin2017domain,akkaya2019solving} were first proposed to encourage exploration. 
% through large-scale exploration
This type of method was later systematically studied for its potential to improve model robustness.
NoisyNet~\citep{fortunato2017noisy} adds parametric noise to the network's weight during training, providing better resilience to both training-time and test-time attacks~\citep{behzadan2017whatever,behzadan2018mitigation},
also reducing the transferability of adversarial examples,
and enabling quicker recovery with fewer number of transitions during phase transition.

Under the \textit{adversarial training} framework,
\citet{kos2017delving} and \citet{behzadan2017whatever} show that re-training with random noise and FGSM perturbations increases the resilience against adversarial examples.
\citet{pattanaik2018robust} leverage attacks using an engineered loss function specifically designed for RL
to significant increase the robustness to parameter variations.
RS-DQN~\citep{fischer2019online} is an \textit{imitation learning} based approach that trains a robust student-DQN in parallel with a standard DQN in order to incorporate the constrains such as SOTA adversarial defenses~\citep{madry2017towards,mirman2018differentiable}. 
% We did not evaluate on their method due to no access to open-source code and missing details for reproducing the experiments.

SA-DQN~\citep{zhang2021robust} is a \textit{regularization} based method that 
adds regularizers to the training loss function to 
encourage the top-$1$ action to stay unchanged under perturbation.

Built on top of the \textit{neural network verification} algorithms~\citep{gowal2018effectiveness,weng2018towards}, Radial-RL~\citep{oikarinen2020robust} proposes to minimize an adversarial loss function that incorporates the upper bound of the perturbed loss, computed using certified bounds from verification algorithms.
CARRL~\citep{everett2021certifiable} aims to compute the  lower bounds of action-values under potential perturbation and select actions according to the worst-case bound, but it relies on linear bounds~\citep{weng2018towards} and is only suitable for low-dimensional environments.

These robust RL methods only provide empirical robustness against perturbed state inputs during test time, but cannot provide theoretical guarantees for the performance of the trained models under any bounded perturbations.

\noindent\textbf{Robust RL against Poisoning Attacks.}\quad
\citet{banihashem2021defense} considers the \textit{threat model} of reward poisoning attacks proposed by~\citet{ma2019policy,rakhsha2020policy,zhang2020adaptive}, where the attacker aims to force learning a target policy while minimizing the cost of reward manipulation. As shown in~\citet{ma2019policy,rakhsha2020policy,zhang2020adaptive}, this optimization problem is feasible and always has a unique optimal solution. Leveraging this property,~\citet{banihashem2021defense} formulates the defense task as another optimization problem which aims to optimize the agent’s worst case performance among the set of plausible candidates of the true reward function. They specifically consider two settings regarding the agent’s knowledge of the attack parameter, and provide lower bounds on the performance of the defense policy. In contrast to~\citet{banihashem2021defense} which focuses on a specific type of attack, our paper considers the \textit{threat model} of general poisoning attacks, where the attacker has the power to manipulate the training trajectories arbitrarily. Given limited knowledge regarding the attack, our proposed \sysname framework is general and applicable to any potential attack. Our robustness is derived from the aggregation over both sub-policy level and temporal level. One similarity between~\citet{banihashem2021defense} and our work is that we both aim to provide lower bounds of the cumulative reward for our proposed method as the provable guarantee / certification criteria.


\subsection{Robustness Certification for RL}

\citet{wu2022crop} provide the first robustness certification for RL against \textit{test-time evasion attacks} following the line of work on randomized smoothing~\citep{cohen2019certified,salman2019provably}. Concretely, they apply per-state smoothing to achieve the certification for per-state action stability, as well as trajectory smoothing to obtain the certification for cumulative reward.
Notably, \citet{wu2022crop} propose an adaptive tree search algorithm to explore all possible trajectories and thus derive the robustness guarantee for cumulative reward. The relationship between our \adasearch and their Algorithm 3 is discussed in detail in~\Cref{adxsubsec:alg-reward}.
In comparison, robustness in their work is derived from \textit{smoothing}, while our robustness comes from \textit{aggregation}. We propose aggregation protocols and certification methods that leverage the temporal information by dynamically aggregating over the past time steps, which is not covered in~\citet{wu2022crop}.




\end{document}


==> [ICLR 2022] COPA/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [ICLR 2022] COPA/tables/tab_action_change.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small {\textbf{Action change ratio (in percentage)} of three \textit{aggregation protocols} (PARL, TPARL, and DPARL) applied on subpolicies trained in Highway environment using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, \#partitions) $u$ equal to $30$, $50$, or $100$. 
    We report results averaged over $20$ runs of varying randomness in the environment.
    }}
    \label{tab:action_change}



\resizebox{.55\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\multirow{3}{*}{$u$} &
\multirow{3}{*}{\makecell{RL \\Algorithm}} &
\multicolumn{3}{c}{Aggregation Protocol}
\\
\cmidrule(lr){3-5}
&  & \multirow{2}{*}{PARL} & \multirow{2}{*}{\shortstack{TPARL \\($W = 4$)}} & \multirow{2}{*}{\shortstack{DPARL \\($W_{\rm max}=5$)}} \\
& & & & \\
\midrule
\multirow{3}{*}{$30$}  & DQN & 59.79 {\tiny  $\pm$   8.99 } & 24.89 {\tiny  $\pm$   10.47 } & 33.82 {\tiny  $\pm$   8.75 } \\
& QR-DQN & 61.00 {\tiny  $\pm$   12.74 } & 31.14 {\tiny  $\pm$   6.43 } & 37.80 {\tiny  $\pm$   7.16 } \\
& C51 & 59.00 {\tiny  $\pm$   10.39 } & 18.17 {\tiny  $\pm$   11.52 } & 35.44 {\tiny  $\pm$   8.65 } \\
\midrule
\multirow{3}{*}{$50$}  & DQN & 55.50 {\tiny  $\pm$   8.84 } & 26.05 {\tiny  $\pm$   11.69 } & 40.07 {\tiny  $\pm$   13.74 } \\
& QR-DQN & 60.37 {\tiny  $\pm$   10.31 } & 28.48 {\tiny  $\pm$   6.81 } & 37.78 {\tiny  $\pm$   12.15 } \\
& C51 & 59.39 {\tiny  $\pm$   12.34 } & 28.04 {\tiny  $\pm$   10.71 } & 38.21 {\tiny  $\pm$   11.23 } \\
\midrule
\multirow{3}{*}{$100$}  & DQN & 48.67 {\tiny  $\pm$   5.91 } & 22.17 {\tiny  $\pm$   7.65 } & 33.45 {\tiny  $\pm$   9.70 } \\
& QR-DQN & 61.17 {\tiny  $\pm$   8.38 } & 24.12 {\tiny  $\pm$   9.85 } & 36.76 {\tiny  $\pm$   7.87 } \\
& C51 & 61.83 {\tiny  $\pm$   10.41 } & 22.91 {\tiny  $\pm$   13.34 } & 34.06 {\tiny  $\pm$   9.19 } \\
\bottomrule
\end{tabular}
}




\end{table}
}

==> [ICLR 2022] COPA/tables/tab_ave_poison_size.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small \textbf{Average tolerable poisoning thresholds} of three \textit{aggregation protocols} (PARL, TPARL, and DPARL) applied on subpolicies trained using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, \#partitions) $u$ equal to $30$ or $50$. 
    We report results averaged over $20$ runs of varying randomness in the environment.
    }
    \label{tab:ave-poison-size}



\resizebox{.8\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Freeway}} &  \multicolumn{3}{c}{\small $u=30$}  & \multicolumn{3}{c}{\small $u=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} &  \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}}  \\\midrule
DQN & 9.90 {\tiny  $\pm$   0.14 } & 10.21 {\tiny  $\pm$   0.09 } & 10.30 {\tiny  $\pm$   0.09 } & 16.78 {\tiny  $\pm$   0.42 } & 17.16 {\tiny  $\pm$   0.29 } & 16.88 {\tiny  $\pm$   0.45 } \\
QR-DQN & 9.87 {\tiny  $\pm$   0.20 } & 10.11 {\tiny  $\pm$   0.30 } & 10.16 {\tiny  $\pm$   0.34 } & 16.79 {\tiny  $\pm$   0.52 } & 17.31 {\tiny  $\pm$   0.29 } & 17.03 {\tiny  $\pm$   0.40 } \\
C51 & 9.57 {\tiny  $\pm$   0.24 } & 9.83 {\tiny  $\pm$   0.15 } & 10.11 {\tiny  $\pm$   0.19 } & 16.82 {\tiny  $\pm$   0.40 } & 17.08 {\tiny  $\pm$   0.34 } & 17.61 {\tiny  $\pm$   0.15 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.8\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Breakout}} &  \multicolumn{3}{c}{\small $u=30$}  & \multicolumn{3}{c}{\small $u=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} &  \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} \\\midrule
DQN & 1.08 {\tiny  $\pm$   0.09 } & 1.28 {\tiny  $\pm$   0.15 } & 0.85 {\tiny  $\pm$   0.09 } & 2.07 {\tiny  $\pm$   0.22 } & 1.92 {\tiny  $\pm$   0.30 } & 1.55 {\tiny  $\pm$   0.28 } \\
QR-DQN & 1.38 {\tiny  $\pm$   0.09 } & 1.33 {\tiny  $\pm$   0.18 } & 1.18 {\tiny  $\pm$   0.10 } & 2.12 {\tiny  $\pm$   0.27 } & 1.93 {\tiny  $\pm$   0.14 } & 1.71 {\tiny  $\pm$   0.19 } \\
C51 & 1.10 {\tiny  $\pm$   0.08 } & 1.42 {\tiny  $\pm$   0.19 } & 0.93 {\tiny  $\pm$   0.13 } & 2.43 {\tiny  $\pm$   0.21 } & 2.37 {\tiny  $\pm$   0.19 } & 1.90 {\tiny  $\pm$   0.19 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.8\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{{Highway}}} &  \multicolumn{3}{c}{\small $u=30$}  & \multicolumn{3}{c}{\small $u=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} &  \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} \\\midrule
DQN & 4.38 {\tiny  $\pm$   0.78 } & 2.99 {\tiny  $\pm$   1.08 } & 3.75 {\tiny  $\pm$   1.85 } & 7.16 {\tiny  $\pm$   1.58 } & 6.27 {\tiny  $\pm$   1.61 } & 6.32 {\tiny  $\pm$   0.98 } \\
QR-DQN & 4.18 {\tiny  $\pm$   0.91 } & 3.35 {\tiny  $\pm$   1.44 } & 2.84 {\tiny  $\pm$   0.55 } & 6.52 {\tiny  $\pm$   1.17 } & 5.02 {\tiny  $\pm$   1.60 } & 4.61 {\tiny  $\pm$   1.20 } \\
C51 & 4.97 {\tiny  $\pm$   1.09 } & 4.31 {\tiny  $\pm$   1.45 } & 4.12 {\tiny  $\pm$   0.95 } & 7.95 {\tiny  $\pm$   1.46 } & 6.55 {\tiny  $\pm$   2.20 } & 6.69 {\tiny  $\pm$   1.47 } \\
\bottomrule
\end{tabular}
}


\end{table}
}

==> [ICLR 2022] COPA/tables/tab_ave_window_size.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small \textbf{Average window size} (\ie, $\sum_{t=1}^{T} W_t / T$) for the \textit{aggregation protocol} DPARL ($W_{\rm max}=5$) applied on subpolicies trained using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, \#partitions) $u$ equal to $30$ or $50$. 
    We report results averaged over all time steps in $20$ runs.
    }
    \label{tab:ave-window-size}



\resizebox{.75\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{}} &  \multicolumn{3}{c}{\small $u=30$}  & \multicolumn{3}{c}{\small $u=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small DQN}  & \multicolumn{1}{c}{\makecell{\small QR-DQN}} & \multicolumn{1}{c}{\makecell{\small C51}} &  \multicolumn{1}{c}{\small DQN} & \multicolumn{1}{c}{\makecell{\small QR-DQN}} & \multicolumn{1}{c}{\makecell{\small C51}}  \\\midrule
Freeway & 2.69 {\tiny  $\pm$   1.73 } & 2.59 {\tiny  $\pm$   1.71 } & 2.64 {\tiny  $\pm$   1.74 } & 2.79 {\tiny  $\pm$   1.73 } & 2.70 {\tiny  $\pm$   1.73 } & 2.72 {\tiny  $\pm$   1.73 } \\
Breakout & 2.28 {\tiny  $\pm$   1.46 } & 2.44 {\tiny  $\pm$   1.55 } & 2.32 {\tiny  $\pm$   1.48 } & 2.33 {\tiny  $\pm$   1.48 } & 2.40 {\tiny  $\pm$   1.52 } & 2.39 {\tiny  $\pm$   1.52 } \\
Highway & 1.97 {\tiny  $\pm$   0.44 } & 2.21 {\tiny  $\pm$   0.27 } & 2.16 {\tiny  $\pm$   0.37 } & 2.23 {\tiny  $\pm$   0.32 } & 2.26 {\tiny  $\pm$   0.24 } & 2.18 {\tiny  $\pm$   0.37 } \\
\bottomrule \\
\end{tabular}
}


\end{table}
}

==> [ICLR 2022] COPA/tables/tab_empirical_reward.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small \textbf{Benign empirical cumulative reward} of three \textit{aggregation protocols} (PARL, TPARL, and DPARL) applied on subpolicies trained using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, partition number) $k$ equal to $30$ or $50$. 
    We report results averaged over $20$ runs of varying randomness in the environment.
    }
    \label{tab:emp-reward}



\resizebox{.9\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Freeway}} &  \multicolumn{3}{c}{\small $k=30$}  & \multicolumn{3}{c}{\small $k=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} & \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} \\\midrule
DQN & 10.90 {\tiny  $\pm$   0.77 } & 12.00 {\tiny  $\pm$   0.45 } & 11.45 {\tiny  $\pm$   0.74 } & 10.95 {\tiny  $\pm$   0.97 } & 11.65 {\tiny  $\pm$   0.65 } & 11.90 {\tiny  $\pm$   0.89 } \\
QR-DQN & 11.60 {\tiny  $\pm$   0.66 } & 11.80 {\tiny  $\pm$   0.87 } & 12.10 {\tiny  $\pm$   0.99 } & 11.50 {\tiny  $\pm$   0.92 } & 12.80 {\tiny  $\pm$   0.51 } & 11.90 {\tiny  $\pm$   0.77 } \\
C51 & 11.20 {\tiny  $\pm$   0.60 } & 11.40 {\tiny  $\pm$   0.66 } & 12.40 {\tiny  $\pm$   0.49 } & 11.70 {\tiny  $\pm$   1.27 } & 11.50 {\tiny  $\pm$   0.87 } & 11.95 {\tiny  $\pm$   0.92 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.9\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Breakout}} &  \multicolumn{3}{c}{\small $k=30$}  & \multicolumn{3}{c}{\small $k=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} & \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} \\\midrule
DQN & 58.65 {\tiny  $\pm$   40.83 } & 13.50 {\tiny  $\pm$   11.41 } & 36.00 {\tiny  $\pm$   13.39 } & 60.25 {\tiny  $\pm$   31.99 } & 14.95 {\tiny  $\pm$   7.24 } & 45.00 {\tiny  $\pm$   13.44 } \\
QR-DQN & 76.50 {\tiny  $\pm$   79.76 } & 19.05 {\tiny  $\pm$   6.91 } & 42.05 {\tiny  $\pm$   15.60 } & 62.80 {\tiny  $\pm$   28.71 } & 17.30 {\tiny  $\pm$   7.89 } & 41.00 {\tiny  $\pm$   13.87 } \\
C51 & 51.80 {\tiny  $\pm$   10.74 } & 13.55 {\tiny  $\pm$   7.37 } & 34.75 {\tiny  $\pm$   10.91 } & 60.55 {\tiny  $\pm$   20.44 } & 19.65 {\tiny  $\pm$   7.30 } & 39.90 {\tiny  $\pm$   14.69 } \\\bottomrule
\end{tabular}
}


\end{table}
}

==> [ICLR 2022] COPA/tables/tab_empirical_reward_full.tex <==
{
\setlength{\tabcolsep}{3pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small \textbf{Benign empirical performance} of three \textit{aggregation protocols} (PARL, TPARL, and DPARL) applied on subpolicies trained using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, \#partitions) $u$ equal to $30$ or $50$. 
    We report results averaged over $20$ runs of varying randomness in the environment.
    }
    \label{tab:emp-reward-full}



\resizebox{.98\linewidth}{!}{%
        \begin{tabular}{ccccccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Freeway}} &  \multicolumn{5}{c}{\small $u=30$}  & \multicolumn{5}{c}{\small $u=50$} \\
    \cmidrule(lr){2-6}\cmidrule(lr){7-11}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} &
    \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} & 
    \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}}
    \\\midrule
DQN & 10.90 {\tiny  $\pm$   0.77 } & 11.65 {\tiny  $\pm$   0.57 } & 11.25 {\tiny  $\pm$   0.54 } & 12.00 {\tiny  $\pm$   0.45 } & 11.45 {\tiny  $\pm$   0.74 } & 10.95 {\tiny  $\pm$   0.97 } & 11.60 {\tiny  $\pm$   1.02 } & 12.40 {\tiny  $\pm$   0.58 } & 11.65 {\tiny  $\pm$   0.65 } & 11.90 {\tiny  $\pm$   0.89 } \\
QR-DQN & 11.60 {\tiny  $\pm$   0.66 } & 11.85 {\tiny  $\pm$   1.15 } & 11.25 {\tiny  $\pm$   0.62 } & 11.80 {\tiny  $\pm$   0.87 } & 12.10 {\tiny  $\pm$   0.99 } & 11.50 {\tiny  $\pm$   0.92 } & 11.60 {\tiny  $\pm$   1.02 } & 12.15 {\tiny  $\pm$   0.57 } & 12.80 {\tiny  $\pm$   0.51 } & 11.90 {\tiny  $\pm$   0.77 } \\
C51 & 11.20 {\tiny  $\pm$   0.60 } & 12.45 {\tiny  $\pm$   0.50 } & 12.55 {\tiny  $\pm$   0.50 } & 11.40 {\tiny  $\pm$   0.66 } & 12.40 {\tiny  $\pm$   0.49 } & 11.70 {\tiny  $\pm$   1.27 } & 11.80 {\tiny  $\pm$   0.75 } & 12.70 {\tiny  $\pm$   0.46 } & 11.50 {\tiny  $\pm$   0.87 } & 11.95 {\tiny  $\pm$   0.92 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.98\linewidth}{!}{%
        \begin{tabular}{ccccccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Breakout}} &  \multicolumn{5}{c}{\small $u=30$}  & \multicolumn{5}{c}{\small $u=50$} \\
    \cmidrule(lr){2-6}\cmidrule(lr){7-11}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} &
    \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} & 
    \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}}
    \\\midrule
DQN & 58.65 {\tiny  $\pm$   40.83 } & 38.05 {\tiny  $\pm$   10.22 } & 26.00 {\tiny  $\pm$   12.79 } & 13.50 {\tiny  $\pm$   11.41 } & 36.00 {\tiny  $\pm$   13.39 } & 60.25 {\tiny  $\pm$   31.99 } & 37.90 {\tiny  $\pm$   11.55 } & 25.90 {\tiny  $\pm$   9.55 } & 14.95 {\tiny  $\pm$   7.24 } & 45.00 {\tiny  $\pm$   13.44 } \\
QR-DQN & 76.50 {\tiny  $\pm$   79.76 } & 45.25 {\tiny  $\pm$   42.70 } & 22.05 {\tiny  $\pm$   9.13 } & 19.05 {\tiny  $\pm$   6.91 } & 42.05 {\tiny  $\pm$   15.60 } & 62.80 {\tiny  $\pm$   28.71 } & 32.10 {\tiny  $\pm$   9.27 } & 40.25 {\tiny  $\pm$   52.97 } & 17.30 {\tiny  $\pm$   7.89 } & 41.00 {\tiny  $\pm$   13.87 } \\
C51 & 51.80 {\tiny  $\pm$   10.74 } & 37.60 {\tiny  $\pm$   11.38 } & 24.75 {\tiny  $\pm$   12.77 } & 13.55 {\tiny  $\pm$   7.37 } & 34.75 {\tiny  $\pm$   10.91 } & 60.55 {\tiny  $\pm$   20.44 } & 34.85 {\tiny  $\pm$   11.92 } & 26.15 {\tiny  $\pm$   9.98 } & 19.65 {\tiny  $\pm$   7.30 } & 39.90 {\tiny  $\pm$   14.69 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.98\linewidth}{!}{%
        \begin{tabular}{ccccccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{{Highway}}} &  \multicolumn{5}{c}{\small $u=30$}  & \multicolumn{5}{c}{\small $u=50$} \\
    \cmidrule(lr){2-6}\cmidrule(lr){7-11}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} &
    \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} & 
    \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\makecell{\small TPARL \\($W=2$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=3$)}} &
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}}
    \\\midrule
DQN & 28.07 {\tiny  $\pm$   3.86 } & 19.16 {\tiny  $\pm$   10.26 } & 16.83 {\tiny  $\pm$   8.35 } & 12.69 {\tiny  $\pm$   6.17 } & 23.55 {\tiny  $\pm$   9.01 } & 29.05 {\tiny  $\pm$   0.62 } & 16.63 {\tiny  $\pm$   9.93 } & 15.85 {\tiny  $\pm$   8.52 } & 13.43 {\tiny  $\pm$   8.29 } & 22.51 {\tiny  $\pm$   8.01 } \\
QR-DQN & 28.52 {\tiny  $\pm$   1.22 } & 18.63 {\tiny  $\pm$   8.07 } & 15.53 {\tiny  $\pm$   7.46 } & 12.77 {\tiny  $\pm$   6.39 } & 23.11 {\tiny  $\pm$   7.94 } & 27.64 {\tiny  $\pm$   3.01 } & 20.59 {\tiny  $\pm$   7.70 } & 14.94 {\tiny  $\pm$   7.76 } & 14.13 {\tiny  $\pm$   7.54 } & 23.49 {\tiny  $\pm$   7.95 } \\
C51 & 28.86 {\tiny  $\pm$   1.08 } & 20.20 {\tiny  $\pm$   9.21 } & 13.30 {\tiny  $\pm$   8.65 } & 9.36 {\tiny  $\pm$   5.96 } & 21.51 {\tiny  $\pm$   10.04 } & 27.44 {\tiny  $\pm$   4.32 } & 15.12 {\tiny  $\pm$   9.36 } & 16.13 {\tiny  $\pm$   8.46 } & 10.61 {\tiny  $\pm$   6.52 } & 19.94 {\tiny  $\pm$   11.14 } \\
\bottomrule \\
\end{tabular}
}

\end{table}
}

==> [ICLR 2022] COPA/tables/tab_runtime.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small {\textbf{Runtime (unit: seconds)} of the \textit{aggregation protocol} DPARL ($W_{\rm max}=5$) applied on subpolicies trained using \textit{offline RL algorithm} DQN,
    with the number of subpolicies (\ie, partition number) $u$ equal to $30$ or $50$. 
    We compare with the \textit{standard testing} which tests the runtime of a single trained DQN policy without using our 
    % partition-based training and aggregation certification 
    framework.
    We report results averaged over $20$ runs of varying randomness in the environment, where each run is an episode of length at most $1000$.% \chejianm{for Atari games and $30$ for Highway environment}.
    % Note that the time complexity of DPARL scales quasilinearly with the number of subpolicies $u$, and quadratically with the action set size $|\cal A|$, which is $3$ for Freeway and $4$ for Breakout.
    }}
    \label{tab:runtime}



\resizebox{.6\linewidth}{!}{%
        \begin{tabular}{cccc
}
    \toprule
    {}
    &    \multicolumn{1}{c}{\small standard testing}   & \multicolumn{1}{c}{\small DPARL ($u=30$)}   & \multicolumn{1}{c}{\small DPARL ($u=50$)} \\\midrule
Freeway & 2.53 {\tiny  $\pm$   0.50 } & 56.37 {\tiny  $\pm$   1.75 } & 79.05 {\tiny  $\pm$   4.27 } \\
Breakout & 2.00 {\tiny  $\pm$   0.56 } & 72.05 {\tiny  $\pm$   13.09 } & 108.05 {\tiny  $\pm$   8.71 } \\
% \chejianm{Highway} & 1.09 {\tiny  $\pm$   0.26 } & 9.10 {\tiny  $\pm$   8.24 } & 10.05 {\tiny  $\pm$   8.30 } \\
\bottomrule \\
\end{tabular}
}




\end{table}
}

==> [ICLR 2022] COPA/tables/tab_testing_cmp.tex <==
{
\setlength{\tabcolsep}{3pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small {\textbf{The \textit{policy quality} measured by \textit{empirical cumulative reward} of the proposed aggregation protocols (PARL, TPARL, and DPARL) compared with the standard training.}
    In our aggregation, we aggregate over $u$ subpolicies with $u$ equal to $30$ or $50$ .
    We report results averaged over $20$ runs of varying randomness in the environment, where each run is an episode of length at most $1000$ for Atari games and $30$ for Highway environment. The offline RL algorithm used is DQN.}
    }
    \label{tab:testing-cmp}



\resizebox{.9\linewidth}{!}{%
        \begin{tabular}{cccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{\makecell{}}} & \multirow{3}{*}{\makecell{standard \\ trained\\ policy }} & \multicolumn{3}{c}{\small $u=30$}  & \multicolumn{3}{c}{\small $u=50$} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & &    \multicolumn{1}{c}{\small PARL}  & 
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} &
    \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}} & 
    \multicolumn{1}{c}{\small PARL} & 
    \multicolumn{1}{c}{\makecell{\small TPARL \\($W=4$)}} & \multicolumn{1}{c}{\makecell{\small DPARL \\($W_{\rm max}=5$)}}
    \\\midrule
Freeway & 12.00 {\tiny  $\pm$   0.89 } & 10.90 {\tiny  $\pm$   0.77 } &  12.00 {\tiny  $\pm$   0.45 } & 11.45 {\tiny  $\pm$   0.74 } & 10.95 {\tiny  $\pm$   0.97 } &  11.65 {\tiny  $\pm$   0.65 } & 11.90 {\tiny  $\pm$   0.89 } \\
Breakout & 97.60 {\tiny  $\pm$   117.28 } & 58.65 {\tiny  $\pm$   40.83 } &  13.50 {\tiny  $\pm$   11.41 } & 36.00 {\tiny  $\pm$   13.39 } & 60.25 {\tiny  $\pm$   31.99 } &  14.95 {\tiny  $\pm$   7.24 } & 45.00 {\tiny  $\pm$   13.44 } \\
Highway & 28.90 {\tiny  $\pm$   0.87 } & 28.07 {\tiny  $\pm$   3.86 } & 12.69 {\tiny  $\pm$   6.17 } & 23.55 {\tiny  $\pm$   9.01 } & 29.05 {\tiny  $\pm$   0.62 } & 13.43 {\tiny  $\pm$   8.29 } & 22.51 {\tiny  $\pm$   8.01 } \\
\bottomrule \\
\end{tabular}
}


\end{table}
}

==> algos-PA-RL.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified poison sizes along time steps}
\SetKwFunction{funca}{pre-processing}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Pn{\funca{}} {
%     % \Comment*[l]{\footnotesize Preprocessing: given a trained $Q$ network, compute its output range and the \lip constant of its smoothed version}
%     Sample the input states and pass them to the given network $Q$ to compute the minimum value $V_{\min}$ and maximum value $V_{\max}$\;
%     $L=\frac{ V_{\max} - V_{\min} }{\sigma}\sqrt{\nicefrac{2}{\pi}}$\;
% }\;

% \Fn{\funcb{$s,\eps$}} {
    \Comment*[l]{\footnotesize Training Phase}
    
    \KwIn{training dataset $D$, number of partitions $k$}
	\KwOut{\rlalgo policy $\mpi$}
    
    Separate the training data $D$ into $k$ partitions $\{P_i\}_{i=0}^{k-1}$\;
    \For {each partition $P_i$} {
    	$\pi_i \leftarrow $ base policy trained on an partition $P_i$
    }
    $\mpi \leftarrow $ aggregation of $\{\pi_i\}_{i=0}^{k-1}$ via Eq.~\ref{eq:agg}\;
	\KwRet{$\mpi$}
    \columnbreak
    
    
    \Comment*[l]{\footnotesize Testing Phase}
    \KwIn{initial state distribution $d_0$, \rlalgo policy $\mpi$}
	\KwOut{a sequence of certified poison sizes along time steps}

    $s_0 \sim d_0, t \leftarrow 0$ \Comment*[r]{\scriptsize initial state observation}
    \While {$s_t \neq \perp$} {
	    \Comment*[l]{\scriptsize take action according to $\mpi$}
    	$a_t \leftarrow \mpi (s_t)$ \;
   		\Comment*[l]{\scriptsize compute the certified poison size}
    	$I_t \leftarrow \left\lfloor\frac{n_{a_t}(s_t)-\max _{a^{\prime} \neq a_t}\left(n_{a^{\prime}}(s_t)+\mathds{1}_{a^{\prime}<a_t}\right)}{2}\right\rfloor$\;
    	\Comment*[l]{\scriptsize transition to the next state}
    	$s_{t+1} \leftarrow \Gamma(s_t,a_t), t \leftarrow t+1$\;
    }
    \KwRet{ $I_0,I_1, \ldots$ }
% }
\end{multicols}
\caption{\small \textbf{PA-RL}: training, action prediction, and certification
}\label{alg:PA-RL}
\end{algorithm}


==> algos-PTA-RL-fixed.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified attack magnitudes along time steps}
\SetKwFunction{funca}{\textsc{ ComputePoisonSize}}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \Fn{\funcb{$s,\eps$}} {
    
    \KwIn{$k$ trained base policies $\{\pi_i\}_{i=0}^{k-1}$, fixed window size $W$, current time step $t$, and state $s_t$}
	\KwOut{action prediction $a_t$ and certification $I_t$}

	\Comment*[l]{\scriptsize Compute the smallest poison size required to alter the action selection from $a_t$ to $a$}
	 \Fn{\funca{$a_t,a,\{n_a^W\},\{c_a^i\}$}} {
		\For { $i$ from $0$ to $k-1$ } {
    		$h_i \leftarrow c_{a_t}^i + W - c_a^i$
    	}
    	sort $h_0, \ldots, h_{k-1}$ decreasingly\;
% 		$\delta \leftarrow \left\lfloor\frac{n_{a_t}^W-\left(n_{a}^W+\mathds{1}_{a<a_t}\right)}{2}\right\rfloor$\;
		$\delta \leftarrow n_{a_t}^W-\left(n_{a}^W+\mathds{1}_{a<a_t}\right)$\;
%		$I \leftarrow $ 
		\KwRet smallest $j$ such that $\sum_{i=0}^{j-1} h_i > \delta$\;
	 }

	\Comment*[l]{\scriptsize Initialization}
	\For { $a \in \gA$ } {
		$L_a^W \leftarrow \emptyset$ \Comment*[r]{\scriptsize list of models voting for $a$}
		$n_a^W \leftarrow 0$ \Comment*[r]{\scriptsize count of models voting for $a$}
	}\;
	
	\columnbreak

	\Comment*[l]{\scriptsize Compute temporal aggregated action count}
	\For { $j$ from $0$ to $\min\{W-1,t\}$ } {
		\For { $i$ from $0$ to $k-1$ } {
			$a \leftarrow \pi_i(s_{t-j})$\;
			$L_a^W \leftarrow L_a^W \cup \{ \pi_i \}$\;
			$n_a^W \leftarrow n_a^W + 1$
		}
	}
	
%	$c_a^i \leftarrow $ count of $\pi_i$ in $L_{a}^W$ \textbf{for} { $a \in \gA$ } \textbf{and} { $i$ from $0$ to $k-1$ }
	\For { $a \in \gA$ } {
    	\For { $i$ from $0$ to $k-1$ } {
    		$c_a^i \leftarrow $ count of $\pi_i$ in $L_{a}^W$
    	}
    }



	\Comment*[l]{\scriptsize Compute temporal aggregated action prediction}
	$a_t \leftarrow \argmax_{a \in \gA} n_a^W$\;

    
    \Comment*[l]{\scriptsize Compute certification}
    
%    $m \leftarrow \left\lfloor\frac{n_{a}^W-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}^W+\mathds{1}_{a^{\prime}<a}\right)}{2}\right\rfloor$
    
    
    $I_t \leftarrow \min_{a \in \gA,a \neq a_t}$ \texttt{\textsc{ ComputePoisonSize}}($a_t,a,\{n_a^W\},\{c_a^i\}$) $- 1$
        
    \KwRet{ $a_t,I_t$ }
% }
\end{multicols}
\caption{\small \textbf{PTA-RL}: action prediction and certification
}\label{alg:PTA-RL-fixed}
\end{algorithm}


==> algos-PTA-RL-flex.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
%\KwIn{\textbf{(training)} training dataset $D$, number of partitions $k$; \textbf{(testing)} initial state distribution $d_0$ }
%\KwOut{\textbf{(training)} \rlalgo policy $\mpi$; \textbf{(testing)} a sequence of certified attack magnitudes along time steps}
\SetKwFunction{funca}{pre-processing}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Pn{\funca{}} {
%     % \Comment*[l]{\footnotesize Preprocessing: given a trained $Q$ network, compute its output range and the \lip constant of its smoothed version}
%     Sample the input states and pass them to the given network $Q$ to compute the minimum value $V_{\min}$ and maximum value $V_{\max}$\;
%     $L=\frac{ V_{\max} - V_{\min} }{\sigma}\sqrt{\nicefrac{2}{\pi}}$\;
% }\;

% \Fn{\funcb{$s,\eps$}} {
    
    \KwIn{$k$ trained base policies $\{\pi_i\}_{i=0}^{k-1}$, maximum window size $U$, current time step $t$, and state $s_t$}
	\KwOut{action prediction $a_t$ and certification $I_t$}

	\Comment*[l]{\scriptsize Initialization}
	\For { $a \in \gA$ } {
		\For { $ W \in \{1,\ldots,  \min\{U, t+1\} \}$} {
			$L_a^{W} \leftarrow \emptyset$\;
			$n_a^{W} \leftarrow 0$
		}
	}

	\Comment*[l]{\scriptsize Compute temporal aggregated action count}
	\For { $W$ from $1$ to $\min\{U,t+1\}$ } {
		\If { $W > 1$ } {
			$ L_a^{W} \leftarrow L_a^{W-1} $\;
			$ n_a^{W} \leftarrow n_a^{W-1} $\;
		}
		\For { $i$ from $0$ to $k-1$ } {
			$a \leftarrow \pi_i(s_{t-W+1})$\;
			$L_a^{W} \leftarrow L_a^{W} \cup \{ \pi_i \}$\;
			$n_a^{W} \leftarrow n_a^{W} + 1$
		}
	}

    \columnbreak	
    
    \Comment*[l]{\scriptsize Compute temporal wise action margin}
	\For { $W$ from $1$ to $\min\{U,t+1\}$ } {
		$a_W^1, a_W^2 \leftarrow$ actions of \nth{1} and \nth{2} highest vote counts among $\{ n_a^{W} \}_{a \in \gA}$\;
		$\Delta_t^{W} \leftarrow n_{a_W^1}^{W} - n_{a_W^2}^{W}$
	}


    
    \Comment*[l]{\scriptsize Compute optimal window size $W_t$ and corresponding action prediction $a_t$}
	$W_t \leftarrow \argmax_{W} \Delta_t^{W}$\;
	$a_t \leftarrow \argmax_{a \in \gA} n_{a}^{W_t}$ \Comment*[l]{\scriptsize \ie, $a_t \leftarrow a_{W_t}^1$}
    
    \Comment*[l]{\scriptsize Compute certification $I_t$}
    
%    $m \leftarrow \left\lfloor\frac{n_{a}^W-\max _{a^{\prime} \neq a}\left(n_{a^{\prime}}^Whds{1}_{a^{\prime}<a}\right)}{2}\right\rfloor$
    
    \For {$i$ from $0$ to $k-1$} {
    	$c_i \leftarrow $ count of $\pi_i$ in $L_{a_t}^{W_t}$
    }
    sort $c_0,\ldots,c_{k-1}$ decreasingly\;
    $I_t \leftarrow $ largest $j$ such that $\sum_{i=0}^{j-1}c_i \leq \left\lfloor\frac{\Delta_{t}^{W_t}-\max_{W \neq W_t}\left( \mathrm{sgn}(a_W^1 \neq a_t) \cdot \Delta_{t}^{W}+\mathds{1}_{a_W^1<a}\right)}{2}\right\rfloor$
    
    \KwRet{ $a_t, I_t$ }
% }
\end{multicols}
\caption{\small \textbf{PDTA-RL}: action prediction and certification
}\label{alg:PTA-RL-flex}
\end{algorithm}


==> fig_desc/fig_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightaction}
\settoheight{\utilheightaction}{\includegraphics[width=.17\linewidth]{figs/freeway_action_dqn_30.pdf}}%


\newlength{\legendheightaction}
\setlength{\legendheightaction}{0.4\utilheightaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightaction]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $k=30$}}}
        & \makecell{\small{\textbf{Freeway, $k=50$}}}
        & \makecell{\small{\textbf{Breakout, $k=30$}}}
        & \makecell{\small{\textbf{Breakout, $k=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_dqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_dqn_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_dqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_qrdqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_qrdqn_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_qrdqn_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_c51_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/freeway_action_c51_50.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_c51_30.pdf}&
\includegraphics[height=\utilheightaction]{figs/breakout_action_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($k=30$ and $k=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> fig_desc/fig_action_50.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionfifty}
\settoheight{\utilheightactionfifty}{\includegraphics[width=.49\linewidth]{figs/Freeway_action_full_dqn_50.pdf}}%


\newlength{\legendheightactionfifty}
\setlength{\legendheightactionfifty}{0.25\utilheightactionfifty}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionfifty][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionfifty]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway}}}
        & \makecell{\small{\textbf{Breakout}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_dqn_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionfifty]{figs/freeway_action_full_c51_50.pdf}&
\includegraphics[height=\utilheightactionfifty]{figs/breakout_action_full_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($k=30$ and $k=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> fig_desc/fig_action_half.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionhalf}
\settoheight{\utilheightactionhalf}{\includegraphics[width=.17\linewidth]{figs/freeway_action_half_dqn_30.pdf}}%


\newlength{\legendheightactionhalf}
\setlength{\legendheightactionhalf}{0.4\utilheightactionhalf}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionhalf][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionhalf]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=30$}}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        & \makecell{\small{\textbf{Breakout, $u=30$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize count}}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/freeway_action_half_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalf]{figs/breakout_action_half_c51_50.pdf}
\\
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
        & \makecell{\footnotesize{$\wbar K$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action.}
We plot the histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps in one trajectory.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide results on two games (Freeway and Breakout), two partition numbers ($u=30$ and $u=50$), and a comparison of three certification methods (PARL, TPARL, DPARL).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs considering the randomness in the game environment, and the short vertical bar on top of each bar represents the standard deviation.
}%
\label{fig:statewise}
\end{figure}



==> fig_desc/fig_action_half_cum.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightactionhalfcum}
\settoheight{\utilheightactionhalfcum}{\includegraphics[width=.17\linewidth]{figs/freeway_action_half_cum_dqn_30.pdf}}%


\newlength{\legendheightactionhalfcum}
\setlength{\legendheightactionhalfcum}{0.4\utilheightactionhalfcum}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightactionhalfcum][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightactionhalfcum]{figs/legend_bar_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{.925\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, $u=30$}}}
        & \makecell{\small{\textbf{Freeway, $u=50$}}}
        & \makecell{\small{\textbf{Breakout, $u=30$}}}
        & \makecell{\small{\textbf{Breakout, $u=50$}}}
        \\
\rowname{\makecell{\small \textbf{DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_dqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_dqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_dqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_qrdqn_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_qrdqn_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_qrdqn_50.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\scriptsize stability ratio}}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/freeway_action_half_cum_c51_50.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_c51_30.pdf}&
\includegraphics[height=\utilheightactionhalfcum]{figs/breakout_action_half_cum_c51_50.pdf}
\\
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
        & \makecell{\scriptsize{$\geq \wbar K$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for per-state action stability.}
We plot the cumulative histogram of the \textit{tolerable poisoning size} $\protect\wbar K$ for all time steps.
% Each bar at $\protect\wbar K$ denotes the count of time steps that achieve the tolerable poisoning size $\protect\wbar K$, \ie, $\sum_{t=0}^{T-1}\1 [\protect\wbar K_t=I]$.
We provide the certification for different aggregation protocols (PARL, TPARL, DPARL) on two games (Freeway and Breakout) and two \#partitions ($u\in \{30, 50\}$).
% We constrain the maximum trajectory length $H$ to be $1000$ for ease of comparison.
The results are averaged over $20$ runs with the vertical bar on top denoting the standard deviation.
}%
\label{fig:statewise}
\vspace{-2.2em}
\end{figure}



==> fig_desc/fig_breakout_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightbreakoutaction}
\settoheight{\utilheightbreakoutaction}{\includegraphics[width=.33\linewidth]{figs/breakout_action_dqn_30.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakoutaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakoutaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$k=30$}}
        & \makecell{\small{$k=50$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_dqn_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_dqn_50.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_qrdqn_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_qrdqn_50.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_c51_30.png}&
\includegraphics[height=\utilheightbreakoutaction]{figs/breakout_action_c51_50.png}
\\[-1.2ex]
        & \makecell{\small{robust size $I$}}
        & \makecell{\small{robust size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Histogram of the robust size} computed on Breakout. The results are averaged over $20$ runs, where each run corresponds to one trajectory with randomness in the environment. For ease of comparison, we constrain the maximum trajectory length to be $1000$.
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> fig_desc/fig_breakout_reward.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheightbreakout}
\settoheight{\utilheightbreakout}{\includegraphics[width=.33\linewidth]{figs/breakout_c51_50.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakout}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakout][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=50$}}
        & \makecell{\small{trajectory length $t=75$}}
        & \makecell{\small{trajectory length $t=125$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_dqn_125.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_qrdqn_125.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_50.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_75.png}&
\includegraphics[height=\utilheightbreakout]{figs/breakout_c51_125.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for the cumulative reward on game Breakout.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under three different certification methods (PA, TPA (W=4), DTPA).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{TODO: fill in conclusion}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> fig_desc/fig_breakout_reward_tight.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightbreakouttight}
\settoheight{\utilheightbreakouttight}{\includegraphics[width=.33\linewidth]{figs/breakout_c51_50_tight.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightbreakouttight}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakouttight][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=50$}}
        & \makecell{\small{trajectory length $t=75$}}
        & \makecell{\small{trajectory length $t=125$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_dqn_125_tight.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_qrdqn_125_tight.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_50_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_75_tight.png}&
\includegraphics[height=\utilheightbreakouttight]{figs/breakout_c51_125_tight.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Comparison of the loose and tight lower bound for the cumulative reward certification when $W=1$, evaluated on Breakout.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under two certification methods (loose vs. tight).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{This part may go into appendix if no space in main paper, or we can think about how to merge the figures?}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}

==> fig_desc/fig_freeway_action.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightfreewayaction}
\settoheight{\utilheightfreewayaction}{\includegraphics[width=.33\linewidth]{figs/freeway_action_dqn_30.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightfreewayaction}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightfreewayaction][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$k=30$}}
        & \makecell{\small{$k=50$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_dqn_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_dqn_50.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_qrdqn_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_qrdqn_50.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_c51_30.png}&
\includegraphics[height=\utilheightfreewayaction]{figs/freeway_action_c51_50.png}
\\[-1.2ex]
        & \makecell{\small{robust size $I$}}
        & \makecell{\small{robust size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Histogram of the robust size} computed on Breakout. The results are averaged over $20$ runs, where each run corresponds to one trajectory with randomness in the environment. For ease of comparison, we constrain the maximum trajectory length to be $1000$.
}%
\label{fig:statewise}
\end{figure}



==> fig_desc/fig_freeway_reward.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheighta}
\settoheight{\utilheighta}{\includegraphics[width=.19\linewidth]{figs/freeway_c51_100.pdf}}%


\newlength{\legendheight}
\setlength{\legendheight}{0.5\utilheighta}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheighta][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheight]{figs/legend_all.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{6mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{\textbf{Freeway, }$t=100$}}
        & \makecell{\small{\textbf{Freeway, }$t=200$}}
        & \makecell{\small{\textbf{Freeway, }$t=400$}}
        & \makecell{\small{\textbf{Breakout, }$t=50$}}
        & \makecell{\small{\textbf{Breakout, }$t=75$}}\\
\rowname{\makecell{\small \textbf{DQN} \\\footnotesize $J$ }}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_dqn_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_dqn_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_dqn_75.pdf}
\\
\rowname{\makecell{\small \textbf{QR-DQN} \\\footnotesize $J$}}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_qrdqn_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_qrdqn_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_qrdqn_75.pdf}
\\
\rowname{\makecell{\small \textbf{C51} \\\footnotesize $J$}}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_100.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_200.pdf}&
\includegraphics[height=\utilheighta]{figs/freeway_c51_400.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_c51_50.pdf}&
\includegraphics[height=\utilheighta]{figs/Breakout_c51_75.pdf}
\\[-1.2ex]
        & \makecell{\footnotesize{poison size $I$}}
        & \makecell{\footnotesize{poison size $I$}}
        & \makecell{\footnotesize{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Robustness certification for the on game Freeway.}
We plot the lower bound of \textit{$J$} w.r.t. \textit{poison size} $I$ under three different certification methods (PA, TPA (W=4), DTPA).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of $t$.
\fan{TODO: fill in conclusion}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}



==> fig_desc/fig_freeway_reward_tight.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}



\newlength{\utilheightatight}
\settoheight{\utilheightatight}{\includegraphics[width=.33\linewidth]{figs/freeway_dqn_100_tight.png}}%


% \newlength{\legendheight}
% \setlength{\legendheight}{0.3\utilheightatight}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightatight][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subtable}[]{\linewidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheight]{figures/legend.pdf}
% \end{tabular}
% \end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}}
        & \makecell{\small{trajectory length $t=100$}}
        & \makecell{\small{trajectory length $t=200$}}
        & \makecell{\small{trajectory length $t=400$}}\\
\rowname{\makecell{\small DQN}}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_dqn_400_tight.png}\\
\rowname{\makecell{\small QR-DQN}}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_qrdqn_400_tight.png}\\
\rowname{\makecell{\small C51}}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_100_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_200_tight.png}&
\includegraphics[height=\utilheightatight]{figs/freeway_c51_400_tight.png}
\\[-1.2ex]
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
        & \makecell{\small{poison size $I$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \textbf{Comparison of the loose and tight lower bound for the cumulative reward certification when $W=1$, evaluated on Freeway.}
We plot the lower bound of \textit{cumulative reward $J$} w.r.t. \textit{poison size} $I$ under two certification methods (loose vs. tight).
Each row corresponds to one RL algorithm, and each column corresponds to one setting of trajectory length $t$.
\fan{This part may go into appendix if no space in main paper, or we can think about how to merge the figures?}
}%
\label{fig:statewise}
\vspace{-1em}
\end{figure}

==> tables/tab_empirical_reward.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[tbp]
    \centering

    \caption{\small \textbf{Benign empirical cumulative reward} of three \textit{aggregation protocols} (PARL, TPARL, and DPARL) applied on subpolicies trained using three \textit{offline RL algorithms} (DQN, QR-DQN, and C51),
    with the number of subpolicies (\ie, partition number) $k$ equal to $30$ or $50$. 
    We report results averaged over $20$ runs of varying randomness in the environment.
    }
    \label{tab:emp-reward}



\resizebox{.9\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Freeway}} &  \multicolumn{3}{c}{\small $k=30$}  & \multicolumn{3}{c}{\small $k=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} & \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} \\\midrule
DQN & 10.90 {\tiny  $\pm$   0.77 } & 12.00 {\tiny  $\pm$   0.45 } & 11.45 {\tiny  $\pm$   0.74 } & 10.95 {\tiny  $\pm$   0.97 } & 11.65 {\tiny  $\pm$   0.65 } & 11.90 {\tiny  $\pm$   0.89 } \\
QR-DQN & 11.60 {\tiny  $\pm$   0.66 } & 11.80 {\tiny  $\pm$   0.87 } & 12.10 {\tiny  $\pm$   0.99 } & 11.50 {\tiny  $\pm$   0.92 } & 12.80 {\tiny  $\pm$   0.51 } & 11.90 {\tiny  $\pm$   0.77 } \\
C51 & 11.20 {\tiny  $\pm$   0.60 } & 11.40 {\tiny  $\pm$   0.66 } & 12.40 {\tiny  $\pm$   0.49 } & 11.70 {\tiny  $\pm$   1.27 } & 11.50 {\tiny  $\pm$   0.87 } & 11.95 {\tiny  $\pm$   0.92 } \\
\bottomrule \\
\end{tabular}
}

\resizebox{.9\linewidth}{!}{%
        \begin{tabular}{ccccccc
}
    \toprule
    \multirow{2}{*}{\textbf{Breakout}} &  \multicolumn{3}{c}{\small $k=30$}  & \multicolumn{3}{c}{\small $k=50$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &    \multicolumn{1}{c}{\small PARL}  & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} & \multicolumn{1}{c}{\small PARL} & \multicolumn{1}{c}{\small TPARL} & \multicolumn{1}{c}{\small DPARL} \\\midrule
DQN & 58.65 {\tiny  $\pm$   40.83 } & 13.50 {\tiny  $\pm$   11.41 } & 36.00 {\tiny  $\pm$   13.39 } & 60.25 {\tiny  $\pm$   31.99 } & 14.95 {\tiny  $\pm$   7.24 } & 45.00 {\tiny  $\pm$   13.44 } \\
QR-DQN & 76.50 {\tiny  $\pm$   79.76 } & 19.05 {\tiny  $\pm$   6.91 } & 42.05 {\tiny  $\pm$   15.60 } & 62.80 {\tiny  $\pm$   28.71 } & 17.30 {\tiny  $\pm$   7.89 } & 41.00 {\tiny  $\pm$   13.87 } \\
C51 & 51.80 {\tiny  $\pm$   10.74 } & 13.55 {\tiny  $\pm$   7.37 } & 34.75 {\tiny  $\pm$   10.91 } & 60.55 {\tiny  $\pm$   20.44 } & 19.65 {\tiny  $\pm$   7.30 } & 39.90 {\tiny  $\pm$   14.69 } \\\bottomrule
\end{tabular}
}


\end{table}
}
